Marking Data-Informativity and Data-Driven Supervisory Control of Discrete-Event Systems

In this paper we develop a data-driven approach for marking nonblocking supervisory control of discrete-event systems (DES). We consider a setup in which models of DES to be controlled are unknown, but a set of data concerning the behaviors of DES is available. We ask the question: Under what conditions of the available data set can a valid marking noblocking supervisor be designed for the unknown DES to satisfy a given specification? Answering this question, we identify and formalize a novel concept called marking data-informativity. Moreover, we design an algorithm for the verification of this concept. Next, if the data set fails to be marking informative, we propose two related new concepts of restricted marking data-informativity and marking informatizability. Finally, we develop an algorithm to compute the largest subset of control specification for which the data set is least restricted marking informative.

==> tex/Abstract.tex <==
\begin{abstract}

Decentralized supervisory control has received much attention for large-scale discrete-event systems (DES). 
In this thesis, we consider a problem for which there are no streamlined algorithmic solutions for global nonblocking supervisor control. 
This thesis aims to extend the abstraction-based approach into a streamlined algorithm that can conduct horizontal decomposition and vertical aggregation and achieve global nonblocking for large-scale DES.
We first synthesize decentralized supervisors for enforcing each imposed control specification. 
Then we propose a method based on the Markov Cluster Algorithm so that system decomposition is done automatically without the need of engineering insight. 
Then we ensure the nonblockingness of global controlled behavior by computing a coordinator to remove the conflicts among decentralized supervisors on the abstraction level.
The effectiveness of our method is demonstrated on three case studies.

\end{abstract}

==> tex/Acknowledgment.tex <==
\chapter*{Acknowledgment}
I would first like to thank my thesis advisor Dr. Kai Cai of the Dept. of Electrical and Information Engineering, Graduate School of Engineering at Osaka City University. 
The door to Dr. Cai's office was always open whenever I ran into trouble or had a question about my research. 
He steered me in the right direction whenever he thought I needed it. 

I would also like to thank other professors in the department who gave me a lot of help for this research. 
Without their passionate input, the research could not have been successfully conducted. 
Finally, I must express my very profound gratitude to my classmates for providing me with unfailing support and continuous encouragement throughout my years of study and throughout the process of writing this thesis. 
This accomplishment would not have been possible without them. 

==> tex/Chap5.1_Least_restricted_marking_data-informativity.tex <==
%\subsection{Least Restricted Marking Data-Informativiity}\label{sec:Least restricted marking data-informativiity}

We start by defining the following family of subsets of $K_{D_m}$ with respect to which the data set $(D, D_m, D^-)$ is restricted marking informative:
\begin{align} \label{eq:family of K-informative}
    I(K_{D_m}) := \{ K \subseteq K_{D_m} \mid (D, D_m, D^-) \ \text{is} \ \textit{K}\text{-informative} \}.
\end{align}

Thus if $(D, D_m, D^-)$ is marking informatizable, the family $I(K_{D_m})$ contains a nonempty member. Note also that since $K_{D_m} (= D_m \cap E)$ is finite, the number of members in $I(K_{D_m})$ is finite. 

The next result is key, which asserts that the family 

\begin{proposition}\label{prop:K-informatie is closed under the union}
    Consider the family of $I(K_{D_m})$ in (\ref{eq:family of K-informative}). If $K_1, K_2\in I(K_{D_m})$, then $K_1\cup K_2\in I(K_{D_m})$.
\end{proposition}

\begin{proof}
    According to the definition of limited marking informativity, letting $s \in \overline{K_1 \cup K_2}$ and $\sigma \in \Sigma_u$, we will show that $s\sigma \in \overline{K_1 \cup K_2} \cup D^-$. Since $s \in \overline{K_1 \cup K_2} = \overline{K}_1 \cup \overline{K}_2$, either $s \in \overline{K_1}$ or $s \in \overline{K_2}$. Consider the former case $s \in \overline{K_1}$ (the latter case $s \in \overline{K_2}$ is symmetric). Since $(D, D_m, D^-)$ is $K_1$-informative, we have
\begin{align*}
    s\sigma \in \overline{K_1} \cup D^- \subseteq (\overline{K_1} \cup \overline{K_2}) \cup D^- = \overline{K_1 \cup K_2} \cup D^-.
\end{align*}
This completes the proof. 
\end{proof}

\noindent
In view of Proposition \ref{prop:K-informatie is closed under the union}, the family $I(K_{D_m})$ contains a unique largest member $K_{\sup}$, which is the union of all the members in the family:
\begin{align} \label{eq:K_sup}
    K_{\sup} := \bigcup \{K \mid K \in I(K_{D_m})\}. 
\end{align}

With respect to this $K_{\sup} \subseteq \overline{K_{D_m}}$, the data set $(D, D_m, D^-)$ is least restricted marking informative.

The supervisor that enforces $K_{\sup}$ can be constructed for every plant consistent with $(D, D_m, D^-)$ in the same way as Proposition \ref{prop:data-driven supervisor}; due to the maximum largeness of $K_{\sup}$, this supervisor is maximally permissive.

Now that we have shown the existence and uniqueness of the largest subset $K_{\sup}$, we proceed to develop an algorithm to compute $K_{\sup}$.

==> tex/Chap5.2_Non_informative_state.tex <==
\subsection{Non-Informative State}
\label{sec:Non informative state}
For computing $K_{\sup}$, we first introduce a useful concept of \textit{non-informative state}.

Given an event set $\Sigma$, a control specification $E$, and finite data sets $D, D_m, D^- \subseteq \Sigma^*$ (satisfying $D_m\subseteq\overline{D}$ and $\overline{D} \cap D^- = \emptyset$), construct the corresponding data-driven automaton $\hat{G}(\Sigma, D, D_m, D^-) = (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$ with state subsets $Q_K$ (corresponding to $K_{D_m} = D_m \cap E$) and $Q_-$ (corresponding to $D^-$) as in Definition \ref{def:DDA}. We identify those states in $Q_K$ that violate the condition (\ref{eq:informativity}) of marking informativity. These are exactly the states for which the condition in Line 4 of Algorithm \ref{alg:checking informativity} holds. According to the condition, we state the following definition.

\begin{definition}(Non-informative state). \label{def:non-informative state}
Consider the data-driven automaton \\$\hat{G}(\Sigma, D, D_m, D^-) = (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$ with state subsets $Q_K$, $Q_-$ (as in Definition \ref{def:DDA}). We say that $\hat{q} \in Q_K$ is a non-informative state if
\begin{align} \label{eq:non-informative state}
    (\exists \sigma \in \Sigma_u) \hspace{0.1cm}\hat{\delta}(\hat{q}, \sigma) \in \hat{Q} \setminus (Q_K \cup Q_-) \quad \text{or} \quad \neg \hat{\delta}(\hat{q}, \sigma)!
\end{align}
In addition, define the set of non-informative states as follows:
\begin{align} \label{eq:non-informative state set}
    N(Q_K) := \{ \hat{q} \in Q_K \mid \hat{q} \ \text{is a non-informative state} \}. 
\end{align}
\end{definition}

The set $N(Q_K)$ in (\ref{eq:non-informative state set}) provides an alternative characterization (to Proposition \ref{prop:correctness of checking informativity}) for marking informativity as asserted below.

\begin{proposition} \label{prop:Non-informative state set and informativity}
Consider an event set $\Sigma = \Sigma_c \cup \Sigma_u$, finite data sets $D, D_m, D^- \subseteq \Sigma^*$ (satisfying $D_m\subseteq\overline{D}$, $\overline{D} \cap D^- = \emptyset$), a control specification $E \subseteq \Sigma^*$, a subset $K \subseteq K_{D_m}$ with $K_{D_m}$ in (\ref{eq:spec besed on Dm}), a corresponding data-driven automaton $\hat{G}(\Sigma, D, D_m, D^-) = (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$, and the non-informative state set $N(Q_K)$ in (\ref{eq:non-informative state set}). Then the following hold:
\begin{center}
    $N(Q_K) = \emptyset$ if and only if $(D, D_m, D^-)$ is marking informative for $E$.
\end{center}
\end{proposition}

\begin{proof}
  According to Algorithm \ref{alg:checking informativity}, $N(Q_K) = \emptyset$ if and only if the condition in Line 4 is never satisfied, which in turn means that Algorithm\ref{alg:checking informativity} returns “marking informative”. It then follows from Proposition \ref{prop:correctness of checking informativity} that Algorithm \ref{alg:checking informativity} returns “marking informative” if and only if $(D, D_m, D^-)$ is marking informative for $E$; hence the conclusion holds.
\end{proof}

The computation of the non-informative state set can be
adapted from Algorithm~\ref{alg:checking informativity}: instead of returning “not marking informative” immediately after identifying the first non-informative state, the new algorithm checks all states in $Q_K$ against all uncontrollable events in $\Sigma_u$, and stores all identified non-informative states. This new algorithm of computing $N(Q_K)$ is presented in Algorithm~\ref{alg:non-informative state set} below.

\begin{algorithm}
\caption{Non-informative state set}
\label{alg:non-informative state set}
\begin{algorithmic}[1]
\REQUIRE Event set $\Sigma = \Sigma_c \cup \Sigma_u$, finite sets $D, D_m, D^- (\subseteq \Sigma^*)$, control specification $K_{D_m} = D_m \cap E$
\ENSURE Non-informative state set $N(Q_K)$
\STATE Construct a data-driven automaton $\hat{G}(\Sigma, D, D_m, D^-) = (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$ and $Q_K, Q_-$ (as in Definition \ref{def:DDA})
\STATE $N(Q_K) = \emptyset$
\FORALL{$\hat{q} \in Q_K$}
    \FORALL{$\sigma \in \Sigma_u$}
        \IF{($\hat{\delta}(\hat{q}, \sigma)!$ \AND $\hat{\delta}(\hat{q}, \sigma) \in \hat{Q} \setminus (Q_K \cup Q_-)$) \OR ($\neg\hat{\delta}(\hat{q}, \sigma)!$)}
            \STATE $N(Q_K) = N(Q_K) \cup \{\hat{q}\}$
        \ENDIF
    \ENDFOR
\ENDFOR
\RETURN $N(Q_K)$
\end{algorithmic}
\end{algorithm}

The correctness of Algorithm \ref{alg:non-informative state set} is immediate from Definition \ref{def:non-informative state}.

==> tex/Chap5.3_Algorithm_for_checking_informatizability_and_computing_K_sup.tex <==
\subsection{Algorithm for Checking Marking Informatizability and Computing $K_{sup}$}
\label{sec:Algorithm for checking informatizability and computing K_sup}
Having introduced and identified the set $N(Q_K)$ of non-informative states in the data-driven automaton $\hat{G}$, it follows from its definition (Definition \ref{def:non-informative state}) that any string in $\overline{K_{D_m}}$ that reaches a non-informative state in $N(Q_K)$ must be excluded in order to achieve restricted marking informativity.
For achieving least restricted marking informativity, namely computing $K_{\sup} \subseteq K_{D_m}$ (as in (\ref{eq:K_sup})), such exclusion (of strings entering $N(Q_K)$) must be done in a minimally intrusive manner.

We propose to compute $K_{\sup}$ in (\ref{eq:K_sup}) based on the structure of the data-driven automaton $\hat{G}$. 
Thus intuitively, the above mentioned string exclusion amounts to ‘avoiding’ the subset $N(Q_K)$ of states in the data-driven automaton $\hat{G}$. 
In order to obtain the largest $K_{\sup} \subseteq K_{D_m}$, the ‘avoidance’ of $N(Q_K)$ should be performed as ‘close’ as possible to $N(Q_K)$ and by means of removing a controllable event. 
This strategy is similar to that of computing the supremal controllable sublanguage in the standard model-based supervisory control theory. 
In view of this, we craft a supervisory control problem based on a modified structure of the data-driven automaton with the specification of avoiding $N(Q_K)$, and solve this problem by the \textbf{supcon} function in (\ref{eq:supcon}) in order to obtain $K_{\sup}$ in (\ref{eq:K_sup}).

Specifically, we define the following relevant automaton. Given an event set $\Sigma$, a control specification $E$, and finite data sets $D, D_m, D^- \subseteq \Sigma^*$, construct the corresponding data-driven automaton $\hat{G}(\Sigma, D, D_m, D^-) = (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$ with state subsets $Q_K$ (corresponding to $K_{D_m} = D_m \cap E$) and $Q_-$ (corresponding to $D^-$) as in Definition \ref{def:DDA}. First, construct a subautomaton $G_D$ of the data-driven automaton $\hat{G}$ by removing $Q_{r_1}:= \{\hat{q}_s \mid (\forall s\in \overline{D\cup D^-}) s \notin \overline{D}\}$ 
(i.e. the state set of subautomaton is $\{\hat{\delta}(\hat{q}_{\epsilon}, s)! \mid \forall s \in \overline{D} \}$ )
and the corresponding transitions; namely
\begin{align} \label{eq:PLANT for K_sup}
    G_D = (Q_D, \Sigma, \delta_D, \hat{q}_\epsilon, \hat{Q}_m) 
\end{align}
where $Q_D := \hat{Q} \setminus Q_{r_1}$ and $\delta_D := \hat{\delta} \setminus \{ (\hat{q}, \sigma) \to \hat{q}' \mid \hat{q} \in Q_{r_1}$ or $\hat{q}' \in Q_{r_1} \}$. Note that from Definition \ref{def:DDA} and $D_m \subseteq \overline{D}$, it follows that the marker states remain unchanged even when $Q_{r_1}$ is removed from $\hat{Q}$.
Also, we have $L(G_D) = \overline{D}, L_m(G_D)=D_m$. This automaton $G_D$ will serve as the plant in \textbf{supcon} function.

Next, let $Q_{r_2} := Q_D \setminus Q_K$ and construct a subautomaton $S_D$ of $G_D$ by removing $N(Q_K) \cup Q_{r_2}$ and the corresponding transitions; namely
\begin{align} \label{eq:SPEC for K_sup}
    S_D = (Q_S, \Sigma, \delta_S, \hat{q}_\epsilon, Q_{S,m})
\end{align}
where $Q_S = Q_D \setminus (N(Q_K) \cup Q_{r_2}) = Q_K \setminus N(Q_K)$ and $\delta_S := \delta_D \setminus \{ (\hat{q}, \sigma) \to \hat{q}' \mid \hat{q} \in N(Q_K) \cup Q_{r_2} \ \text{or} \ \hat{q}' \in N(Q_K) \cup Q_{r_2} \}$, $Q_{S, m}:= \hat{Q}_m\setminus N(Q_K)\cup Q_{r_2}$. This automaton $S_D$ will serve as the specification in \textbf{supcon} function. Note that since $Q_S = Q_K \setminus N(Q_K)$, every state in $q \in Q_S$ satisfies the negation of (\ref{eq:non-informative state}):
\begin{align} \label{eq:property of S_D}
    (\forall \sigma \in \Sigma_u) \ \hat{\delta}(q, \sigma)! \ \text{and} \ \hat{\delta}(q, \sigma) \in Q_K \cup Q_-. 
\end{align}

Let the plant be \( G_D \) in (\ref{eq:PLANT for K_sup}) and the specification be \( S_D \) in (\ref{eq:SPEC for K_sup}). Using the \textbf{supcon} function, the maximally permissive supervisor is computed, which is also an automaton (indeed in this case a subautomaton of \( S_D \)):
\begin{align}\label{eq:supcon(G_D, G_S)}
    P_D=\textbf{supcon}(G_D, S_D)=(Q_P, \Sigma, \delta_P, \hat{q}_\epsilon, Q_{P,m})  
\end{align}
where $Q_P\subseteq Q_S$, $\delta_P\subseteq \delta_S$ and 
$Q_{P,m}\subseteq Q_{S,m}$ such that
\begin{align*}
    L_m(P_D)=\text{sup} \hspace{0.08cm}C(L_m(S_D))
\end{align*}
where
\begin{align}\label{eq:C(L_m(S_D))の性質}
    C(L_m(S_D))=\{K\subseteq L_m(S_D) \mid \overline{K}\Sigma_u\cap L(G_D)\subseteq \overline{K}\}.
\end{align}.

We summarize the above procedure in the form of an algorithm below. The resulting $L_m(P_D)$ is exactly the largest $K_{\sup}$ in (\ref{eq:K_sup}) we are after. Also, if $L_m(P_D)=K_{\sup}\neq \emptyset$, then ($D, D_m, D^-$) is $K_{\sup}$-informative, so ($D, D_m, D^-$) is marking informatizable. On the other hand, if $L_m(P_D)=K_{\sup}= \emptyset$, then no nonempty subset exists for which ($D, D_m, D^-$) is restricted marking informative, so ($D, D_m, D^-$) is nor marking informatizable. Hence the nonemptyness of the following Alghrithm \ref{alg:informatizability and K_sup} serves checking marking informatizability.

\begin{algorithm}
\caption{checking marking informatizability and computing $K_{\sup}$}
\label{alg:informatizability and K_sup}
\begin{algorithmic}[1]
\REQUIRE Event set $\Sigma = \Sigma_c \cup \Sigma_u$, finite sets $D, D_m, D^- (\subseteq \Sigma^*)$, control specification $K_{D_m} = D_m \cap E$
\ENSURE (``marking informatizable'' and $L_m(P_D)$) or ``not marking informatizable''
\STATE Construct a data-driven automaton $\hat{G}(\Sigma, D, D_m, D^-)$\\ $= (\hat{Q}, \Sigma, \hat{\delta}, \hat{q}_\epsilon, \hat{Q}_m)$ and $Q_K, Q_-$ (as in Definition \ref{def:DDA})
\STATE Construct a subautomaton $G_D$ of $\hat{G}$ as in (\ref{eq:PLANT for K_sup})
\STATE Compute non-informative state set $N(Q_K)$ by Algorithm \ref{alg:non-informative state set}
\STATE Construct a subautomaton $S_D$ of $G_D$ as in (\ref{eq:SPEC for K_sup})
\STATE Compute $P_D=\textbf{supcon}(G_D, S_D)$ as in (\ref{eq:supcon(G_D, G_S)})
\IF{$L_m(P_D) \neq \emptyset$ }
\RETURN ``marking informatizable'' and $L_m(P_D)$
\ELSE
\RETURN ``not marking informatizable''
\ENDIF
\end{algorithmic}
\end{algorithm}

\begin{proposition} \label{prop:Informatizability and K_sup of algorithm}
 The following statements hold for Algorithm \ref{alg:informatizability and K_sup}:

1. The language $L_m(P_D)$ returned by Algorithm \ref{alg:informatizability and K_sup} satisfies $L_m(P_D) = K_{\text{sup}}$ in (\ref{eq:K_sup}).

2. Algorithm \ref{alg:informatizability and K_sup} returns ``marking informatizable'' if and only if $(D, D_m, D^-)$ is ``marking informatizable'' for $E$.


\end{proposition}

\begin{proof}
The proof proceeds in two parts. In Part 1, we establish that the language \(L_m(P_D)\) returned by Algorithm \ref{alg:informatizability and K_sup} satisfies \(L_m(P_D) = K_{\text{sup}}\) in (\ref{eq:K_sup}). We make the following key claim:
\[
C(L_m(S_D)) = I(K_{D_m}).
\]
\noindent
Namely, the family \(C(L_m(S_D))\) in (\ref{eq:C(L_m(S_D))の性質}) of all controllable sublanguages of \(L_m(S_D)\) is exactly the same as the family \(I(K_{D_m})\) in (\ref{eq:family of K-informative}) of all subsets of \(K_{D_m}\) for which \((D, D_m, D^-)\) is restricted marking informative. Under this claim, we derive
\[
L_m(P_D) = \sup C(L_m(S_D)) = \bigcup \{K \mid K \in C(L_m(S_D))\}
= \bigcup \{K \mid K \in I(K_{D_m})\} = K_{\text{sup}}.
\]
\noindent
The last equality is from (\ref{eq:K_sup}), and our conclusion is established.

Now we prove the claim. First, let \(K \in C(L_m(S_D))\), which means that \(K_{D_m} \subseteq L(S_D)\) and \(\overline{K}\Sigma_u \cap L(G_D) \subseteq \overline{K}\). By the definition of \(S_D\) in (\ref{eq:SPEC for K_sup}), \(Q_S \subseteq Q_K\) and thus \(L_m(S_D) \subseteq K_{D_m}\), which in turn implies that \(K \subseteq K_{D_m}
\). In order to show that \(K \in I(K_{D_m})\), we must prove that \((D, D_m, D^-)\) is \(K\)-informative.
For this, let \(s \in \overline{K}\) and \(\sigma \in \Sigma_u\). If \(s\sigma \in L(G_D)\), then it follows from \(\overline{K}\Sigma_u \cap L(G_D) \subseteq \overline{K}\) that \(s\sigma \in \overline{K}\). On the other hand, if \(s\sigma \notin L(G_D)\), we derive \(s\sigma \in D^-\). To see this, consider the state \(q_s\), which is in \(Q_S = Q_K \setminus N(Q_K)\). This means that (\ref{eq:property of S_D}) holds for \(q_s\). But \(\delta(q_s, \sigma)\) cannot be in \(Q_K\) since \(s \notin L(G_D) = \overline{D} \subseteq K_{D_m}\). Thus it is only possible that \(\delta(q_s, \sigma) \in Q_-\), which implies that \(s\sigma \in D^-\). 
To summarize, for an arbitrary \(s \in \overline{K}\) and an arbitrary \(\sigma \in \Sigma_u\), we have \(s\sigma \in \overline{K} \cup D^-\), which means that \((D, D_m, D^-)\) is \(K\)-informative. Therefore, \(K \in I(K_{D_m})\), and \(C(L_m(S_D)) \subseteq I(K_{D_m})\).

It remains to prove that \(I(K_{D_m}) \subseteq C(L_m(S_D))\). Let \(K \in I(K_{D_m})\), which means that \(K \subseteq K_{D_m}\) and \((D, D_m, D^-)\) is \(K\)-informative. Consider an arbitrary string \(s \in K \subseteq K_{D_m}\). Since \((D, D_m, D^-)\) is \(K\)-informative, the state \(q_s \in Q_K \setminus N(Q_K) = Q_S\). Hence \(s \in L_m(S_D)\), and in turn we have \(K \subseteq L_m(S_D)\). 
To show that \(K \in C(L_m(S_D))\), we need to establish that \(K\) is controllable with respect to \(G_D\). To this end, let \(s \in \overline{K}, \sigma \in \Sigma_u\), and assume that \(s\sigma \in L(G_D) = \overline{D}\). It follows again from \(K\)-informativity of \((D, D_m, D^-)\) that \(s\sigma \in \overline{K} \cup D^-\). But we have assumed that \(s\sigma \in \overline{D}\), so it is impossible that \(s\sigma \in D^-\) (by \(\overline{D} \cap D^- = \emptyset\)). Hence \(s\sigma \in \overline{K}\), which means that \(K\) is controllable with respect to \(G_D\). Therefore \(K \in C(L_m(S_D))\), and $I(K_D) \subseteq C(L(S_D))$.

In view of the above, we have established our claim that 
$I(K_{D_m}) = C(L_m(S_D))$,
and the proof of Part 1 is now completed. 

Next, we proceed to Part 2, where we prove that Algorithm \ref{alg:informatizability and K_sup} returns ``marking informatizable'' if and only if \((D, D_m, D^-)\) is ``marking informatizable'' for \(E\). By the first statement of Propositon \ref{prop:Informatizability and K_sup of algorithm}, Algorithm \ref{alg:informatizability and K_sup}
correctly computes the largest subset of $K_{D_m}$ for which the data set $(D, D_m, D^-)$ is least restricted marking informative. If Algorithm \ref{alg:informatizability and K_sup} returns ``marking informatizable'', then $L_m(P_D)=K_{\sup}\neq\emptyset$, which in turn implies $(D, D_m, D^-)$ is $K_{\sup}$-informative, so $(D, D_m, D^-)$ is marking informatizable. On the other hand, if Algorithm \ref{alg:informatizability and K_sup} returns ``not marking informatizable'', then $L_m(P_D)=K_{\sup}=\emptyset$, which in turn implies no empty subset exists for which $(D, D_m, D^-)$ is restricted marking informative, which means that $(D, D_m, D^-)$ is not marking informatizable. The proof of Part 2 is completed.
\end{proof}

We provide an illustrative example for Algorithm \ref{alg:informatizability and K_sup}. 

\begin{example} \label{ex9: checking informatizability and compute K_sup}
Consider the event set $\Sigma=\Sigma_c\cup \Sigma_u$, where $\Sigma_c=\{a, b, c, e, f\}$ and $\Sigma_u=\{d\}$, and  the finite date set $(D_5, D_{m5}, D_5^-)$, where
\begin{align*}
    D_5\hspace{0.22cm} &= \{abe, acfd, aed\},\\
    D_{m5} &= \{ab, abe, acf, aed\},\\
    D_5^-\hspace{0.18cm} &=\{d, ad, acd, aedd\}.
\end{align*}
Let $E=\{ab, acf, aed\}$. Then the control specification in (\ref{eq:spec besed on Dm}) is $K_{D_{m4}}=\{ab, acf, aed\}$. The corresponding data-driven automaton $\hat{G}_5$ is shown in Fig \ref{fig:DDA_G5}.

\begin{figure}[H]
  \centering
  \includegraphics[width=80mm]
  {fig/Chap5_DDA_G5}
  \caption{Data-driven automaton $\hat{G}_5$ corresponding to $(D_5, D_{m5}, D_5^-)$. \label{fig:DDA_G5}}
\end{figure}

\noindent
By applying Algorithm \ref{alg:checking informativity}, it is determined that $(D_5, D_{m5}, D_5^-)$ is ``not marking informative'' for $E$. 
However, $(D_5, D_{m5}, D_5^-)$ may be ``marking informatizable'', and there may exist a nonempty sublanguage of $K_{D_{m5}}$ for which $(D_5, D_{m5}, D_5^-)$ is limited marking informative. 
Next we apply Algorithm \ref{alg:informatizability and K_sup} to check marking informatizability and compute the largest such sublanguage.

Line 1 in Algorithm \ref{alg:informatizability and K_sup} of constructing the data-driven automaton \( \hat{G}_5 \) has been done, as displayed in Fig. \ref{fig:DDA_G5}.
Line 2 computes the subautomaton \( G_{D_5} \) by removing the states in \( Q_{r1}=Q_- \) from \( \hat{G}_5 \) and the relevant transitions (as in (\ref{eq:PLANT for K_sup})); the result is displayed in Fig. \ref{fig:PLANT G_D5}.
\begin{figure}[H]
  \centering
  \includegraphics[width=80mm]
  {fig/Chap5_G_D5}
  \caption{Subautomaton $G_{D_5}$ by Line 2 of Algorithm \ref{alg:informatizability and K_sup}. \label{fig:PLANT G_D5}}
\end{figure}

\noindent
Line 3 applies Algorithm \ref{alg:non-informative state set} to derive the set of non-informative states: \( N(Q_K) = \{ \hat{q}_{ab}, \hat{q}_{acf} \} \). The reason why these two states are non-informative states is as follows: for $\hat{q}_{ab}\in Q_K$ and the uncontrollable event $d$, $\neg\hat{\delta}(\hat{q}_{ab}, d)!$; for $\hat{q}_{acf}\in Q_K$ and the uncontrollable event $d$, $\hat{\delta}(\hat{q}_{acf}, d)!$ and $\hat{\delta}(\hat{q}_{acf}, d)\notin Q_K \cup Q_-$. 
Line 4 constructs subautomaton $S_{D_5}$ by removing the two states in $N(Q_K)$ and the two states in $Q_{r_2}$ (white color coded) from $G_{D_5}$ including the relavant transitions; the result is displayed in Fig. \ref{fig:SPEC S_D5}.
\begin{figure}[H]
  \centering
  \includegraphics[width=80mm]
  {fig/Chap5_S_D5}
  \caption{Subautomaton $S_{D_5}$ by Line 4 of Algorithm \ref{alg:informatizability and K_sup}. \label{fig:SPEC S_D5}}
\end{figure}

\noindent
Finally, Line 5 compute the maximally permissive supervisor $P_{D_5}=\textbf{supcon}(G_{D_5}, S_{D_5})$; the result is displayed in Fig \ref{fig:supervisor P_D5}. 
\begin{figure}[H]
  \centering
  \includegraphics[width=80mm]
  {fig/Chap5_P_D5}
  \caption{Supervisor $P_{D_5}$ by Line 5 of Algorithm \ref{alg:informatizability and K_sup}. \label{fig:supervisor P_D5}}
\end{figure}

\noindent
Comparing to $S_{D_5}$, $\hat{q}_{ac}$ is removed. This is because ensuring the supervisor $P_{D_5}$ is nonblocking ($\hat{q}_{ac}$ is reachable but not coreachable). Hence the final result is ($D_5, D_{m5}, D_5^-$) is marking informatizable and $L_m(P_{D_5})=\{aed\}$ which is the largest subset of $K_{D_{m5}}$ for which the data set $(D_5, D_{m5}, D_5^-)$ is least restricted marking informative.

Based on $K_{\sup}=L_m(P_{D_5})$, we can construct the corresponding supervisor $V_{\sup}:\overline{D_5}\to Pwr(\Sigma_c)$ such that $L_m(V_{\sup}/G) = K_{\sup}$ for every plant $G$ consistent with ($D_5, D_{m5}, D_5^-$) as follows:
\begin{align}
V_{\sup}(s) = \left\{
\begin{array}{ll}
     \{b, c, e, f\} &\text{if } s = \epsilon, \\
     \{a, b, c, f\} &\text{if } s = a, \\
     \{a, b, c, e, f\} &\text{if } s \in \{ae, aed\}, \\
     \emptyset & \text{if } s \in \overline{D_5} \setminus \overline{K_{\sup}}. \nonumber
\end{array}
\right.
\end{align}
\end{example}

==> tex/Chap5_Least_restricted_marking_data-informativity.tex <==
\chapter{Least Restricted Marking Data-Informativity}
\label{chap:Least restricted marking data-informativity}

If marking informatizability of the data set $(D, D_m, D^-)$ is verified to hold, then the existence of a nonempty subset $K \subseteq K_{D_m}$ is assured such that $(D, D_m, D^-)$ is \textit{K}-informative. Namely, $(D, D_m, D^-)$ satisfies restricted marking informative wrt. $K$. In this chapter, we further investigate how to systematically find such a nonempty $K$. Of particular interest is to find (if possible) the largest $K_{\sup} \subseteq K_{D_m}$, so that $(D, D_m, D^-)$ is least restricted marking informative wrt. $K_{\sup}$. Then the corresponding supervisor that enforces $K_{\sup}$ is the maximally permissive one in the sense of allowing the largest set of behaviors as possible.

\input{tex/Chap5.1_Least restricted marking data-informativity}
\input{tex/Chap5.2_Non informative state}
\input{tex/Chap5.3_Algorithm for checking informatizability and computing K_sup}

==> tex/Chapter1_Introduction.tex <==
\chapter{Introduction}
In the past decades, the drastically growing communication networks have reduced the cost of distributed systems particularly the discrete-event system (DES).
The supervisory control theory(SCT) \cite{SCT1987} \cite{SCT1989} is one common method being used for DES. For large-scale DES, considerable attention have been paid\cite{SUPLOC}: examples include automated guided vehicles system, multi-robot search teams, and wireless sensor networks. 
 However, the SCT implementation in large-scale DES are facing challenges due to the state space explosion \cite{SCT1989,GW00}.
%%总介绍

To reduce the computational effort of the supervisor synthesis for large-scale DES, various modular control architectures have been conducted: decentralized \cite{Rudie1992,Queiroz2000,Goorden2021RCNMS},
hierarchical \cite{Zhong1990,Wong1996}, and heterarchical \cite{Wong1998,Feng2008,Su2010,Mohajerani2015,Schmidt2011,Komenda2016,Goorden2020}.
Decentralized architecture \cite{Rudie1992,Queiroz2000,Goorden2021RCNMS} can be classified as horizontal modularity, wherein the overall supervision task is divided into several smaller-scale subtasks.
By contrast, the hierarchical architecture \cite{Zhong1990,Wong1996} can be classified as vertical modularity, which separates the overall supervision task
into high-level commands and low-level implementation.
Heterarchical synthesis explores both horizontal and vertical modularity of large-scale DES. In heterarchical architecture, the plant is controlled by a hierarchy of decentralized supervisors and coordinators.
%De 和Hi 是 Heter的特殊情况
Heterarchical synthesis consists of horizontal decomposition and vertical aggregation, which can be effective approaches to handling complexity.
%d)	Heter还不能解决的的问题
%HD和VA的说明

Horizontal decomposition means partitioning the plant components and specifications into subsystems. Papers \cite{Wong1998,Feng2008,Su2010,Mohajerani2015,Schmidt2011,Komenda2016,Goorden2020} all include horizontal decomposition. 
Most of these approaches need engineering insight which means the specific information of structure in conducting horizontal decomposition, but recent research \cite{Goorden2020} presents an algorithm that does not need the information of system structure.
In \cite{Feng2008}, horizontal decomposition is supported by a directed graph called the $control$-$flow$ $net$ \cite{Feng2006}. All plant components and specifications in \cite{Feng2006} are first constructed into a control-flow net by checking the share events between plant components and specifications. 
Then the graph is simplified by temporarily disregarding the parts irrelevant to the global nonblocking property described in \cite{Feng2006}.
After the control-flow net conduct, the conflicts check can be carried out on a simplified system. But in the large-scale system, the simplified system
%用shareevent造有向图，然后减少图的体积，但是最后的图如果系统太大的话，还是需要人去判断分subsystem
still needs more partition before the conflicts check, see \cite{Feng2008}.

%VA
Vertical aggregation includes two methods. One is the model abstraction, and the other is constructing a tree-structured for multilevel supervisory
control. These two methods can be implemented algorithmically. The model abstraction way can achieve global nonblocking, but the multilevel way can not. \cite{Wong1998,Feng2008,Su2010,Mohajerani2015,Schmidt2011} use several model abstraction techniques to do supervisor synthesis and coordination on abstracted models achieving the overall nonblocking control. Moreover, \cite{Wong1998,Feng2008,Schmidt2011} introduce the conditions that make model abstraction also achieve maximal permission.
%没有自动化
%multilevel 不归到
%介绍vertical 时要介绍multilevel
%所有文章都有做HD
%但是martin有自动化的方法
%Ver有两种方法，两种方法都能自动实现，但是只有abs的方法可以实现无冲突
%vertical移到后面去，先说HD，HD里要加上control flow net
%The vertical aggregation  The relationship between each plant component and specification also can be found easily by checking share events. However, partitioning the plant components and specifications for horizontal decomposition still needs engineering insight about the system.
%control-flow
On the other hand, \cite{Goorden2020} presents an approach to algorithmically construct a set of plant models and a set of requirement models into a tree-structured multilevel discrete-event system (MLDES) defined in \cite{Komenda2016}.
But \cite{Goorden2020} is unable to guarantee that the multilevel supervisors are nonblocking when the case of non-prefix closed requirements exist.
%
%system decomposition

%clustering

%i所以，综合起来说，现在还没有一个自动能解决
%我们需要一个overall alg，它既可以自动做HD和VA，而且可以实现gobal nonblocking
So far, the algorithmic horizontal decomposition methods in abstraction-based approaches like events sharing may make the partition in the large system too big for computation. Our study aims to extend the abstraction-based approach into a streamlined algorithm that can conduct horizontal decomposition and vertical aggregation and achieve global nonblocking for large-scale DES. We combine the horizontal decomposition by algorithmic construction, including the clustering method and the abstraction-based heterarchical nonblocking supervisory control for large-scale systems. We will introduce these two types of approaches in the following.

%接下来开始介绍两种方法
First, for the approach for horizontal decomposition,
\cite{Goorden2020} presents a framework that algorithmically constructs a set of plant models and a set of specification models into a tree-structured multilevel discrete-event system (MLDES) originated in \cite{Komenda2016}.
In a multilevel system in \cite{Komenda2016}, each subsystem has a unique parent node and may have a set of one or more lower-level nodes, and a supervisor be synthesized in each node.
The main contribution of \cite{Goorden2020} is constructing MLDES without the additional information about the system's structure by using Dependency Structure Matrices (DSMs) to record the relationship between each plant and control specification models. Each node in the tree structure is determined by the extended-Markov clustering algorithm (MCL) stated in \cite{Wilschut2017} which is originally from \cite{MCL}.
The details of DSM and MCL will be introduced in Chapter 2.
%我们为什么不直接用7和8，因为没法nonblock
The MLDES approach is still unable to guarantee that the multilevel supervisors are nonblocking. That is the reason that we use both the abstraction-based and clustering approach.

%%%%%2.	直接介绍【Feng2008】：建一个ABS的方法，解决NB，ABS的方法，用了natob occ我们基于18
The abstraction-based synthesis is a powerful way for nonblocking verification and synthesis of large-scale heterarchical control.
There are several similar abstraction techniques \cite{Feng2008,Su2010,Mohajerani2015,Schmidt2011}.
%%写明我们只是选了其中一个代表的来
In this thesis, we select the abstraction-based approach in \cite{Feng2008}, but our approach also can be applied using the others abstraction approach in a similar way.
\cite{Feng2008} constructs a system architecture by the procedure that decomposes the system comprised of modules(subsystems) and abstracts the subsystems by natural projections with special properties. Thus, the conflicts check can be applied in smaller abstracted automaton to reduce computational cost. Then coordinators for the abstracted models are designed to resolve the conflicts. To ensure that when the abstracted models are nonconflicting, then so is the original subsystems, there are two essential concepts: the {\it Natural Observer} property \cite{Wong1996} for nonblocking and {\it Output Control Consistency} (OCC) \cite{OCC} for maximal permission.
The natural observer and OCC property are introduced in Chapter 2.
These two properties are used as sufficient conditions to ensure obtaining correct abstraction.

For the other abstraction-based approaches\cite{Su2010,Mohajerani2015,Schmidt2011}, below is a brief introduction.
%Su2010
\cite{Su2010} presents the automaton-based abstraction.
%Mohajerani2015
\cite{Mohajerani2015} constructs the abstraction for an extend finite state machine (EFSM) and FSM by finding the local events that only appear in one automaton in the system first, then hiding local events and merging the state that is connected by the local events.
%Schmidt201 用了不同的natural projection , (msa-projection)
\cite{Schmidt2011} uses another observer property for nonblocking in natural projection, called {\it marked string
accepting (msa)-observers} property. %还要加msa说明
For maximal permission, \cite{Schmidt2011} also presents a  property {\it local control consistency} (LCC) for model abstraction and LCC is less restrictive than OCC.
%which can be used in \cite{Feng2008}.
%但是他们分大系统时都没有自动的方法
However, horizontal decomposition in abstraction-based approaches requires engineering insight into the 
structure of the specific system.
%
%%加连接！！
%%%现在我们已经介绍了这两种方法了，接下来是我们方法的和他们各自的区别。

We have introduced the clustering approach and the abstraction-based approach. 
Now let us introduce our approach and point out the difference from above two approaches.
%和martin有主要2个区别
%解释为什么DSM的区别？我们要为了做ABS的做的调整
%DSM区别：Goodren里的cluster主体是plant conponent，如果没有只和这些cluster有关的spec，这个cluster就不会被分配spec
%【If a node does not show a requirement model Kn, none of the original requirements is placed at this node. A node will not get assigned any requirement if there are no requirements related to only the plant models in that node.】
%%
%%%先介绍我们的方法
We first model all plant components and specifications, and then synthesize a decentralized supervisor for each specification.
We employ the MCL algorithm to cluster these synthesized decentralized supervisors. 
To this end, we use DSM to record the relationship between each plant and control specification models.
We then check if conflicts exist in each cluster. If so, we design a supervisor called coordinator to remove the conflicts.
After ensuring each cluster is nonblocking, we then employ the model abstraction approach to compute an abstract model of each nonblocking cluster.
Repeat the clustering, conflicts removing, and model abstraction steps until there are not greater than two only clusters.
Finally ensure the nonblockingness of this single, top-level cluster by coordinator design. Thereby, a set of decentralized supervisors and hierarchical coordinators are generated which collectively guarantee the overall nonblocking of the entire system.
%%
Our approach mainly has two differences compared to \cite{Goorden2020}.
%DSM
The first is about using DSM to record the relationship between each plant and control specification models.
%Goorden的理由
\cite{Goorden2020} finds clusters in plant components to construct a tree structure, 
so the DSM in \cite{Goorden2020} records the number of specification that uses events from plant components so that the output of MCL will be the plant component clusters.
%我们的理由
In contrast, we record the number of plant components that use events from specifications.
We make this change because we synthesize a decentralized supervisor of each specification before clustering, and we aim to find clusters of decentralized supervisors. The clustering results are the input for the model abstraction step.
The second difference is that we conduct model abstraction in vertical aggregation for ensuring global nonblockingness, which is not guaranteed in [16]. 

Moreover, several other methods are used for horizontal decomposition, including share events checking for \cite{Wong1998,Su2010} and using control-flow net to simplify the structure \cite{Feng2008,Schmidt2011}. However, there is no algorithmic method combining the clustering technique for horizontal decomposition with the vertical abstraction-based approach.
%The control-flow net method \cite{Feng2008} used can also reduce the effort of horizontal decomposition but still require the understanding of system structure in large-scale systems.
%贡献
The contribution of this thesis is to fill this gap by developing an algorithmic solution for the nonblocking heterarchical supervisor control problem. Our approach does not require engineering insight for system structure. Our approach needs only three inputs: plant component models, specifications models, and a clustering parameter (which will be introduced in the next Chapter). The outputs are decentralized supervisors and coordinators, and these supervisors' joint behavior is globally nonblocking (and can be made maximal permissive as well).

%不是单纯的combination，什么贡献：可以重复clustering，自动结束
%We also not only combine these two approaches, we find cluster and do model abstraction multiple times automatically until there is only one cluster remain.






%处理nonbloc 也有16 17这种方法 identify结构上的特
In a different direction, an approach to nonblocking modular control is reported in \cite{Goorden2021RCNMS}.
\cite{Goorden2021RCNMS} firstly introduces a property called Controllable and Nonblocking Modular Supervisors Properties (CNMSP) that the supervisor synthesis is not needed if the system satisfies the CNMSP properties. Namely, only synthesizing the plant and requirement of a control problem satisfying these properties is already controllable and nonblocking.
There are two properties in CNMSP for the plant model: the alphabets of plant components are pairwise disjoint; each automaton is nonblocking and at least has one marked state. CNMSP also has seven properties for requirement model details see Section III in \cite{Goorden2021RCNMS}.
\cite{Goorden2021RCNMS} extends the CNMS properties which is called RCNMS. Namely, the supervisor synthesis step is also unnecessary if a control problem does not satisfy the CNMS properties but satisfies the relaxed RCNMS properties.
The approach introduced in \cite{Goorden2021RCNMS} first checks whether the system satisfies the CNMS properties. If not, check whether that system satisfies RCNMS properties and construct its dependency graph.
The dependency graph is the directed graph, and vertices relate the plant models and the edges to the requirement models. The synthesis step is unnecessary if the dependency graph is acyclic.
%%CNMS的缺点
However, in this approach, plant models need to be partitioned into a set of sensor automaton and actuator automaton.
An automaton is called a sensor automaton if its alphabet has only uncontrollable events and an actuator automaton if its alphabet has only controllable events. These classifications still need comprehension of the system.








%% modular 
%Modular control of DES, introduced in \cite{modular1988}, has been developed to reduce the combinatorial explosion of the state complexity of monolithic supervisor synthesis in large systems. A generalization of the modular supervisory approach applied to DES introduced in \cite{modular2000-1}. Since purely modular approaches fail in general to guarantee the nonblocking safe behavior, \cite{modular1988} initiated an approach that designing an additional supervisor called the coordinator resolves the conflicts between the decentralized supervisors.
%%直接判断会遇到计算上限
%The process of local modularity verification still requires the computation the joint behavior of all interacting decentralized supervisors, what may not commutable in large scale DES. To overcome this difficulty, two directions of approaching introduced bellow.%%第一个分支，减少计算量

%









In the rest of this thesis, preliminaries on decentralized supervisors and coordinators will be introduced in Chapter \ref{chap:pre1}.
Our proposed method is presented in Chapter \ref{chap:method}.
Then we show three case studies to demonstrate the effectiveness of our method in Chapter \ref{chap:4}.

==> tex/Chapter2_Preliminary_DES.tex <==
\chapter{Preliminary}\label{chap:pre1}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Language and Automaton}\label{sec:pre_language}

First, we introduce events, strings, and languages. Let $\Sigma$ be a nonempty finite alphabet of symbols $\sigma, \alpha, \beta, \ldots$. These symbols will denote \textsl{events} and $\Sigma$ the \textsl{event set}. A \textsl{string} $s = \sigma_1 \sigma_2 \dots \sigma_k,k \leq 1$, is a finite sequence of events. Let $\Sigma ^ \ast $ be the set of all finite-length strings including the \textsl{empty string} $\epsilon$, meaning `do noting'. A \textsl{language} $L$ is an arbitrary subset of strings in $\Sigma ^ \ast$, i.e. $L \subseteq \Sigma ^ \ast$.

A string $s_1$ is a \textsl{prefix} of another string $s$, written $s_1 \leq s $, if there exists $s_2$ such that $s_1 s_2 = s$. Both $\epsilon$ and $s$ are prefixes of $s$. The \textsl{prefix closure} of a language $L$, written $\overline{L}$, is 
\begin{equation}
\overline{L} := \{s_1 \in \Sigma ^ \ast | ( \exists s \in L) s_1 \leq s \} .
\end{equation}
It is always true that $L \subseteq \overline{L}$. We say that a language $L$ is \textsl{closed} if $L = \overline{L}$.

A finite-state \textsl{automaton} \textbf{G} is a five-tuple
\begin{equation}
\textbf{G} := (Q,\Sigma,\delta,q_0,Q_m)
\end{equation}
and definition of elements is following.
\begin{itemize}
\setlength{\leftskip}{1.0cm}
\item[$Q$]：The finite state set.
\item[$\Sigma$]：The finite event set.
\item[$\delta$]：The state transition function.
\item[$q_0\in Q$]：The initial state.
\item[$Q_m\subseteq Q$]：The set of marker states.
\end{itemize}
 $\delta : Q\times\Sigma \rightarrow Q$ the (partial) \textsl{state transition function}. 
Letting $\Sigma^*$ denote the set of all finite-length strings of events in $\Sigma$, 
we extend $\delta$ such that $\delta : Q \times \Sigma^* \rightarrow Q$ and write $\delta(q, s)!$ to mean that $\delta(q, s)$ is defined. 

The \textsl{closed behavior} of \textbf{G} is the set of all strings that can be generated by \textbf{G}:
\begin{equation}
L(\textbf{G}):=\{s \in \Sigma^*|\delta(q_0,s)!\}.
\end{equation}
As defined $L(\textbf{G})$ is closed. On the other hand, the \textsl{marked behavior} of \textbf{G} is the subset of strings that can reach a marker state:
\begin{equation}
L_m(\textbf{G}):=\{s \in L(\textbf{G})|\delta(q_0,s) \in Q_m \}\subseteq L(\textbf{G}).
\end{equation}

As in the case of an automaton, a state $q \in Q$ is \textsl{reachable} if 
\begin{equation}
    (\exists s \in \Sigma ^ \ast) \delta(q_0,s)! \: \& \: \delta(q_0,s)=q;
\end{equation}
\textbf{G} itself is \textsl{reachable} if $q$ is reachable for all $q \in Q$. A state $q \in Q$ is \textsl{coreachable} if 
\begin{equation}
    (\exists s \in \Sigma ^ \ast) \delta(q,s) \in Q_m;
\end{equation}
\textbf{G} itself is \textsl{coreachable} if $q$ is coreachable for all $q \in Q$.
\textbf{G} is \textsl{nonblocking} if every reachable state is coreachable, or equivalently $L(\textbf{G}) = \overline{L_m(\textbf{G})}$, namely every string in the closed behavior may be completed to a string in the marked behavior. Finally, \textbf{G} is \textsl{trim} if it is both reachable and coreachable. 


\section{Synchronous Product}\label{sec:pre_sync}
Let $\textbf{G}_i :=  (Q_i,\Sigma_i,\delta_i,q_{0,i},Q_{m,i}),i=1,2$, be two automata. Their \textsl{synchronous product} $\textbf{G}_1 || \textbf{G}_2 = \textbf{G} =  (Q,\Sigma,\delta,q_0,Q_m)$ is defined according to

\begin{align}
Q & =Q_1 \times Q_2, \\
\Sigma & = \Sigma_1 \cup \Sigma_2, \\
q_0 & = (q_{0,1},q_{0,2}), \\
Q_m & = Q_{m,1}\times Q_{m,2}, 
\end{align}

$(\forall (q_1,q_2) \in Q_1 \times Q_2, \forall \sigma \in \Sigma_1 \cup \Sigma_2)$
\begin{equation}
    \delta((q_1,q_2),\sigma)= \left\{\begin{array}{ll}
    (\delta_1(q_1,\sigma),q_2) & (\sigma \in \Sigma_1 \backslash \Sigma_2 \: \textrm{and} \: \delta_1(q_1,\sigma)!); \\
    (q_1,\delta_2(q_2,\sigma)) & (\sigma \in \Sigma_2 \backslash \Sigma_1 \: \textrm{and} \: \delta_2(q_2,\sigma)!); \\
    (\delta_1(q_1,\sigma),\delta_2(q_2,\sigma)) & (\sigma \in \Sigma_1 \cap \Sigma_2\: \textrm{and}\: \delta_1(q_1,\sigma)! \: \textrm{and} \: \delta_2(q_2,\sigma)!); \\
    \textrm{ not\,} \textrm{defined} & \textrm{otherwise}. \end{array} \right. 
\end{equation}

For a subset $\Sigma_o \subseteq \Sigma$, the \textsl{natural projection} $P : \Sigma ^ \ast \rightarrow \Sigma ^ \ast _ o$ is defined according to 

\begin{align}
P(\epsilon)&=\epsilon; \\
P(\sigma) &=   \left\{\begin{array}{ll} 
      \epsilon, \sigma \not \in \Sigma_o, \\
      \sigma, \sigma \in \Sigma_o ;
\end{array} \right. \\
P(s \sigma) &= P(s)P(\sigma), s \in \Sigma^\ast , \sigma \in \Sigma.
\end{align}

That is, $P$ extracts only events included in $\Sigma _o$, ignoring events not included.
Extend $P$ to $P: Pwr(\Sigma^\ast)\rightarrow Pwr(\Sigma^\ast_o)$, where $Pwr(\cdot)$ denotes \textsl{powerset}, and write $P^{-1} : Pwr (\Sigma^\ast_o)\rightarrow Pwr(\Sigma^\ast)$ for the \textsl{inverse-image function} of $P$.
Synchronous product of $L_1$ and $L_2$ is defined as follows:
\begin{equation}
L_1||L_2 := P^{-1}_1 (L_1)\cap P^{-1}_2 (L_2)
\end{equation}
The closed and marked behaviors of the synchronous product $\textbf{G} = \textbf{G}_1 || \textbf{G}_2$ satisfy
\begin{equation}
L(\textbf{G}) = L(\textbf{G}_1) || L(\textbf{G}_2) , \: L_m (\textbf{G}) = L_m (\textbf{G}_1) || L_m (\textbf{G}_2).
\end{equation}


\section{Centralized Supervisory Control}\label{sec:centr_sup}
Now, let \textbf{G} model the plant to be controlled. A \textsl{supervisory control}  enables or disables events in $\Sigma$ from occurring.   
The event set $\Sigma$ of \textbf{G} is partitioned into a subset $\Sigma_c$ of \textsl{controllable} events and a subset $\Sigma_u$ of \textsl{uncontrollable} events. $\Sigma_c$ and $\Sigma_u$ satisfy
\begin{align}
    \Sigma_c \cap \Sigma_u = \emptyset, \\
    \Sigma_c \cup \Sigma_u = \Sigma.
\end{align}

Let $\Gamma$ be the collection of event subsets that always include $\Sigma_u$, i.e.
\begin{equation}
    \Gamma = \{ \gamma \subseteq \Sigma | \Sigma _u \subseteq \gamma \};
\end{equation}
we call each $ \gamma \in \Gamma $ a \textsl{control pattern}, and a supervisory control enables only events which are included in control pattern. 

A \textsl{supervisory control} $S$ for \textbf{G} is any map $S:L(\textbf{G}) \rightarrow \Gamma$, associating to each string in $L(\textbf{G})$ a control pattern. The closed-loop system where \textbf{G} is under the control of $S$ is written $S/\textbf{G}$. The closed language $L(S/\textbf{G})$ of the system  $S/\textbf{G}$ is defined as follow:
\begin{itemize}
    \item $\epsilon \in L(S/\textbf{G})$;
    \item if $s \in L(S/\textbf{G}) \: \& \: \sigma \in S(s) \: \& \: s\sigma \in L(\textbf{G})$, then $s\sigma \in L(S/\textbf{G})$;
    \item no other strings belong to $L(S/\textbf{G})$;
\end{itemize}
where $S(s)$ is the set of events that supervisory control $S$ enables. Thus $\sigma \in S(s)$ means that supervisory control $S$ enables the occurrence of event $\sigma$ just after occurrence of string $s$.
As defined above $L(S/\textbf{G})$ is closed. Let $M \subseteq L_m(\textbf{G}); S$ is \textsl{marking} supervisory control for $(M,\textbf{G})$ if the marked language 
\begin{equation}
    L_m(S/\textbf{G})=L(S/\textbf{G})\cap M.    
\end{equation}
 $S$ is \textsl{nonblocking} if $\overline{L_m(S/\textbf{G})} =L(S/\textbf{G})$.
 
 
%\subsection{Existence Condition of Supervisory Control}\label{sec:pre_condition}
Let \textbf{G} be the plant to be controlled, and \textbf{SPEC} the \textsl{specification} automaton which satisfies $L_m(\textbf{SPEC}) \subseteq L_m(\textbf{G})$.
The goal of the supervisor control problem is to design a \textsl{nonblocking marking supervisor} that satisfies the following:
\begin{equation}
    L_m(S/\textbf{G}) = K,
\end{equation}
where $K = L_m(\textbf{SPEC})$.

A language $K \subseteq \Sigma^*$ is said to be \textsl{controllable} (with respect to \textbf{G}) if $\overline{K}\Sigma_u \cap L(\textbf{G}) \subseteq \overline{K}$, i.e. 
\begin{equation}
(\forall s\in \Sigma^*, \forall \sigma \in \Sigma) s \in \overline{K}, \sigma \in \Sigma_u, s\sigma \in L(\textbf{G}) \Rightarrow s\sigma \in \overline{K}.
\end{equation}
That $K$ is controllable means that if an arbitrary uncontrollable event $\sigma \in \Sigma_u$ occurs after a string $s \in \overline{K}$ and string $s\sigma$ is an element of $L(\textbf{G})$, $s\sigma$ is also an element of $\overline{K}$.

Let $K \subseteq L_m(\textbf{G}), K \not = \emptyset$. Then there exists a \textsl{marking nonbloking supervisory control} $S$ for $(K,\textbf{G})$ such that $L_m(S/\textbf{G}) = K$ if and only if $K$ is controllable.

When the specification language $K$ does not satisfy the necessary and sufficient condition above, that is, there is no supervisory control $S$ that satisfies $L_m(S/\textbf{G}) = K$, one aims to design a supervisory control  that allows as many strings that satisfy the control specification as possible. 

Let $K \subseteq L_m(\textbf{G})$ be a specification language imposed on the plant \textbf{G}. Denote by $\mathcal{C}(K)$ the family of controllable sublanguages of $K$, i.e. 
\begin{equation}\label{eq:ck}
\mathcal{C}(K) := \{ K' \subseteq K \mid \overline{K'}\Sigma_u \cap L(\textbf{G}) \subseteq \overline{K'} \}.
\end{equation}

\iffigure
\begin{figure}[t]
  \centering
  \includegraphics[clip,width=7.0cm]{fig/supervisor_implementation.pdf}
  \caption{Supervisory control implementation} 
  \label{fig:sup_implemention}
\end{figure}
\fi

Then the \textsl{supremal controllable sublanguage} \cite{SCT1987} of $K$ exists and is given by $\sup \mathcal{C}(K) = \cup \{K' \mid K' \in \mathcal{C}(K)\}$. Let \textbf{SUP} be a (nonblocking) automaton such that $L_m(\textbf{SUP}) = \sup \mathcal{C}(K)$. We call  \textbf{SUP} the \textsl{monolithic supervisor} for plant \textbf{G} that enforces $\sup \mathcal{C}(K) \subseteq L_m(\textbf{G})$.The implementation of \textbf{SUP} is illustrated in Fig~\ref{fig:sup_implemention}.

The control action of \textbf{SUP} after an arbitrary string $s \in L(\textbf{G})$ is to enable the events in 
\begin{equation}
\label{gammas}
\gamma := \{\sigma \in \Sigma_u \mid s\sigma \in L(\textbf{G})\} \cup \{\sigma \in \Sigma_c \mid s\sigma \in L(\textbf{SUP})\}.
\end{equation}


==> tex/Chapter2_Preliminary_DeSUP.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Nonblocking and Optimal Decentralized Supervisory Control}

\subsection{Coordinator Design and Model Abstraction}
\label{sec:desup}

    For large-scale DES, the $\textit{decentralized}$ approach usually is used because monolithic supervisor may not be computable owing to state explosion.
Consider a plant ${\bf G}$ consisting of \textit{N} component agents: 
\begin{align}
{\bf G}_k = (Q_k{,}\Sigma_k{,}\delta_k{,}q_{0{,}k}{,}Q_{m{,}k} ), \ k=1,...,N
\end{align}

The behavioral constrain imposed through (local) specification languages $\textit{E}_i\subseteq\Sigma^{\ast}_{\textit{E}_i}(i\in\it{I})$
where $\Sigma_{\textit{E}_i}\subseteq\Sigma$ 
shows the alphabet of $\textit{E}_i$ and the $\it{I}$ is index set.
For each specification $\textit{E}_i$, the decentralized plant $\textbf{G}_{\textit{E}_i}$ is synthesized from the agents that share events with $\Sigma_{\textit{E}_i}$:
\begin{eqnarray}
\textbf{G}_{\textit{E}_i} := ||\{\textbf{G}_k | \Sigma_k \cap \Sigma_{{\it E_i}} \neq\emptyset\}
\end{eqnarray}
Then we synthesize an optimal and nonblocking {\it decentralized} {\it supervisor} $\textbf{SUP}_i$:
\begin{eqnarray}
L_m({\bf SUP}_i)=\textrm{sup}\textit{C}(L_m({\bf E}_i)||L_m(\textbf{G}_{E_i})) 
\end{eqnarray}
In general, the joint behavior of the decentralized supervisors fails to be nonblocking, 
i.e. $||_{i\in I} L(\textbf{SUP}_i)^{\supset}_{\neq} \overline{||{}_{i\in I}L_m(\textbf{SUP}_i)}$.
An additional supervisor $\textbf{CO}$ called the $\textit{coordinator}$ needs to be designed to resolve conflicts:
\begin{eqnarray}
L_m({\bf CO}) := {\rm sup} {\it C}(|| _{{\it i}\in{\it I}}L_m( {\bf SUP}_i))|| \Sigma^{\ast} )\\
||_{i\in I} L(\textbf{SUP}_i) ||L(\textbf{CO})= 
\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||L_m(\textbf{CO})}
\end{eqnarray}
The joint behavior of the supervisors and the coordinator is identical to the monolithic controlled behavior.\\
%%按写完CO然后为了降低SUB复杂度，用ABS去除ABS的冲突，用CO
However, checking conflicts and designing the coordinator as above also may not be feasibly computable 
since the synchronous product of all $\textbf{SUP}_i$ is required. Therefore, we create the abstracted model $\textbf{ABS}_i$ for each $\textbf{SUP}_i$,
and check conflicts and design coordinators for the abstractions. Abstractions $\textbf{ABS}_i$ are obtained by natural projection $\textit{P}_i$ from $\textbf{SUP}_i$:
%%先加上射影的定义，
\begin{eqnarray}
L(\textbf{ABS}_i)=\textit{P}_i L(\textbf{SUP}_i),  \ L_m(\textbf{ABS}_i)=\textit{P}_i L_m(\textbf{SUP}_i)
\end{eqnarray}
\begin{eqnarray}
\label{formular:natob}
\textit{P}_i : \Sigma^{\ast}_{sup,i} \rightarrow \Sigma^{\ast}_{o,i}
\end{eqnarray}
The $\Sigma_{sup,i}$ is the event set of $\textbf{SUP}_i$, and the $\Sigma_{o,i}\subseteq\Sigma_{sup,i}$
is the event set of $\textbf{ABS}_i$. 
We check conflicts and design the coordinator involve computing only the synchronous product of model abstractions $\textbf{ABS}_i$ instead of $\textbf{SUP}_i$
thereby reducing computational cost. Namely if the coordinator $\textbf{CO}$ can resolve the conflicts of  $\textbf{ABS}_i$, it also resolves the conflicts of $\textbf{SUP}_i$.
We design the coordinator first computing
%%%最后写怎么做CO
\begin{eqnarray}
L_m({\bf CO}) := {\rm sup} {\it C}(|| _{{\it i}\in{\it I}}L_m( {\bf ABS}_i))|| \Sigma^{\ast}_o )
\end{eqnarray}
and then applying supervisor reduction to {\bf CO}; thereby we derive that
\begin{eqnarray}
|| _{\it{i}\in\it{I}}L( {\bf ABS}_i)||L({\bf CO}) = 
\overline{|| _{\it{i}\in\it{I} } L_m( {\bf ABS}_i)|| L_m( {\bf CO})}
\end{eqnarray}
Hence checking conflicts and designing the coordinator involve computing only the synchronous product of model abstractions $\textbf{ABS}_i$, thereby reducing computational cost.

 The coordinator \textbf{CO} designed to resolve the conflict of $\textbf{ABS}_i$, then it also resolves the conflict of $\textbf{SUP}_i$. 
 To achieve this condition, natural projection $\textit{P}_i$ need to satisfy {\it natural observer} and {\it output control consistent}(OCC), as will be discussed in the subsection below.
%%%%%%%%%%%%%%%%%%%%NO and  OCC

\subsection{Natural Observers and Output Control Consistent }


\ Suppose that we check conflicts among decentralized supervisors $\textbf{SUP}_i ( i \in \textit{I} )$ and construct the coordinator $\textbf{CO}$ based on abstractions $\textbf{ABS}_i$. To ensure that the joint behavior of the decentralized supervisors and coordinator is globally optimal and nonblocking, there are two key properties of the natural projections $\textit{P}_i$.


For nonblockingness, the natural projections $\textit{P}_i$ needs to be a $\textit{natural observer}$ for a language $L\subseteq\Sigma^{\ast}$, and the following is definition.
\begin{eqnarray}
(\forall s \in \overline{L}, \forall t_o \in \Sigma^{\ast}_o ) P(s)t_o \in P(L)
\end{eqnarray}
\[
\Rightarrow (\exists t \in \Sigma^{\ast}) P(t) = t_o \& st \in L
\]

The definition means that if $\textit{P}$ is $\textit{natural observer}$ for $L$ , $\textit{P(s)}$ can be extended to $\textit{P(L)}$ by an observable string $\textit{t}_o$, the underlying string $s$ can be extended to $L$ by a string $t$ with $\textit{P(t)} = t_o$.


%最大可控制最早由occ提出，然后提出lcc，本文使用的是OCC
%%%

Next we turn to optimality. i.e. maximally permissive behavior. 
%加上最大可控制的简短说明
Maximally permissive supervisor achieving the control objective by enabling or disabling only the necessary controllable events.
%
For an uncontrollable event $\sigma$, the optimally supervisor disables the `nearest' controllable events from $\sigma$. However, if the nearest controllable events from $\sigma$ are unobservable, the supervisor will have to disable controllable events further `upstream'. In that case the supervisor is not optimal because more than necessary strings are being removed. To ensure the optimality, for all unobservable events, the nearest upstream controllable event must all be observable. This property is named $\textit{Output Control Consistency}$(OCC)\cite{OCC} : for every string $s\in L$ of the form
\begin{eqnarray}
s= s^{\prime}\sigma_1 \cdots \sigma_k , k\geq 1
\end{eqnarray}
where $s^{\prime}$ is either the empty string $\epsilon$ or terminates with an event in $\Sigma_o$, the following holds
\[
( (\forall i \in \{1,k-1\} )\sigma_i \in \Sigma \setminus \Sigma_o )  \ \& \  \sigma_k \in \Sigma_o \cap \Sigma_u
\]
\begin{eqnarray}
\Rightarrow ( (\forall j \in \{1,k\} ) \sigma_j \in \Sigma_u )
\end{eqnarray}
This property shows that whenever event $\sigma_k$ is observable and uncontrollable, its immediately preceding unobservable events must all be uncontrollable.

For the other direction, namely `downstream' of an uncontrollable event $\sigma$, \cite{Schmidt2011} shows that the property $\textit{Locally Control Consistency}$ (LCC) also can 
ensure maximally permissive supervision. In this thesis, we ensure the optimality for supervisors by using OCC. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tex/Chapter2_Preliminary_MCL.tex <==

\section{Markov Clustering Algorithm}

The Markov Clustering Algorithm (MCL)\cite{MCL} is a graph clustering method that find the clusters by producing Random Walk on the graph. The following introduces MCL.

\subsection{Main procedure of MCL algorithm}\label{main_MCL}
The input of MCL algorithm described in \cite{MCLMatrix} is a stochastic matrix {\bf M} and the column elements of {\bf M} sum up to one.
An entry $\textbf{M}_{ij}$ in {\bf M} is the probability of random walk from column element {\it i} to row element {\it j}. 
The MCL algorithm is an iterative algorithm having two steps which are called {\it expansion} and {\it inflation}.

The {\it expansion} is the powers of matrix {\bf M} meaning the random walker does $\alpha$ jumps in each iteration {\it k}, 
\begin{eqnarray}
{\bf M_{\it k+1} =  M^{\alpha}_{\it k}}
\end{eqnarray}
and usually 2 is used as the value of $\alpha$ for the stability of the algorithm \cite{Wilschut2017}.
We also try other values of $\alpha$. When $\alpha = 1$, the clustering will diverge. When $\alpha=3$, the clustering will have less influence on the
clustering results.
The $\textbf{M}_{0}$ is the input of MCL matrix {\bf M}.
The {\it inflation} is the second step to distinguish the probability in {\bf M} after each expansion step, and consists of two procedures that
are determined respectively in following.

\begin{eqnarray}
{\bf (M_{\it k+1})_{\it ij} =(M_{\it k+1})^\beta_{\it ij}}
\end{eqnarray}
\begin{eqnarray}
{\bf (M_{\it k+1})_{\it ij} = \frac{  (M_{\it k+1})_{\it ij} } {\sum\limits_{\it i=1}^{\it N} (M_{\it k+1})_{\it ij}  }}
\end{eqnarray}

Namely, each elements $(\textbf{M}_{\it k+1})_{\it ij}$ to the power of $\beta$ and the columnwise normalization will be applied in the second. 
After the inflation step, high transition probabilities are increased and low transition probabilities are decreased .

Repeat the {\it expansion} and {\it inflation} and the matrix {\bf M} will eventually converge to a stable matrix. 
The number of clusters tend to become bigger if the power $\beta$ in {\it inflation} step is increased  because the difference between the elements in each column of the matrix gets amplified. In other words, the relatively weak connections between individual elements will tend to disappear when using larger $\beta$.
%各个cluster差距会拉得越大. 

%%%%

\subsection{The input of MCL}
\label{sec:input}
In this thesis, we apply the MCL to the approach in \cite{Feng2008} to automate the steps which need the insight of the system. 
To prepare the entry of MCL which is the stochastic square matrix {\bf M}, we using the following three steps which is originally from \cite{Goorden2020}.
\begin{description}
%%%%%%%%%%%%%%%DMM
\item[{\bf Step 1}] 
Consider a set of plant models $\textbf{G}$ and a set of specification models $\textbf{E}$. First generate a binary matrix ${\bf P}$ called Domain Mapping Matrix (DMM) \cite{DMM} to record the result that whether a plant and a specification have shared events.
${\bf P}({\it i,j})=1$ if specification {\it i} and plant {\it j} have shared events; otherwise ${\bf P}({\it i,j})=0$.

 %%%%%%%%%%%%DSM%%%%%%%%%
\item[{\bf Step 2}] 
Multiply ${\bf P}$ with its tranpose matrix ${\bf P^\top}$ to get a square matrix, 
called {\it Dependency Structure Matrice} (DSM)\cite{Steward1981DSM}\cite{Goorden2020}.
\begin{eqnarray}
{\bf P_{D}=P\times P^\top}
\end{eqnarray}
The number of rows in matrix DSM ${\bf P_D}$ represents the number of specification automata. When ${\bf P_D}(i,j)=k$ we know that there exist $k$ plant models that have shared events with both specification models $\textbf{E}_i$ and $\textbf{E}_j$.
%And the value of each element in ${\bf P_D}$ means the number of plant components each specification undertaking.
%%%%%%%%%%%%%column normalize
\item[{\bf Step 3}] 
Convert ${\bf P_D}$ into stochastic matrix $\textbf{M}$ by normalizing the columns of ${\bf P_D}$: 
\begin{eqnarray}
{\bf {M}_{\it ij} = \frac{  {P_{D}}_{\it ij} } {\sum\limits_{\it i} {{P_{D}}_{\it ij}  }}}
\end{eqnarray}

\end{description}

\begin{comment}


\subsection{Overlap}
The phenomenon of overlap described in Sec.10.2 of \cite{MCL} in the setting of undirected graphs has only been observed so far for input graphs with specific symmetry properties.
The overlapping part from which the graph looks the same in different directions.
In other words, the probability of a transition from an overlapping part to other elements in a different cluster to which it belongs is equal.
%
%
\begin{eqnarray}
\textbf{M}_x=\left(
    \begin{matrix}
        0.6 & 0.25 & 0.2\\
        0.2 & 0.5 & 0.2\\
        0.2 & 0.25 & 0.6
    \end{matrix}
\right)
\end{eqnarray}
%
Let a stochastic matrix $\textbf{M}_x$ be the input of MCL.
When we set {\it inflation} $\beta$ as 3, matrix $\textbf{M}_x$ converges to a stable matrix 
%
\begin{eqnarray}
\left(
\begin{matrix}
        1 & 0.5 & 0\\
        0 & 0 & 0\\
        0 & 0.5 & 1
    \end{matrix}
\right)
\end{eqnarray}
%
after the iterative calculation of MCL. Cluster $\{1,2\}$ and cluster $\{2,3\}$ have node $2$ at the same time. 
Figure 1 shows the cluster results where overlap exists. 
%
\begin{figure}[H]

	\centering
	\includegraphics[width=60mm]{fig/overlap.jpg}	
 	
  	\caption{Cluster $\{1,2\}$ and $\{2,3\}$ have overlap $\{2\}$\label{fig:2overlap}}
\end{figure}
%
From the perspective of node $2$, the probabilities of going to node $1$ and node $3$ are equal.
%
%在这篇文章中，遇到存在重复的情况时，我们会将重复部分分别单独分配给其中一个簇，从而消除重复。并将各自作为一个新的结果进行使用。
In this thesis, when we encounter the presence of overlaps, we eliminate the overlaps by assigning each of the overlaps to one of the clusters separately. Then each will be used as a new result. 
For example, we treat the cluster results in the Fig.\ref{fig:2overlap} in the following two cases 
$\{ \{1\},\{2,3\} \}$ and 
$\{ \{1,2\},\{3\} \}$.
%






\begin{eqnarray}
\textbf{P}_\textbf{D}=\left(
    \begin{matrix}
        3 & 1 & 1\\
        1 & 2 & 1\\
        1 & 1 & 3
    \end{matrix}
\right)
\end{eqnarray}



\end{comment}

==> tex/Chapter2_Preliminary_TDES.tex <==
\section{Timed Discrete-Event Systems}


%%%%%%%%%% ALL equations %%%%%
A finite-state automaton $\textbf{G}_{act}$ is the following five-tuple
%
\begin{align}
    \textbf{G}_{\textbf{act}} = (A, \Sigma_{act}, \delta_{act}, a_0, A_m)
\end{align}
%`'
except that the `state set' $Q$ in Sec.\ref{sec:pre_language} has been replaced with an finite $activity$ set $A$ whose elements are $activities$ $a$.
$\Sigma_{act}$ is a finite alphabet of events. 
The $\delta_{act}: A \times \Sigma_{act} \rightarrow A$ is the (partial) $activity$ $transition$ $function$.
$a_0$ is the $initial$ $activity$ and $A_m \subseteq A$ is the subset of $marker$ $activities$.

 Let $\mathbb{N}$ denote the natural numbers $\{0, 1, 2, \dots\}$. 
 In $\Sigma_{act}$, each transition $\sigma$ will be equipped with a $lower$ $time$ $bound$ $l_{\sigma}\in\mathbb{N}$ 
 and an $upper$ $time$ $bound$ $u_{\sigma}\in\mathbb{N}\cup\{\infty\}$. 
 To reflect two distinct possibilities of basic interest we partition $\Sigma_{act}$ according to
%
\begin{align}
    \Sigma_{act}=\Sigma_{spe} \ \dot{\cup}  \ \Sigma_{rem}
\end{align}
%
where `$spe$' denotes `prospective' and `$rem$' denotes `remote'. 
If an event $\sigma$ is prospective, its upper time bound $u_{\sigma}$ is finite 
$(0 \leq u_{\sigma} < \infty)$ and $0 \leq l_{\sigma} < u_{\sigma}$; 
while if $\sigma$ is remote, we set $u_{\sigma} = \infty$ and require $0 \leq l_{\sigma} < \infty$. 

The modeling function of time bounds is straightforward: 
$l_{\sigma}$ would typically represent a delay, in communication or in control enforcement; 
$u_{\sigma}$ a hard deadline, imposed by legal specification or physical necessity. The formal role of time bounds will be treated in detail below.
The triples $\sigma, l_{\sigma}, u_{\sigma}$ will be called $timed$ $events$, and for these we write
%
\begin{align}
    \Sigma_{tim} := \{ (\sigma, l_{\sigma}, u_{\sigma})|\sigma\in\Sigma_{act} \}
\end{align}
%
For $j,k \in \mathbb{N}$ write $[j,k]$ for the set of integers $i$ with $j \leq i \leq k$, and let $T_{\sigma}$ be the $timer$ $interval$ for $\sigma$ defined as follows:
%
\begin{align}
T_{\sigma}=\left\{
    \begin{array}{lll}
   \lbrack 0,u_{\sigma} \rbrack & \textrm{if} & \sigma\in\Sigma_{spe} \\
   \lbrack 0,l_{\sigma} \rbrack & \textrm{if} & \sigma\in\Sigma_{rem}
    \end{array}
    \right.
\end{align}
%
We can now define the $state$ $set$
%
%\begin{comment}
\begin{align}
Q := A \times \prod \{ T_{\sigma}|\sigma\in\Sigma_{act} \}
\end{align}
%
Thus a $state$ is an element of form
%
\begin{align}
q = ( a,\{ t_{\sigma}|\sigma\in\Sigma_{act} \} )
\end{align}
%
where $a \in A$ and $t_{\sigma} \in T_{\sigma}$; namely $q$ consists of an  activity $a$ together with a tuple assigning to each event $\sigma\in\Sigma_{act}$ an integer in its timer interval $T_{\sigma}$.
The component $t_{\sigma}$ of $q$ will be called the $timer$ of $\sigma$ in $q$.
If $\sigma\in\Sigma_{spe}$, the $current$ $deadline$ for $\sigma$ is $t_{\sigma}$, while the $current$ $delay$ is max$\{ t_{\sigma}+l_{\sigma}-u_{\sigma}, 0 \}$.
If $\sigma \in \Sigma_{rem}$, the $current$ $delay$ is $t_{\sigma}$.
The value $u_{\sigma}$ (resp. $l_{\sigma}$) for a prospective (resp. remote) event $\sigma$ will be called the $default$ $value$ of $t_{\sigma}$. The $initial$ $state$ is
%
\begin{align}
q_0 := ( a_0,\{ t_{\sigma 0}|\sigma\in\Sigma_{act} \} )
\end{align}
%
where the $t_{\sigma}$ are set to their default values
%
\begin{align}
t_{\sigma 0} := \left\{
    \begin{array}{lll}
   u_{\sigma} & \textrm{if} & \sigma\in\Sigma_{spe} \\
   l_{\sigma} & \textrm{if} & \sigma\in\Sigma_{rem}
    \end{array}
    \right.
\end{align}
%
The $marker$ $state$ $subset$ will be taken to be of the form
%
\begin{align}
Q_m \subseteq A_m \times \prod \{ T_{\sigma}|\sigma\in\Sigma_{act} \}
\end{align}
%
namely a marker state comprises a marker activity together with a suitable assignment of the timers.

We introduce one additional event, written $tick$, to represent `tick of the global
clock', and take for our total set of events
%
\begin{align}
\Sigma := \Sigma_{act} \dot{\cup}\{ tick \}
\end{align}
%
With the above definitions of state set $Q$, initial state $q_0$, marker state set $Q_m$ and event set $\Sigma$, we write 
%
\begin{align}
\textbf{G} = (Q, \Sigma, \delta, q_0, Q_m)
\end{align}
%
be a $timed$ $discrete$-$event$ $system$ (TDES).
%
The state transition function
$\delta : Q \times \Sigma \rightarrow Q$
for TDES is defined as follows. 
For any event $\sigma\in\Sigma$ and any state $q=(a, \{ t_{\tau} | \tau\in\Sigma_{act} \})\in Q$, 
we write $\delta(q, s)!$ to mean that $\delta(q, s)$ is defined if one of the following three conditions holds.
%

%
\begin{align}
q=(a, \{ t_{\tau} | \tau\in\Sigma_{act} \}),  q' = (a', \{  t'_{\tau} |\tau\in\Sigma_{act} \})
\end{align}
%

\begin{enumerate}[(i)]
  \setlength{\parskip}{0cm} % 段落間
  \setlength{\itemsep}{0cm} % 項目間
  %
    \item $ \sigma = tick \ \textrm{and} \ (\forall\tau\in\Sigma_{ape})
    \delta_{act}(a,\tau)!\Rightarrow t_{\tau} > 0; \textrm{or}$
    %
    \item $ \sigma\in\Sigma_{spe},\delta_{act}(a,\sigma)!,
    \textrm{and} \ 0\leq t_{\sigma}\leq u_{\sigma} - l_{\sigma};\textrm{or} $
    %
    \item $ \sigma\in\Sigma_{rem},\delta_{act}(a,\sigma)!,
    \textrm{and} \ t_{\sigma}=0 $ 
\end{enumerate}
%
When $\delta(q, s)$ is defined, let $\delta(q, s) = q'$ and $q' = (a', \{  t'_{\tau}|\tau\in\Sigma_{act} \})$. The definition of state $q'$ is the following.

%%%%%%%%%% DEF of q' START%%%%%
\begin{enumerate}[(i)]

\item Let $\sigma = tick$. Then $a' := a$. For all $\tau\in\Sigma_{act}$,\\
if $\tau\in\Sigma_{spe}$,
\begin{align}
t'_{\tau}:= \left\{
    \begin{array}{ll}
     u_{\tau}    & \textrm{if} \ not \ \delta_{act}(a,\tau)! \\
     t_{\tau}-1  & \textrm{if} \ \delta_{act}(a,\tau)! \ \textrm{and} \ t_{\tau}>0
    \end{array}
    \right.
\end{align}
%

if $\tau\in\Sigma_{rem}$,
%
\begin{align}
t'_{\tau}:= \left\{
    \begin{array}{ll}
     l_{\tau}    & \textrm{if} \ not \ \delta_{act}(a,\tau)! \\
     t_{\tau}-1  & \textrm{if} \ \delta_{act}(a,\tau)! \ \textrm{and} \ t_{\tau}>0 \\
     0           & \textrm{if} \ \delta_{act}(a,\tau)! \ \textrm{and} \ t_{\tau}=0
    \end{array}
    \right.
\end{align}
%
\item Let $\sigma = \sigma$. Then $a' := \delta_{act}(\sigma , a)$. For all $\tau\in\Sigma_{act}$,\\
%
if $\tau \neq \sigma$ and $\tau\in\Sigma_{spe}$,
\begin{align}
t'_{\tau}:= \left\{
    \begin{array}{ll}
     u_{\tau}  & \textrm{if} \ not \ \delta_{act}(a',\tau)! \\
     t_{\tau}  & \textrm{if} \ \delta_{act}(a',\tau)! 
    \end{array}
    \right.
\end{align}
%
if $\tau = \sigma$ and $\tau\in\Sigma_{spe}$,
%
\begin{align}
t'_{\tau}:= u_{\sigma}
\end{align}
%
if $\tau \neq \sigma$ and $\tau\in\Sigma_{rem}$,
%
\begin{align}
t'_{\tau}:= \left\{
    \begin{array}{ll}
     l_{\tau}  & \textrm{if} \ not \ \delta_{act}(a',\tau)! \\
     t_{\tau}  & \textrm{if} \ \delta_{act}(a',\tau)! 
    \end{array}
    \right.
\end{align}
%
if $\tau = \sigma$ and $\tau\in\Sigma_{rem}$,
%
\begin{align}
t'_{\tau}:= l_{\sigma}
\end{align}
%
\end{enumerate}
%%%%%%%%%% DEF of q' end %%%%%




\subsection{Composition for TDES}
Let $\textbf{G}_1$, $\textbf{G}_2$ be TDES over alphabets $\Sigma_1$, $\Sigma_2$ respectively, where $\Sigma_i = \Sigma_{i,act} \cup \{tick\}$. In general $\Sigma_{1,act}$, $\Sigma_{2,act}$ need not be disjoint. 
To form the $composition$ $\textbf{G}= \textbf{comp}(\textbf{G}_1,\textbf{G}_2)$ we start by defining the alphabet of $\textbf{G}$ as $\Sigma_1 \cup \Sigma_2$,
and the activity transition structure of $\textbf{G}$ as the synchronous product of the component activity structures $\textbf{G}_{\textbf{act}}=\textbf{G}_{\textbf{1,act}} || \textbf{G}_{\textbf{2,act}}$. 
The time bounds $(l_\sigma, u_\sigma)$ in $\textbf{G}$ of an event
%
\begin{align}
\sigma\in(\Sigma_{1,act}-\Sigma_{2,act})\cup(\Sigma_{2,act}-\Sigma_{1,act})
\end{align}
%
remain unchanged from their definition in the corresponding component structure,
while if $\sigma\in\Sigma_{1,act}\cap\Sigma_{2,act}$
then its time bounds in $\textbf{G}$ are defined in obvious notation to be
%
\begin{align}
(l_{\sigma}, u_{\sigma}) = (\textrm{max}\{ l_{1,\sigma}, l_{2,\sigma} \}, \textrm{min}\{ u_{1,\sigma}, u_{2,\sigma} \})
\end{align}
%
provided $l_{\sigma} \leq u_{\sigma} $.

%
%\begin{align}

%\end{align}
%

%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Forcible Event and Controllability}
Let TDES \textbf{G} model the plant in to be controlled.
The event set $\Sigma_{act}$ of \textbf{G} is partitioned into a subset $\Sigma_c$ of \textsl{controllable} events and a subset $\Sigma_u$ of \textsl{uncontrollable} events.
In TDES, the controllable events are assumed to be limited to those whose occurrence can be infinitely delayed by prohibition, i.e. $\Sigma_c\subseteq\Sigma_{rem}$. 
We also consider a subset of events called the $forcible$ events, written $\Sigma_{for}$. 
By introducing these forcible events, it is possible to express control over the event $tick$ that represents the passage of time. Suppose that in state $q\in Q$, a forcible event and $tick$ can occur. 
Then, by forcing the occurrence of the forcible event, it is possible to interpret $tick$ as being preempted. 
Therefore, $tick$ is an event that can be preempted only when a forcible event can occur.

For controllability, define for each string $s \in \Sigma^{\ast}$ a subset of eligible events for TDES \textbf{G},  $\textrm{Elig}_{\textbf{G}}(s)\subseteq \Sigma$ ($ \Sigma_{act}\cup \{tick\} = \Sigma$), as follows
%
\[
\textrm{Elig}_{\textbf{G}}(s):=\{ \sigma \in \Sigma | s\sigma\in L(\textbf{G}) \}
\]
%
Let $K\subseteq L(\textbf{G})$ be arbitrary, and write
%
\begin{align}
\textrm{Elig}_{K}(s):=\{ \sigma \in \Sigma | s\sigma\in \overline{K} \}, s\in\Sigma^{\ast}
\end{align}
%
We define $K$ to be $controllable$ ($respect$ $to$ $\textbf{G}$) if, for all $s\in \Sigma^{\ast}$,
\begin{align}
\textrm{Elig}_{K}(s)\supseteq\left\{
    \begin{array}{lll}
    %
    \textrm{Elig}_{\textbf{G}}(s) \cap (\Sigma_{u}\cup\{tick\}) & \textrm{if} & \textrm{Elig}_{K}(s) \cap \Sigma_{for} = \varnothing\\
    %
    \textrm{Elig}_{\textbf{G}}(s) \cap \Sigma_{u} & \textrm{if} & \textrm{Elig}_{K}(s) \cap \Sigma_{for} \neq \varnothing
    %
    \end{array}
\right.
\end{align}
Thus $K$ controllable means that an event $\sigma$ may occur in $K$ if $\sigma$ is currently eligible in $\textbf{G}$ and either (i) $\sigma$ is uncontrollable, or (ii) $\sigma =
tick$ and no forcible event is currently eligible in $K$.
 As in the usual supervisory control we introduced in Sec.\ref{sec:centr_sup}.
 Define a \textsl{supervisory control} $S$ for \textbf{G} is any map $S:L(\textbf{G}) \rightarrow \Gamma$.
 Let $K \subseteq L_m(\textbf{G})$, $K \neq \varnothing$. There exists a nonblocking supervisory control $S$ for $\textbf{G}$ such that $L_m(S/\textbf{G})=K$ if and only if $K$ is controllable with respect to $\textbf{G}$.
 
 
\begin{comment}

For any state A and any string B, to ensure that the unrealistic behavior of an event occurring infinitely many times in one unit of time does not occur in system G.
This condition implies that there is no loop in G such that it does not contain A.
\end{comment}

==> tex/Chapter3_Medthod.tex <==

\chapter{Algorithmic Approach for Heterarchical Supervisor Synthesis }
\label{chap:method}
Our proposed architectural approach to the heterarchical supervisory control design is the following six steps.

%%数学化


%%
\begin{enumerate}
\item Modeling the system to get all plant components $\textbf{G}_1,...,\textbf{G}_J$ and specification automata $\textbf{E}_1,...,\textbf{E}_I (J,I\in\mathbb{N}^+)$ and synthesize decentralized supervisors $\textbf{SUP}_1,...,\textbf{SUP}_I$ to enforce each of specifications. 
The event set of each plant component $\textbf{G}_j (j\in \{1, \ldots,J \})$ and specification $\textbf{E}_i (i\in \{1,\ldots, I \})$ is written $\Sigma_{\textbf{G}_j}$ and $\Sigma_{\textbf{E}_i}$, respectively.  The decentralized plant $\textbf{G}_{\textbf{E}_i}$ is the synchronous product of the plant components that share events with $\Sigma_{\textbf{E}_i}$, written
$\textbf{G}_{\textbf{E}_i} := ||\{\textbf{G}_j | \Sigma_{\textbf{G}_j} \cap \Sigma_{{\textbf{E}_i}} \neq\emptyset\}$. 
Then we synthesize an optimal and nonblocking {\it decentralized} {\it supervisor} $\textbf{SUP}_i : L_m({\bf SUP}_i)=\textrm{sup}\textit{C}(L_m(\textbf{E}_i)||L_m(\textbf{G}_{\textbf{E}_i})) $. 

%step2
\item Before the clustering, we construct the input of the MCL algorithm by computing the stochastic square matrix {\bf M}. 
First we produce a binary matrix {\bf P}: ${\bf P}({\it i,j})=1$ if the event set $\Sigma_{\textbf{SUP}_{i}}$ of decentralized supervisor $\textbf{SUP}_i$ and the event set $\Sigma_{\textbf{G}_{j}}$ of plant component $\textbf{G}_j$ are not disjoint; otherwise ${\bf P}({\it i,j})=0$. 
Then we multiply {\bf P} with its transpose matrix ${\bf P^\top}$ to get a square matrix: ${\bf P_{D}=P\times P^\top}$. 
Finally we convert ${\bf P_D}$ into stochastic matrix $\textbf{M}$ by normalizing the columns of ${\bf P_D}$.
Setting the {\it expansion} parameter $\alpha$ to 2 and the {\it inflation} parameter $\beta$ can be adjusted to get different clustering results.
We apply the MCL algorithm to design the modular subsystems by partitioning the decentralized supervisors into clusters.   

%step3
\item    
After the clustering process, we get $N$ clusters $\{1,\ldots,N\}$.
Let $\mathcal{X}_n$ $(n\in\{1,\ldots,N\})$ be a set of indices of the decentralized supervisors  in cluster $n$.
The subsystem $\textbf{SUB}_n$ is the synchronous product of all decentralized supervisors in the same cluster, i.e.
\begin{eqnarray}
\textbf{SUB}_{n} = ||\{\textbf{SUP}_i|i\in \mathcal{X}_n\}
%\textit{CLS}_m =  \{ i | i\in I \cap  \textit{CLS}_m \}\\
%(n,m\in N; n\neq m) \ CLS_n \cap CLS_m = \varnothing	
\end{eqnarray}
%
%We synthesize a subsystem $\textbf{SUB}_n \{1,\ldots,N\}$ for each cluster so we get $N$ subsystems $\textbf{SUB}_{1},...,\textbf{SUB}_{N}$, written $\textbf{SUB}_{n} = ||(\textbf{SUP}_i|i\in CLS_n)$. 
%
Check if blocking exists in the subsystem $\textbf{SUB}_n$. If so, a supervisor called {\it coordinator} $\textbf{CO}_n$ \cite{Feng2008} will be designed to remove the blocking states.
This $\textbf{CO}_n$ is constructed in two steps.
First we compute
$L_m({\bf CO}_n) := {\rm sup} {\it C}( L_m( {\bf SUB}_n)|| \Sigma_{\textbf{SUB}_n}^{\ast} )$. 
Then apply supervisor reduction \cite{SUPLOC} to reduce the state size of $\textbf{CO}_n$,
by projecting out the structural constraints of $L_m( {\bf SUB}_n)$ and leaving merely the `backbone' of the blocking-removal control action.
Then the nonblocking subsystem is $\textbf{SUB}_n=||_{i\in \mathcal{X}_n}(\textbf{SUP}_i)||\textbf{CO}_{n}$.

%step4
\item We use the model abstraction method \cite{Feng2008,SUPLOC} to create a smaller model for each subsystem $\textbf{SUB}_n$ called {\it abstraction} $\textbf{ABS}_n$. 
Let $\Sigma_{\textbf{SUB}_n}$ be the event set of $\textbf{SUB}_n$,
and $\Sigma_{\textbf{ABS}_n}\subseteq\Sigma_{\textbf{SUB}_n}$ the event set of $\textbf{ABS}_n$.
To obtain this $\Sigma_{\textbf{ABS}_n}$, we first determine the shared event set $\Sigma_o$ of the subsystems, i.e.
\[
\Sigma_o := \{ \sigma\in\Sigma | (\exists n_1,n_2 \in\{1,\dots,N\}) \
n_1\neq n_2 \ \& \  \sigma \in \Sigma_{\textbf{SUB}_{n_1}}\cap \Sigma_{\textbf{SUB}_{n_2}}  \}.
\]
Then let $\Sigma_{\textbf{ABS}_n} := \Sigma_o \cap \Sigma_{\textbf{SUB}_n}$.
Each $\textbf{ABS}_n$ is generated by a natural projection $\textit{P}_n : \Sigma^{\ast}_{\textbf{SUB}_n} \rightarrow \Sigma^{\ast}_{\textbf{ABS}_n} $. 
The event set $\Sigma_{\textbf{ABS}_n}$ is extended to make
$\textit{P}_n$ satisfy both natural observer and OCC properties.

%step5
\item After step 4, we have $N$ abstractions $\textbf{ABS}_1,...,\textbf{ABS}_N$. 
Repeat the step 2 to step 4 until there are less than or equal 2 clusters. 
Note that if the result of clustering remains the same as before, namely if the number of clusters is not reduced compared to the previous clustering, we will reduce the inflation value $\beta$ introduced in Sec.\ref{main_MCL}.
%
In addition, from the second-time of applying clustering, we partition the set of abstractions (rather than the set of decentralized supervisors as in the first time). 
Hence the binary matrix {\bf P} is constructed such that ${\bf P}({\it n,j})=1$ if the event set $\Sigma_{\textbf{ABS}_{n}}$ of abstraction $\textbf{ABS}_{n}$ and the event set $\Sigma_{\textbf{G}_{j}}$ of plant component $\textbf{G}_j$ are not disjoint; otherwise ${\bf P}({\it n,j})=0$. 
%
\item Check if conflicts exist among the abstractions in the top-level cluster(s).
If so, design a coordinator to ensure the nonblockingness. 

\end{enumerate}

\begin{comment}
From this processing, the input of MCL will be changed from the construction of matrix {\bf P}. The abstractions $\textbf{SUP}_1,...,\textbf{SUP}_I$ in {\bf P} will be replaced into abstractions $\textbf{ABS}_1,...,\textbf{ABS}_N$ which is created in former processing. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Namely ${\bf P}({\it n,j})=1$ if the event set $\Sigma_{o,n}$ of abstraction $\textbf{ABS}_n$ and the event set $\Sigma_{\textbf{G}_j}$ of plant component $\textbf{G}_j$ are not disjoint; otherwise ${\bf P}({\it n,j})=0$.

\end{comment}



==> tex/Chapter3_proof.tex <==
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem*{thm*}{Theorem}
\newtheorem{prop}{Proposition}
\theoremstyle{definition}
\newtheorem{dfn}{Definition}
%%%%proof:
Using the above procedure, we obtain $I$ decentralized supervisors 
$\textbf{SUP}_1,...,\textbf{SUP}_I$ and $H$  coordinators ${\bf CO}_1, \ldots, {\bf CO}_H$ (the number of coordinators is case-dependent). 
We conclude that the synchronized behavior of these supervisors and coordinators is identical to the behavior of the monolithic supervisor \textbf{SUP}.
%%%%%
%Your theorem statement is wrong. You only considered Natural observer and OCC for SUB. You are right if there is only one-level up in the hierarchy. Namely if you do clustering only once. But in general you need to do clustering many times to produce multi-level abstractions. So Natural Observer and OCC properties must hold for all ABS in all levels.
%%%5

\begin{thm}\label{thm1}

Suppose that the proposed procedure terminates after $L (\geq 1)$ levels of clustering/abstraction, and in each level $l \in \{1,\ldots,L\}$ there are $N_l$ clusters ${\bf SUB}_{n_l}$ ($n_l \in \{1,\ldots,N_l\}$). Assume that the procedure generates $I$ decentralized supervisors ${\bf SUP}_i$ $(i \in \{1, \ldots, I\})$ and $H$ coordinators ${\bf CO}_h$ $(h \in \{1, \ldots, H\})$. If for every $l \in \{1,\ldots,L\}, n_l \in \{1,\ldots,N_l\}$, $P_{n_l}$ is an $L_m({\bf SUB}_{n_l})$-observer and OCC for $L_m({\bf SUB}_{n_l})$, then


\begin{eqnarray}
%||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))= 
%\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}\\
%(||_{i\in I} \textbf{SUP}_i)|| (||_{w\in W}\textbf{CO}_w)=\textbf{SUP}
(||_{i \in \{1, \ldots, I\}} L(\textbf{SUP}_i)) || (||_{h \in \{1, \ldots, H\}}L(\textbf{CO}_h)) || L(\textbf{G})=L(\textbf{SUP})\\
(||_{i \in \{1, \ldots, I\}} L_m(\textbf{SUP}_i)) || (||_{h \in \{1, \ldots, H\}}L_m(\textbf{CO}_h)) || L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\end{thm}




%有w层，经过几次抽象化以后的CO，也能去除底层DESUP的冲突。NATOB和OCC的连锁性？

Theorem \ref{thm1} asserts that decentralized supervisors and coordinators designed using our proposed method jointly achieve global optimal and nonblocking controlled behavior. 
%%%开始证明
%
%%
To prove Theorem \ref{thm1}, we need the following proposition from \cite{Feng2008}:
%sub先定义，然后证明我们的sub里面就是sup的组合，sup组合的话已经被证明
\begin{prop}[\cite{Feng2008}]\label{prop1}
Consider $I$ decentralized supervisors $\textbf{SUP}_i$ $(i \in \{1, \ldots, I\})$  and $H$ coordinators ${\bf CO}_h$ $(h \in \{1, \ldots, H\})$  based on abstractions. If for every $i $, 
$P_i$ is an $L_m(\textbf{SUP}_i)$-observer and OCC for $L_m(\textbf{SUP}_i)$, then
\footnotesize
\begin{eqnarray}
(||_{i \in \{1, \ldots, I\}} L(\textbf{SUP}_i)) ||(||_{h \in \{1, \ldots, H\}}L(\textbf{CO}_h))= 
\overline{(||{}_{i \in \{1, \ldots, I\}}L_m(\textbf{SUP}_i))||(||_{h \in \{1, \ldots, H\}}L_m(\textbf{CO}_h))}\\
(||_{i \in \{1, \ldots, I\}} L(\textbf{SUP}_i)) ||(||_{h \in \{1, \ldots, H\}}L(\textbf{CO}_h))||L(\textbf{G})=L(\textbf{SUP})\\
(||_{i \in \{1, \ldots, I\}} L_m(\textbf{SUP}_i)) ||(||_{h \in \{1, \ldots, H\}}L_m(\textbf{CO}_h))||L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\normalsize
\end{prop}
%$\textbf{SUB}_{n} = ||(\textbf{SUP}_i|i\in CLS_n)$ and\\
%
%By Proposition \ref{prop1}, we can easily say that T coordinators $\textbf{CO}_t (t\in T)$ based on subsystems' abstractions also can make remove conflicts in the joint behavior of subsystems, which is shown following.
%
%主要是经过step2之后我们还是可以保证nonblocking
%我们cluster组合后不会忽视supi
%各个cluster好好地被observer和occ
\begin{proof}[Proof of Theorem 1]

Consider a system with $I$ specification models. After step 2, $I$ decentralized supervisors $\textbf{SUP}_1,...,\textbf{SUP}_I$ are partitioned into $N_1$ clusters.
In this level 1,
let $\mathcal{X}_{n_1}$ $(n_1\in \{1, \dots, N_1\})$ be a set of indices of the decentralized supervisors in cluster $n_1$.
Each cluster will form by synchronous product a subsystem $\textbf{SUB}_{n_1}$ 
$(n_1\in \{1, \dots, N_1\})$, written $\textbf{SUB}_{n_1} = ||\{\textbf{SUP}_i|i\in \mathcal{X}_{n_1}\}$.
The subsystem 
$\textbf{SUB}_{n_1} = (||_{i\in \mathcal{X}_{n_1}}(\textbf{SUP}_i))||{\bf CO}_{n_1}$ as in step 3 is nonblocking, namely
%
%
\begin{eqnarray}
(||_{i\in \mathcal{X}_{n_1}}L(\textbf{SUP}_i))||L(\textbf{CO}_{n_1})
=\overline{(||_{i\in \mathcal{X}_{n_1}}L_m(\textbf{SUP}_i))||L_m(\textbf{CO}_{n_1})}
\end{eqnarray}
%
In this level 1, each abstraction $\textbf{ABS}_{n_1}$ $(n_1\in \{1,\dots,N_1\})$ as in step 4 is obtained by natural projection $\textit{P}_{n_1}$ from $\textbf{SUB}_{n_1} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{n_1})=\textit{P}_{n_1} L(\textbf{SUB}_{n_1}), L_m(\textbf{ABS}_{n_1})=\textit{P}_{n_1} L_m(\textbf{SUB}_{n_1})
\end{eqnarray}
%
and the projection $P_{n_1}$ in step 4 is an $L_m(\textbf{SUB}_{n_1})$-observer and OCC for $L_m(\textbf{SUB}_{n_1})$.

When the number of clusters is greater than two, we do further clustering of abstractions $\textbf{ABS}_{1},\dots,\textbf{ABS}_{N_1}$. 
After second level clustering, consider that we get $N_2$ clusters and 
let $\mathcal{X}_{n_2}$ $(n_2\in \{1, \dots, N_2\})$ be a set of indices of the abstractions in cluster $n_2$.
Each cluster will form by synchronous product a subsystem $\textbf{SUB}_{n_2}$ $(n_2\in \{1, \dots, N_2\})$, written $\textbf{SUB}_{n_2} = ||\{\textbf{ABS}_{n_1} | n_1\in \mathcal{X}_{n_2}\}$.
The subsystem 
\[\textbf{SUB}_{n_2} = 
(||_{n_1\in \mathcal{X}_{n_2}}(\textbf{ABS}_{n_1}))||{\bf CO}_{n_2} \
\]as in step 3 is nonblocking, namely
%
%
\begin{eqnarray}
(||_{n_1\in \mathcal{X}_{n_2}}L(\textbf{ABS}_{n_1}))||L(\textbf{CO}_{n_2})
=\overline{(||_{n_1\in \mathcal{X}_{n_2}}L_m(\textbf{ABS}_{n_1}))||L_m(\textbf{CO}_{n_2})}
\end{eqnarray}
%
By Proposition \ref{prop1}, the coordinator $\textbf{CO}_{n_2}$  based on abstractions $\{\textbf{ABS}_{n_1}|n_1\in \mathcal{X}_{n_2}\}$ removes the conflicts among subsystems $\{\textbf{SUB}_{n_1}|n_1\in \mathcal{X}_{n_2}\}$ : 
%
\begin{eqnarray}
(||_{n_1\in \mathcal{X}_{n_2}}L(\textbf{SUB}_{n_1}))||L(\textbf{CO}_{n_2})
=\overline{(||_{n_1\in \mathcal{X}_{n_2}}L_m(\textbf{SUB}_{n_1}))||L_m(\textbf{CO}_{n_2})}
\end{eqnarray}
%
In this level $2$, each abstraction $\textbf{ABS}_{n_2}$ $(n_2\in \{1, \dots, N_2\})$ as in step 4 is obtained by natural projection $\textit{P}_{n_2}$ from $\textbf{SUB}_{n_2} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{n_2})=\textit{P}_{n_2} L(\textbf{SUB}_{n_2}), L_m(\textbf{ABS}_{n_2})=\textit{P}_{n_2} L_m(\textbf{SUB}_{n_2})
\end{eqnarray}
%
and the projection $P_{n_2}$ in step 4 is an $L_m(\textbf{SUB}_{n_2})$-observer and
OCC for $L_m(\textbf{SUB}_{n_2})$.

Consider that the procedure ends with clustering $L (\geq 1)$ times to produce $L$ levels abstractions.  In the top level $L$, let $\mathcal{X}_{n_L}$ $(n_L\in \{1, \dots, N_L\})$ be a set of indices of the abstractions in cluster $n_L$. Here $N_L \leq 2$.
Each cluster will form by synchronous product a subsystem $\textbf{SUB}_{n_L}$ $(n_L\in \{1, \dots, N_L\})$, written $\textbf{SUB}_{n_L} = ||\{ \textbf{ABS}_{n_{(L-1)}} | n_{(L-1)}\in \mathcal{X}_{n_L} \}$.
%
The subsystem 
\[
\textbf{SUB}_{n_L} = (||_{n_{(L-1)}\in \mathcal{X}_{n_L}}(\textbf{ABS}_{n_{(L-1)}}))||{\bf CO}_{n_L}
\]
as in step 3 is nonblocking, namely
%
%
%
\footnotesize
\begin{eqnarray}
(||_{n_{(L-1)} \in \mathcal{X}_{n_L}}L(\textbf{ABS}_{n_{(L-1)}}))||L(\textbf{CO}_{n_L})
=\overline{(||_{n_{(L-1)} \in \mathcal{X}_{n_L}}L_m(\textbf{ABS}_{n_{(L-1)}}))||L_m(\textbf{CO}_{n_L})}
\end{eqnarray}
%
\normalsize
%
Since the natural projection $\textit{P}_{n_{(L-1)}}$ from $\textbf{SUB}_{n_{(L-1)}} $:
%
\footnotesize
\begin{eqnarray}
L(\textbf{ABS}_{n_{(L-1)}})=\textit{P}_{n_{(L-1)}} L(\textbf{SUB}_{n_{(L-1)}}),
L_m(\textbf{ABS}_{n_{(L-1)}})=\textit{P}_{n_{(L-1)}} L_m(\textbf{SUB}_{n_{(L-1)}})
\end{eqnarray}
\normalsize
%
is an $L_m(\textbf{SUB}_{n_{(L-1)}})$-observer and OCC for $L_m(\textbf{SUB}_{n_{(L-1)}})$. 
The coordinator $\textbf{CO}_{n_L}$  based on abstractions $\{\textbf{ABS}_{n_{(L-1)}} | n_{(L-1)}\in \mathcal{X}_{n_L}\}$ removes the conflicts among subsystems $\{\textbf{SUB}_{n_{(L-1)}} | n_{(L-1)}\in \mathcal{X}_{n_L}\}$ : 
%
\footnotesize
\begin{eqnarray}
(||_{n_{(L-1)}\in \mathcal{X}_{n_L}}L(\textbf{SUB}_{n_{(L-1)}}))||L(\textbf{CO}_{n_L})
=\overline{(||_{n_{(L-1)}\in \mathcal{X}_{n_L}}
L_m(\textbf{SUB}_{n_{(L-1)}}))||L_m(\textbf{CO}_{n_L})}
\end{eqnarray}
\normalsize
%
In this level $L$, each abstraction $\textbf{ABS}_{n_L}$ $(n_L \in \{1,\dots, N_L\})$ as in step 4 are obtained by natural projection $\textit{P}_{n_L}$ from $\textbf{SUB}_{n_L} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{n_L})=\textit{P}_{n_L} L(\textbf{SUB}_{n_L}), L_m(\textbf{ABS}_{n_L})=\textit{P}_{n_L} L_m(\textbf{SUB}_{n_L})
\end{eqnarray}
%
and the projection $P_{n_L}$ in step 4 is an $L_m(\textbf{SUB}_{n_L})$-observer and
OCC for $L_m(\textbf{SUB}_{n_L})$.
Now by Proposition \ref{prop1}, we derive that the designed coordinator $ \textbf{CO}$ based on abstractions $\textbf{ABS}_1 , \dots, \textbf{ABS}_{N_L}$ also removes the conflicts among subsystems $\textbf{SUB}_1 ,\dots, \textbf{SUB}_{N_L}$: 





%\footnotesize
%\begin{eqnarray}
%(||_{n\in N} L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(||_{t\in T}L_m(\textbf{CO})})
%\end{eqnarray}
%\normalsize
%

%
\footnotesize
\begin{eqnarray}
(||_{n_L\in \{1,\dots,N_L\}} L(\textbf{SUB}_{n_L}))||L(\textbf{CO})
=\overline{(||_{n_L\in \{1,\dots,N_L\}}L_m(\textbf{SUB}_{n_L}))||L_m(\textbf{CO})}
\end{eqnarray}
\normalsize
%

Since in each level $l \in \{1,\ldots,L\}$ natural projection satisfies $L_m(\textbf{SUB}_{n_l})$-observer and OCC for $L_m(\textbf{SUB}_{n_l})$, removing each subsystem's internal conflict is equivalent to removing the conflict among subsystems at a lower layer contained in this subsystem before it was abstracted.
Therefore, the conflicts among all decentralized supervisors $\textbf{SUP}_1,\dots,\textbf{SUP}_I$ at the bottom layer are also removed by all coordinators $\textbf{CO}_1, \dots, \textbf{CO}_H$:
%
\footnotesize
\begin{eqnarray}
(||_{i \in \{1, \ldots, I\}} L(\textbf{SUP}_i)) || (||_{h \in \{1, \ldots, H\}}L(\textbf{CO}_h)) =
\overline{(||_{i \in \{1, \ldots, I\}} L(\textbf{SUP}_i)) || (||_{h \in \{1, \ldots, H\}}L(\textbf{CO}_h))}
\end{eqnarray}
\normalsize
%
This completes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%Trash%%%%%%%%%%%%%%%%%%%
\begin{comment}

\begin{thm}\label{thm1}
Consider decentralized supervisors $\textbf{SUP}_i(i\in I)$ as in step 1, subsystems $\textbf{SUB}_n(n\in N)$ as in step 3 and coordinator $\textbf{CO}_w(w\in W)$ as in step 3 and step 6 based on subsystem's abstractions. If for every $n \in N$, 
$P_n$ is an $L_m(\textbf{SUB}_n)$-observer and OCC for $L_m(\textbf{SUB}_n)$, then
\footnotesize
\begin{eqnarray}
%||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))= 
%\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}\\
%(||_{i\in I} \textbf{SUP}_i)|| (||_{w\in W}\textbf{CO}_w)=\textbf{SUP}
||_{i\in I} L(\textbf{SUP}_i) ||_{w\in W}L(\textbf{CO}_w)||L(\textbf{G})=L(\textbf{SUP})\\
||_{i\in I} L_m(\textbf{SUP}_i) ||_{w\in W}L_m(\textbf{CO}_w)||L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\normalsize
\end{thm}

The clustering only does partitioning and does not delete any element ($\textbf{SUP}_i$). Therefore, the synthesis of all clusters equals the synthesis of all decentralized supervisors:
%
\footnotesize
\begin{eqnarray}
||_{n\in N}L(\textbf{SUB}_{n})=
(||_{i \in I}L(\textbf{SUP}_{i}))||(||_{h \in H}L(\textbf{CO}_{h}))
\end{eqnarray}
\normalsize
%
Let $W (w\in W)$ be the new indexs of all coordinators, 
the equation $(30)$ becomes:

%
%\footnotesize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(L(\textbf{CO}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(L_m(\textbf{CO}))}\\
%=\overline{(||_{n\in N}(||_{i\in CLS_n}L_m(\textbf{SUP}_i)||L_m(\textbf{CO}_{h})))||(L_m(\textbf{CO}))}\\
%(||_{n\in N}\textbf{SUB}_{n})||(||_{h\in H}L(\textbf{CO}_h)) = (||_{i\in I} L(\textbf{SUP}_i)) ||(||_{h\in H}L(\textbf{CO}_h))
%\end{eqnarray*}
%\normalsize
%



%
%\footnotesize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}_{t}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(||_{t\in T}L_m(\textbf{CO}_{t}))}\\
%=\overline{(||_{n\in N}(||_{i\in CLS_n}L_m(\textbf{SUP}_i)||L_m(\textbf{CO}_{h})))||(||_{t\in T}L_m(\textbf{CO}_{t}))}\\
%(||_{n\in N}\textbf{SUB}_{n})||(||_{h\in H}L(\textbf{CO}_h)) = (||_{i\in I} L(\textbf{SUP}_i)) ||(||_{h\in H}L(\textbf{CO}_h))
%\end{eqnarray*}
%\normalsize
%

%\scriptsize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}_{t}))=
%(||_{i\in I} L(\textbf{SUP}_i))||(||_{h\in H}L(\textbf{CO}_h))||(||_{t\in T}L(\textbf{CO}_{t}))\\
%=\overline{(||_{i\in I} L_m(\textbf{SUP}_i))||(||_{h\in H}L_m(\textbf{CO}_h))(||_{t\in T}L_m(\textbf{CO}_{t}))}
%\end{eqnarray*}
%\normalsize
%
%Since $h\in H$ and $t\in T$ only are the indexs of coordinators, we put $W=H+T$ and relabel each of coordinators by $w, w\in W$.
%
\footnotesize
\begin{eqnarray*}
%(||_{i\in I} L(\textbf{SUP}_i))||(||_{h\in H}L(\textbf{CO}_h))||(||_{t\in T}L(\textbf{CO}_{t}))
%=||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))\\
||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))
=\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}
\end{eqnarray*}
\normalsize
%
Therefore, the synchronized behavior of $I$ decentralized supervisors $\textbf{SUP}_i$ and $W$ coordinators $\textbf{CO}_w$ is nonblocking. Since coordinator only remove the conflicts that proven in \cite{Feng2008},
\footnotesize
\begin{eqnarray*}
||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))=L(\textbf{SUP})\\
||_{i\in I} L_m(\textbf{SUP}_i) || (||_{w\in W}L_m(\textbf{CO}_w))=L_m(\textbf{SUP})
\end{eqnarray*}
\normalsize

When the number of clusters in this level 1 is not greater than two, namely $N\leq 2$, we do not do any further clustering of abstractions. By Proposition \ref{prop1}, we can say that the coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{n_1}$ also can remove the conflicts among subsystems $\textbf{SUB}_{n_1}$ : 
%
\begin{eqnarray}
(||_{n\in N} L(\textbf{SUB}_{n_1}))||_{h\in H}(L(\textbf{CO}_h))
=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n_1}))||_{h\in H}(L_m(\textbf{CO}_h)})
\end{eqnarray}
%

Consider $I$ decentralized supervisors $\textbf{SUP}_i \{i\in I,I\in\mathbb{N}^+\}$ as in step 1.
After $L\{L\in\mathbb{N}^+\}$ levels clustering and abstraction, in each level $l\in L$, consider there are $N$ subsystems $\textbf{SUB}_{n_L}\{n\in N,N\in\mathbb{N}^+\}$ as in step 3 based on subsystem's abstractions.
$H$ coordinators $\textbf{CO}_h\{h\in H,H\in\mathbb{N}^+\}$ as in step 3 and step 6 be designed to remove conflicts of subsystems.
If for every $l \in L$, $n \in N$, 
$P_{n_L}$ is an $L_m(\textbf{SUB}_{n_L})$-observer and OCC for $L_m(\textbf{SUB}_{n_L})$, then

If the number of clusters in this level $L$ is not greater than two, 
namely $N\leq 2$, we do not do any further clustering of abstractions. By Proposition \ref{prop1}, we can also say that the coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{n_L}$ also can remove the conflicts among subsystems $\textbf{SUB}_{n_L}$ : 

 (say in total $H$)
\end{comment}

==> tex/Chapter4_casePC.tex <==
\subsection{Production Cell}
The Production Cell system consists of 9 plant components and 18 control specifications. Due to space limit we refer the description of the system to \cite{FengWonCai2009}, while the detailed step-by-step application of our 6-step approach to \cite{longversion}. 

By our proposed approach with parameter $\beta = 20$, we automatically obtain 18 decentralized supervisors and 4 higher-level coordinators. The hierarchy of these supervisors and coordinators is displayed in Fig.~2, where the clustering results are also shown.

By Theorem~1, the joint behavior of this hierarchy is globally nonblocking. The resulting 4 coordinators are fairly simple: the first three have only 3, 3, and 2 states, while the last one has 16 states. The automata of these 4 coordinators are displayed in Figs.~3 and 4.
In \cite{FengWonCai2009}, by detailed analysis of the specific structural feature of this system, 
2 coordinators with 2 states and 15 state respectively are obtained to ensure global nonblocking behavior. Compared to \cite{FengWonCai2009}, our approach is fully automatic without needing structural analysis; although our approach returns 4 coordinators, their states sizes are fairly close to those handcrafted ones in \cite{FengWonCai2009}.


% : Stock, Feed Belt, Elevating Rotary Table, Rotary Base, Arm1, Arm2,
% Press, Deposit Belt, and Crane. The cell processes workpieces, called
% `blanks', having state size of order 10${}^{7}$. 
% The system is shown Fig.\ref{fig:PC}. 
% \begin{figure}[H]
% 	\centering

% 	\includegraphics[width=80mm]{fig/PC.jpg}
%  	\caption{Overview of Production Cell configuration, taken from \cite{SUPLOC}}	
%  	\label{fig:PC}
% \end{figure}
% These nine asynchronous component agents are modeled by eleven component automata, and there are eighteen control specifications.
% Please see Chap.5 in \cite{SUPLOC} for the detailed description of each automaton and event.
% We construct an abstraction based hierarchical architecture for Production Cell system by our approach. %The result is shown in Fig. \ref{fig:PC_S} above.

% By {\bf Step 1}:  We synthesize a decentralized supervisor for each specification. Then we get eighteen decentralized supervisors. 
% %%%%各个自动机列出来

% \renewcommand{\arraystretch}{1.2}
% \begin{table}[H]
% \label{tab:PC_G_E_SUP}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Components & Specifications & Decentralized supervisors\\
% 		\hline
% 	$\textbf{St}$     & $\textbf{FB1}$ \ $\textbf{FB2}$   &  $\textbf{SUP}_{\textbf{FB1}}$ \ $\textbf{SUP}_{\textbf{FB2}}$ \\
% 	$\textbf{FB}$     & $\textbf{Ta1}$ \ $\textbf{Ta2}$   &  $\textbf{SUP}_{\textbf{Ta1}}$ \ $\textbf{SUP}_{\textbf{Ta2}}$ \\
% 	$\textbf{Ta\_V}$  &  $\textbf{Ta3}$ \ $\textbf{Ta4}$  &  $\textbf{SUP}_{\textbf{Ta3}}$ \ $\textbf{SUP}_{\textbf{Ta4}}$ \\
% 	$\textbf{Ta\_H }$ &  $\textbf{A1T}$ \ $\textbf{Pr1}$  &  $\textbf{SUP}_{\textbf{A1T}}$ \ $\textbf{SUP}_{\textbf{Pr1}}$ \\
% 	$\textbf{Pr }$    &  $\textbf{Pr2}$ \ $\textbf{A1P}$  &  $\textbf{SUP}_{\textbf{Pr2}}$ \ $\textbf{SUP}_{\textbf{A1P}}$ \\
% 	$\textbf{Ro}$     &  $\textbf{A2P}$ \ $\textbf{R1}$   &  $\textbf{SUP}_{\textbf{A2P}}$ \ $\textbf{SUP}_{\textbf{R1}}$ \\
% 	$\textbf{A1}$     &  $\textbf{R2}$ \ $\textbf{R3}$    &  $\textbf{SUP}_{\textbf{R2}}$ \ $\textbf{SUP}_{\textbf{R3}}$ \\
% 	$\textbf{A2}$     &  $\textbf{R4}$ \ $\textbf{DB1}$   &  $\textbf{SUP}_{\textbf{R4}}$ \ $\textbf{SUP}_{\textbf{DB1}}$ \\
% 	$\textbf{DB}$     &  $\textbf{DB2}$ \ $\textbf{DB3}$  &  $\textbf{SUP}_{\textbf{DB2}}$ \ $\textbf{SUP}_{\textbf{DB3}}$ \\
% 	$\textbf{Cr\_V}$  &     &   \\
% 	$\textbf{Cr\_H}$  &    &   \\
		
% 		\hline
% 	\end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}
% %%%
% By {\bf Step 2}:  Next we create a DMM {\bf P} to record the dependencies between these eleven component models and eighteen decentralized supervisors. The matrix {\bf P} is shown below.
% %%%%%%%%%%%%%%%%%PR
% \begin{table}[H]
% \caption{The DMM {\bf P} of the Production Cell system. \\ }
% \label{table:PC_DMM}
% \centering
% \setlength{\tabcolsep}{0.5mm}{
%     \begin{tabular}{c||c|c|c|c|c|c|c|c|c|c|c|}
%             %row1
%              & $\textbf{St}$ & $\textbf{FB}$ & $\textbf{Ta\_V}$ & $\textbf{Ta\_H }$ & $\textbf{Pr }$  & $\textbf{Ro}$ & $\textbf{A1}$ & $\textbf{A2}$ & $\textbf{DB}$ & $\textbf{Cr\_V}$ &  $\textbf{Cr\_H}$\\
%             \hline
%             \hline
%             %row2 
%             $\textbf{SUP}_{\textbf{FB1}}$  & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 \\ 
%              \hline
%             %row3 
%             $\textbf{SUP}_{\textbf{FB2}}$ &1  & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 \\
%              \hline
%             %row4 
%             $\textbf{SUP}_{\textbf{Ta1}}$ & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%              \hline
%             %row5 
%             $\textbf{SUP}_{\textbf{Ta2}}$ & 0 & 0 & 1 & 0 &0  & 0 & 1 & 0 & 0 & 0 & 0 \\ 
%              \hline
%             %row6 
%              $\textbf{SUP}_{\textbf{Ta3}}$ & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%              \hline
%             %row7 
%              $\textbf{SUP}_{\textbf{Ta4}}$ & 0& 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 0 &  0\\ 
%              \hline
%              %row8 
%             $\textbf{SUP}_{\textbf{A1T}}$ & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 \\ 
%              \hline
%             %row9 
%             $\textbf{SUP}_{\textbf{Pr1}}$ & 0 &  0& 0 & 0 & 1 & 0 &1  & 0 &0  & 0 & 0 \\ 
%              \hline
%             %row10 
%             $\textbf{SUP}_{\textbf{Pr2}}$ & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 1 & 0 & 0 &0  \\ 
%              \hline
%             %row11 
%             $\textbf{SUP}_{\textbf{A1P}}$ & 0 &0 & 0 & 0 & 1 &1  & 1 & 0 & 0 &  0&  0\\ 
%              \hline
%             %row12 
%             $\textbf{SUP}_{\textbf{A2P}}$ & 0 & 0 & 0 & 0 & 1 & 1 & 0 &  1&0  & 0& 0 \\ 
%              \hline
%             %row13 
%             $\textbf{SUP}_{\textbf{R1}}$ & 0 & 0 & 0 & 0 & 0 &1  &  1& 0 & 0 & 0 & 0 \\ 
%              \hline
%             %row14 
%             $\textbf{SUP}_{\textbf{R2}}$ & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 &0 \\
%              \hline
%             %row15 
%             $\textbf{SUP}_{\textbf{R3}}$ &  0& 0 &  0&  0& 0 & 1 & 1 & 0 &  0& 0 & 0 \\ 
%              \hline
%             %row16 
%             $\textbf{SUP}_{\textbf{R4}}$ & 0 & 0 & 0 & 0 & 0 &  1& 0 & 1 & 0 & 0 & 0 \\ 
%              \hline
%             %row17 
%             $\textbf{SUP}_{\textbf{DB1}}$ & 0 & 0 & 0 & 0 & 0 &  0& 0 & 1 & 1 & 1 & 1 \\
%              \hline
%             %row18 
%             $\textbf{SUP}_{\textbf{DB2}}$ & 0 & 0 & 0& 0 & 0& 0 & 0 & 1 & 1 & 0 & 0 \\ 
%              \hline
%             %row19 
%             $\textbf{SUP}_{\textbf{DB3}}$ & 0 & 0 & 0 &  0& 0 & 0 &  0& 0 & 1 &1  & 1 \\ 
%              \hline
         
%     \end{tabular}}

% \end{table}
% %
% After this step, we multiply {\bf P} with its tranpose matrix ${\bf P^\top}$ to get the DSM shown in Table \ref{table:PC_DSM}. 
% %%%%%%%%%%%%%%%%%%%%P
% \begin{table}[H]
% \caption{The DSM of the Production Cell system. ${\bf P_{D}=P\times P^\top}$\\ }
% \label{table:PC_DSM}
% \centering
% \setlength{\tabcolsep}{0.6mm}{
%     \begin{tabular}{c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%             %row1
%              & \rotatebox{90}{$\textbf{SUP}_{\textbf{FB1}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{FB2}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Ta1}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Ta2}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Ta3}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Ta4}}$} & \rotatebox{90}
%              {$\textbf{SUP}_{\textbf{A1T}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Pr1}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Pr2}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{A1P}}$} &
%              \rotatebox{90}{$\textbf{SUP}_{\textbf{A2P}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{R1}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{R2}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{R3}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{R4}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{DB1}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{DB2}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{DB3}}$}  \\
%              \hline
%              \hline
%             %row2 
%            $\textbf{SUP}_{\textbf{FB1}}$  & 4 & 4 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 &  0& 0 & 0 & 0 &2  & 0 &  2  \\
%              \hline
%             %row3 
%            $\textbf{SUP}_{\textbf{FB2}}$   & 4 & 4 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 &  0& 0 & 0 & 0 &2  & 0 &  2  \\ 
%              \hline
%             %row4 
%            $\textbf{SUP}_{\textbf{Ta1}}$ & 1 & 1 & 2 & 1 & 1 & 0 &1  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0   \\
%              \hline
%             %row5 
%            $\textbf{SUP}_{\textbf{Ta2}}$  & 0 & 0 & 1 & 2 & 0 & 1 &  1& 1 & 0 & 1 &0  & 1 & 0 & 1 & 0 & 0 & 0 & 0   \\ 
%              \hline
%             %row6 
%             $\textbf{SUP}_{\textbf{Ta3}}$ & 1 & 1 &1  & 0 & 2 & 1 & 0 & 0 &  0& 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0   \\
%              \hline
%             %row7 
%             $\textbf{SUP}_{\textbf{Ta4}}$ & 0 & 0 &0 & 1 & 1 & 2 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0   \\ 
%              \hline
%              %row8 
%             $\textbf{SUP}_{\textbf{A1T}}$ & 0 & 0 & 1 & 1 & 0 & 0 & 2 & 0 & 0 & 1 & 1 & 1 & 1 &  1&1  & 0 & 0 & 0   \\ 
%              \hline
%             %row9 
%             $\textbf{SUP}_{\textbf{Pr1}}$ & 0 & 0 &  0& 1 & 0 & 1 & 0& 2 &  1& 2 & 1 & 1 &  0& 1 & 0 & 0 & 0 & 0   \\ 
%              \hline
%             %row10 
%             $\textbf{SUP}_{\textbf{Pr2}}$ &0  & 0 & 0 & 0 & 0 & 0& 0 & 1 & 2 &  1& 2 & 0 & 1 & 0 & 1 & 1 & 1 &  0  \\ 
%              \hline
%             %row11 
%             $\textbf{SUP}_{\textbf{A1P}}$ & 0 & 0 & 0 & 1 & 0 & 1 & 1 & 2 & 1& 3 &  2&  2& 1 & 2 & 1 & 0 & 0 & 0   \\
%              \hline
%             %row12 
%             $\textbf{SUP}_{\textbf{A2P}}$ & 0 & 0 & 0 & 0 & 0 & 0 &  1& 1& 2 &  2& 3 &  1& 2 & 1 & 2 &  1& 1 & 0   \\ 
%              \hline
%             %row13 
%             $\textbf{SUP}_{\textbf{R1}}$ & 0 & 0 & 0 & 1 & 0 & 1 & 1 &  1& 0 & 2 & 1 & 2 & 1 & 2 & 1 &  0& 0 & 0   \\ 
%              \hline
%             %row14 
%             $\textbf{SUP}_{\textbf{R2}}$ & 0 & 0 & 0 & 0 & 0 & 0 & 1& 0 & 1 & 1 &  2& 1 &  2& 1 & 2 & 1 & 1 &0    \\ 
%              \hline
%             %row15 
%             $\textbf{SUP}_{\textbf{R3}}$ & 0& 0 & 0 & 1 & 0 & 1 & 1 & 1 & 0 & 2 &  1& 2 &1  & 2 & 1 &0  & 0 & 0  \\ 
%              \hline
%             %row16 
%             $\textbf{SUP}_{\textbf{R4}}$ & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 1 & 2 & 1 & 2 & 1 & 2 & 1 & 1 &  0  \\ 
%              \hline
%             %row17 
%             $\textbf{SUP}_{\textbf{DB1}}$ & 2 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 & 4 & 2 & 3   \\
%              \hline
%             %row18 
%             $\textbf{SUP}_{\textbf{DB2}}$ & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 1 & 0 & 1 &2  &2  & 1   \\ 
%              \hline
%             %row19 
%             $\textbf{SUP}_{\textbf{DB3}}$ & 2 & 2 &0  & 0 & 0 & 0 & 0 &0  & 0 & 0 &  0& 0 & 0 & 0 & 0 & 3 &1  & 3   \\ 
%              \hline     
%     \end{tabular}}
% \end{table}
% %
% %
% To turn the DSM ${\bf P_{D}}$ into a probability matrix $\textbf{M}$ for the clustering step, we do the column normalization. The result is given by:
% %%%%%%%%%%%%%%%%%%%%%M
% \begin{tiny}
% \begin{fleqn}[-40pt]
% \[
% \textbf{M}=
% \left(
% \begin{smallmatrix}
% %
%     0.2857  &  0.2857  &  0.1429  &       0  &  0.1667   &      0  &       0   &      0   &      0  &       0  &       0  &       0  &       0 &        0 &        0 &   0.1176 &        0  &  0.1818\\
%     0.2857  &  0.2857  &  0.1429  &       0  &  0.1667   &      0  &       0   &      0    &     0  &       0  &       0  &       0  &       0 &        0  &       0 &   0.1176 &        0  &  0.1818\\
%     0.0714  &  0.0714  &  0.2857  &  0.1111  &  0.1667   &      0  &  0.1000   &      0    &     0  &       0  &       0  &       0  &       0  &       0 &        0 &        0 &        0  &       0\\
%          0  &       0  &  0.1429  &  0.2222  &       0   & 0.1250  &  0.1000   & 0.1000    &     0  &  0.0588  &       0  &  0.0769  &       0 &   0.0769 &        0 &        0 &        0 &        0\\
%     0.0714  &  0.0714  &  0.1429  &       0  &  0.3333   & 0.1250  &       0   &      0   &      0  &       0  &       0  &       0  &       0 &        0 &        0 &        0 &        0     &    0\\
%          0  &       0  &       0  &  0.1111  &  0.1667   & 0.2500  &       0   & 0.1000   &      0  &  0.0588  &       0  &  0.0769  &       0 &   0.0769 &        0 &        0 &        0 &        0\\
%          0  &       0  &  0.1429  &  0.1111  &       0   &      0  &  0.2000   &      0   &      0  &  0.0588  &  0.0588  &  0.0769  &  0.0769 &   0.0769 &   0.0769 &        0 &        0 &        0\\
%          0  &       0  &       0  &  0.1111  &       0   & 0.1250 &        0   & 0.2000   & 0.1000  &  0.1176  &  0.0588  &  0.0769  &       0 &   0.0769 &        0 &        0 &        0 &        0\\
%          0  &       0  &       0  &       0  &       0   &      0 &        0  &  0.1000   & 0.2000  &  0.0588  &  0.1176  &       0  &  0.0769  &       0 &   0.0769  &  0.0588 &   0.1111 &        0\\
%          0  &       0  &       0  &  0.1111  &       0   & 0.1250  &  0.1000   & 0.2000   & 0.1000  &  0.1765  &  0.1176  &  0.1538  &  0.0769 &   0.1538 &   0.0769 &        0 &        0 &        0\\
%          0  &       0  &       0  &       0  &       0   &      0  &  0.1000  &  0.1000   & 0.2000  &  0.1176  &  0.1765  &  0.0769  &  0.1538 &   0.0769 &   0.1538 &   0.0588 &   0.1111 &        0\\
%          0  &       0  &       0  &  0.1111  &       0   & 0.1250  &  0.1000   & 0.1000   &      0  &  0.1176  &  0.0588  &  0.1538  &  0.0769 &   0.1538 &   0.0769 &        0  &       0 &        0\\
%          0  &       0  &       0  &       0  &       0   &      0  &  0.1000   &      0   & 0.1000  &  0.0588  &  0.1176  &  0.0769  &  0.1538 &   0.0769 &   0.1538 &   0.0588 &   0.1111 &        0\\
%          0  &       0  &       0  &  0.1111  &       0   & 0.1250  &  0.1000   & 0.1000   &      0  &  0.1176  &  0.0588  &  0.1538  &  0.0769 &   0.1538 &   0.0769 &        0 &        0 &        0\\
%          0  &       0  &       0  &       0  &       0   &      0  &  0.1000  &       0   & 0.1000  &  0.0588  &  0.1176  &  0.0769  &  0.1538 &   0.0769 &   0.1538 &   0.0588 &   0.1111 &        0\\
%     0.1429  &  0.1429  &       0  &       0  &       0   &      0   &      0   &      0   & 0.1000  &       0  &  0.0588  &       0  &  0.0769 &        0 &   0.0769 &   0.2353 &   0.2222  &  0.2727\\
%          0  &       0  &       0  &       0  &       0   &      0  &       0   &      0   & 0.1000   &      0   & 0.0588  &       0   & 0.0769 &        0 &   0.0769 &   0.1176 &   0.2222 &   0.0909\\
%     0.1429  &  0.1429  &       0  &       0  &       0   &      0   &      0   &      0    &     0   &      0   &      0  &       0   &      0  &       0 &        0 &   0.1765 &   0.1111  &  0.2727\\
% \end{smallmatrix}
% \right)
% \]
% \end{fleqn}
% \end{tiny}
% %
% This {\bf M} is used as input of MCL for clustering the decentralized supervisors.
% Note that in this Production Cell system, the computation is feasible only when $inflation$ $\beta = 20$.
% After first clustering, the eighteen decentralized supervisors are grouped into five clusters:\\
% %
% Cluster1 :$\textbf{SUP}_{\textbf{DB1}}$, $\textbf{SUP}_{\textbf{DB2}}$, $\textbf{SUP}_{\textbf{DB3}}$.\\
% Cluster2 :$\textbf{SUP}_{\textbf{Pr2}}$, $\textbf{SUP}_{\textbf{A2P}}$, $\textbf{SUP}_{\textbf{R2}}$, $\textbf{SUP}_{\textbf{R4}}$.     \\
% Cluster3 :$\textbf{SUP}_{\textbf{Ta2}}$, $\textbf{SUP}_{\textbf{Ta4}}$, $\textbf{SUP}_{\textbf{A1T}}$, $\textbf{SUP}_{\textbf{Pr1}}$, 
% $\textbf{SUP}_{\textbf{A1P}}$, $\textbf{SUP}_{\textbf{R1}}$, $\textbf{SUP}_{\textbf{R3}}$.   \\
% Cluster4 :$\textbf{SUP}_{\textbf{Ta1}}$.\\
% Cluster5 :$\textbf{SUP}_{\textbf{FB1}}$, $\textbf{SUP}_{\textbf{FB2}}$, $\textbf{SUP}_{\textbf{Ta3}}$.   \\
% %

% By {\bf Step 3}:  We synchronize the automata in the same cluster, and obtain five subsystems $\textbf{SUB}_{layer1,1}$,..., $\textbf{SUB}_{layer1,5}$:
% % sync SUB_l1
% \begin{itemize}
%     %C1
%     \item $\textbf{SUB}_{layer1,1} = \textbf{SUP}_{\textbf{DB1}} || \textbf{SUP}_{\textbf{DB2}} || \textbf{SUP}_{\textbf{DB3}} $.
%     %C2
%     \item $\textbf{SUB}_{layer1,2} = \textbf{SUP}_{\textbf{Pr2}} || \textbf{SUP}_{\textbf{A2P}} || \textbf{SUP}_{\textbf{R2}} || \textbf{SUP}_{\textbf{R4}} $.
%     %C3
%     \item $\textbf{SUB}_{layer1,3} = \textbf{SUP}_{\textbf{Ta2}} || \textbf{SUP}_{\textbf{Ta4}} || \textbf{SUP}_{\textbf{A1T}} || \textbf{SUP}_{\textbf{Pr1}} || 
%           \textbf{SUP}_{\textbf{A1P}}\\ || \textbf{SUP}_{\textbf{R1}} || \textbf{SUP}_{\textbf{R3}}$.
%     %C4
%     \item $\textbf{SUB}_{layer1,4} = \textbf{SUP}_{\textbf{Ta1}}  $.    
%     %C5
%     \item $\textbf{SUB}_{layer1,5} = \textbf{SUP}_{\textbf{FB1}} || \textbf{SUP}_{\textbf{FB2}} ||\textbf{SUP}_{\textbf{Ta3}}  $.
%     %
% \end{itemize}
% %
% Check conflicts inside each subsystem and find that there are two subsystems with conflicts, so we design the coordinators $\textbf{CO}_1$ and $\textbf{CO}_2$ to remove conflicts in $\textbf{SUB}_{layer1,2}$ and $\textbf{SUB}_{layer1,3}$, respectively.

% By {\bf Step 4}:  We abstract the subsystems and get five abstraction models $\textbf{ABS}_{layer1,1},...,\textbf{ABS}_{layer1,5}$.
 
% Return back to {\bf Step 2}: Construct a new DMM \textbf{P} to record the dependencies between abstractions and plant components.
% The matrices $\textbf{P}$, $\textbf{P}_\textbf{D}$ and $\textbf{M}$ for this second level clustering are shown below.
% %%%%%%%%PR ABS
% \begin{table}[H]
% \caption{The DMM {\bf P} of abstractions on layer 1. \\ }
% \label{table:PC_DMM_ABSL1}
% \centering
% \setlength{\tabcolsep}{0.6mm}{
%     \begin{tabular}{c||c|c|c|c|c|c|c|c|c|c|c|}
%             %row1
%              & $\textbf{St}$ & $\textbf{FB}$ & $\textbf{Ta\_V}$ & $\textbf{Ta\_H }$ & $\textbf{Pr }$  & $\textbf{Ro}$ & $\textbf{A1}$ & $\textbf{A2}$ & $\textbf{DB}$ & $\textbf{Cr\_V}$ &  $\textbf{Cr\_H}$\\
%             \hline
%             \hline
%             %row2
%    $\textbf{ABS}_{layer1,1}$ & 0  &   0  &   0 &    0  &   0  &   0  &   0  &   1  &   1  &   1  &   1\\
%    \hline
%    $\textbf{ABS}_{layer1,2}$ & 0  &   0  &   0 &    0  &   1  &   1  &   0  &   1  &   0  &   0  &   0\\
%    \hline
%    $\textbf{ABS}_{layer1,3}$ & 0  &   0  &   1 &    1  &   1  &   1  &   1  &   0  &   0  &   0  &   0\\
%    \hline
%    $\textbf{ABS}_{layer1,4}$ & 0  &   1  &   1 &    0  &   0  &   0  &   0  &   0  &   0  &   0  &   0\\
%    \hline
%    $\textbf{ABS}_{layer1,5}$ & 1  &   1  &   0 &    1  &   0  &   0  &   0  &   0  &   0  &   1  &   1\\
%    \hline
%     \end{tabular}}
% \end{table}
% %
% %%%%%%%%%%%%%P_ABS
% %
% \begin{table}[H]
% \caption{The DSM of of abstractions on layer 1. ${\bf P_{D}=P\times P^\top}$\\ }
% \label{table:PC_DSM_ABSL1}
% \centering
% \setlength{\tabcolsep}{1.0mm}{
%     \begin{tabular}{c||c|c|c|c|c|}
%      & \rotatebox{90}{ $\textbf{ABS}_{layer1,1}$} & \rotatebox{90}{$\textbf{ABS}_{layer1,2}$} & \rotatebox{90}{ $\textbf{ABS}_{layer1,3}$} & \rotatebox{90}{ $\textbf{ABS}_{layer1,4}$} & \rotatebox{90}{$\textbf{ABS}_{layer1,5}$} \\
%     \hline
%     \hline
%     $\textbf{ABS}_{layer1,1}$ & 4 &    1 &    0 &    0 &    2\\
%     \hline
%     $\textbf{ABS}_{layer1,2}$ & 1 &    3 &    2 &    0 &    0\\
%     \hline
%     $\textbf{ABS}_{layer1,3}$ & 0 &    2 &    5 &    1 &    1\\
%     \hline
%     $\textbf{ABS}_{layer1,4}$ & 0 &    0 &    1 &    2 &    1\\
%     \hline
%     $\textbf{ABS}_{layer1,5}$ & 2 &    0 &    1 &    1 &    5\\
%     \hline

    
%     \end{tabular}}
% \end{table}
% %
% %%%%%%%%%%%%%%%M_ABS
% \[
% \textbf{M}=
% \left(
% \begin{matrix}
%     0.5714 &   0.1667 &        0 &        0 &   0.2222\\
%     0.1429 &   0.5000 &   0.2222 &        0 &        0\\
%          0 &   0.3333 &   0.5556 &   0.2500 &   0.1111\\
%          0 &        0 &   0.1111 &   0.5000 &   0.1111\\
%     0.2857 &        0 &   0.1111 &   0.2500 &   0.5556\\
% \end{matrix}
% \right)
% \]
% %
% %
% %ABS cluster

% By {\bf Step 3}: By  clustering these five abstractions, we get 3 clusters as shown below.
% \renewcommand{\arraystretch}{1.4}
% \begin{table}[H]
% \label{tab:PC_ABSL1_C}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Cluster 1 &Cluster 2 & Cluster 3 \\
% 		\hline
% 		\hline
% 		$\textbf{ABS}_{layer1,5}$ & $\textbf{ABS}_{layer1,2}$ & $\textbf{ABS}_{layer1,1}$\\
%                                   &$\textbf{ABS}_{layer1,3}$ &\\
%                                   &$\textbf{ABS}_{layer1,4}$ &\\
% 		\hline
% 	\end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}

% %
% %SUB_L2
% The components of each cluster are combined using synchronous product to create the subsystems $\textbf{SUB}_{layer2,1},\dots,\\ \textbf{SUB}_{layer2,3}$.
% Since cluster 1 and cluster 3 only have one abstraction, abstractions $\textbf{ABS}_{layer1,1}$ and $\textbf{ABS}_{layer1,5}$ are already the new subsystems respectively:
% \begin{itemize}
% \item $\textbf{SUB}_{layer2,1} = \textbf{ABS}_{layer1,5}$
% \item $\textbf{SUB}_{layer2,2} =\textbf{ABS}_{layer1,1} || \textbf{ABS}_{layer1,3} || \textbf{ABS}_{layer1,4}$
% \item $\textbf{SUB}_{layer2,3} = \textbf{ABS}_{layer1,1}$
% \end{itemize}

% %
%  The second subsystem $\textbf{SUB}_{layer2,2}$ has conflicts, so a coordinator $\textbf{CO}_3$ is designed to make $\textbf{SUB}_{layer2,2}$ nonblocking. 
% %

% By {\bf Step 4}: These three subsystems $\textbf{SUB}_{layer2,1},..,\textbf{SUB}_{layer2,3}$ in layer 2 are further abstracted into three abstractions $\textbf{ABS}_{layer2,1}$, $\textbf{ABS}_{layer2,2}$, $\textbf{ABS}_{layer2,3}$.

% Return back to {\bf Step 2}: For this upper layer, we also construct a new DMM $\textbf{P}$ to record the dependencies between abstractions $\textbf{ABS}_{layer2,1}$, $\textbf{ABS}_{layer2,2}$, $\textbf{ABS}_{layer2,3}$ and plant components.
% The matrices $\textbf{P}$, $\textbf{P}_\textbf{D}$ and $\textbf{M}$ for this third level clustering are shown below.
% %
% %%%%%%%%PR ABSL2
% %
% \begin{table}[H]
% \caption{The DMM {\bf P} of abstractions on layer 2. \\ }
% \label{table:PC_DMM_ABSL1}
% \centering
% \setlength{\tabcolsep}{0.5mm}{
%     \begin{tabular}{c||c|c|c|c|c|c|c|c|c|c|c|}
%             %row1
%              & $\textbf{St}$ & $\textbf{FB}$ & $\textbf{Ta\_V}$ & $\textbf{Ta\_H }$ & $\textbf{Pr }$  & $\textbf{Ro}$ & $\textbf{A1}$ & $\textbf{A2}$ & $\textbf{DB}$ & $\textbf{Cr\_V}$ &  $\textbf{Cr\_H}$\\
%             \hline
%             \hline
%             %row2
%    $\textbf{ABS}_{layer2,1}$ & 1  &   1  &   0 &    1  &   0  &   0  &   0  &   0  &   0  &   1  &   1\\
%    \hline
%    $\textbf{ABS}_{layer2,2}$ & 0  &   1  &   0 &    1  &   0  &   0  &   0  &   1  &   0  &   0  &   0\\
%    \hline
%    $\textbf{ABS}_{layer2,3}$ & 0  &   0  &   0 &    0  &   0  &   0  &   0  &   1  &   1  &   1  &   1\\
%    \hline
%     \end{tabular}}
% \end{table}
% %%%
% %%
% %
% %
% %%%%%%%%%%%%%P_ABS_L2
% %
% \begin{table}[H]
% \caption{The DSM of of abstractions on layer 2. ${\bf P_{D}=P\times P^\top}$\\ }
% \label{table:PC_DSM_ABSL2}
% \centering
%     \begin{tabular}{c||c|c|c|}
%      & $\textbf{ABS}_{layer2,1}$ &  $\textbf{ABS}_{layer2,2}$ & $\textbf{ABS}_{layer2,3}$  \\
%     \hline
%     \hline
%     $\textbf{ABS}_{layer2,1}$ & 5 &    2 &    2 \\
%     \hline
%     $\textbf{ABS}_{layer2,2}$ & 2 &    3 &    1 \\
%     \hline
%     $\textbf{ABS}_{layer2,3}$ & 2 &    1 &    4 \\
%     \hline    
%     \end{tabular}
% \end{table}
% %%%
% %%
% %
% %%%%%%%%%%%%%%%M_ABSL2
% \[
% \textbf{M}=
% \left(
% \begin{matrix}
%     0.5556   & 0.3333 &   0.2857\\
%     0.2222   & 0.5000 &   0.1429\\
%     0.2222   & 0.1667 &   0.5714\\
% \end{matrix}
% \right)
% \]
% %%%
% %%
% %
% By {\bf Step 3}: Perform the clustering again for these three abstractions and we obtain two clusters:\\
% %cluster on layer3
% \renewcommand{\arraystretch}{1.4}
% \begin{table}[H]
% \label{tab:PC_ABSL3_C}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Cluster 1 &Cluster 2\\
% 		\hline
% 		\hline
% 		$\textbf{ABS}_{layer2,1}$ & $\textbf{ABS}_{layer2,3}$\\
%         $\textbf{ABS}_{layer2,2}$ & \\	                         
% 		\hline
% 	\end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}
% %
% %
% %SUB on layer 3
% For cluster 1, we perform synchronous product of these two abstractions to obtain a new subsystem $\textbf{SUB}_{layer3,1}$. 
% There is only one abstraction in cluster 2, so $\textbf{ABS}_{layer2,3}$ already is the new subsystem $\textbf{SUB}_{layer3,2}$.
% \begin{itemize}
% \item $\textbf{SUB}_{layer3,1} =\textbf{ABS}_{layer2,1} || \textbf{ABS}_{layer2,3}$
% \item $\textbf{SUB}_{layer3,2} = \textbf{ABS}_{layer2,2}$
% \end{itemize}
% %
% Each of these two subsystems $\textbf{SUB}_{layer3,1},\textbf{SUB}_{layer3,2}$ is checked to be nonblocking, so no new coordinator is designed.

% By {\bf Step 4}: We further abstract $\textbf{SUB}_{layer3,1}$ and $\textbf{SUB}_{layer3,2}$ to get abstractions 
% $\textbf{ABS}_{layer3,1}$ and $\textbf{ABS}_{layer3,2}$. 
% We treat these two abstractions as one cluster. In this cluster, the two abstractions are conflicting, so $\textbf{CO}_4$ is designed to remove the conflicts. 

% The design procedure ends here since the number of clusters is no more than two. There are eighteen decentralized supervisors and four coordinators $\textbf{CO}_1,...,\textbf{CO}_4$. 
%  The state number of the coordinators is shown Table \ref{tab:PCCO}. We also give the models of $\textbf{CO}_1,...,\textbf{CO}_4$ which are shown in Fig.\ref{fig:PC_CO123} and Fig.\ref{fig:PC_CO4}. The system construct obtained by our approach  is shown in Fig.\ref{fig:PC_S}.


% %%%

% \renewcommand{\arraystretch}{1.5}
% \begin{table}[H]
% \caption{Four coordinators are computed}
% \label{tab:PCCO}
% 	\centering
% 	\begin{tabular}{|c||c|c|c|c|}
% 		\hline
		
% 		$\beta = 20$ &  ${\bf CO_1} $& ${\bf CO_2}$ & ${\bf CO_3}$ & ${\bf CO_4}$\\
% 		\hline
% \hline
% 	State numbers	& 3         &   3 &  2& 16 \\

% 		\hline
% 	\end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}
% %%%
\begin{figure}[t]
	\centering

	\includegraphics[width=90mm]{fig/PC_struscture.jpg}
 	\caption{Hierarchy of 18 decentralized supervisors (all at the bottom level) and 4 coordinators (across different levels)}	
 	\label{fig:PC_S}
\end{figure}
%
\begin{figure}[H]
	\centering

	\includegraphics[width=90mm]{fig/PC_CO123.jpg}
 	\caption{Coordinators $\textbf{CO}_1$, $\textbf{CO}_2$, $\textbf{CO}_3$}	
 	\label{fig:PC_CO123}
\end{figure}
%


%
\begin{figure}[H]
	\centering

	\includegraphics[width=90mm]{fig/PC_CO4.jpg}
 	\caption{Coordinator $\textbf{CO}_4$}	
 	\label{fig:PC_CO4}
\end{figure}

%
% {\bf Comparison of coordinators }
% Here we compare the coordinators $\textbf{CO}_{01}$ and $\textbf{CO}_{02}$ designed by the approach in \cite{Feng2008} and our obtained coordinators  $\textbf{CO}_1,...,\textbf{CO}_4$, where $\textbf{CO}_{01}$ and $\textbf{CO}_{02}$ are shown in Fig.\ref{fig:PC_CO_old1} and Fig.\ref{fig:PC_CO_old2}.
% %
% \begin{figure}[H]
% 	\centering

% 	\includegraphics[width=40mm]{fig/PC_CO_old1.jpg}
%  	\caption{Coordinator $\textbf{CO}_{01}$ by approach in \cite{Feng2008}}	
%  	\label{fig:PC_CO_old1}
% \end{figure}

% %
% \begin{figure}[H]
% 	\centering

% 	\includegraphics[width=90mm]{fig/PC_CO_old2.jpg}
%  	\caption{Coordinator $\textbf{CO}_{02}$ by approach in \cite{Feng2008}}	
%  	\label{fig:PC_CO_old2}
% \end{figure}
% %
% The control logic of $\textbf{CO}_{01}$ shows that the event $A2\_F80$ (Arm2 extends its length to 80) is disabled before event $Pr\_B$ occurs (Press descends back to bottom and prepares to unload the forged blank to Arm2), to make Arm2 to stay at its initial state during the first work cycle of Press.

% The control logic of $\textbf{CO}_{02}$ is to disable event $St\_add$ (adding a blank into the cell) if and when there are 7 blanks. 
% The reason is that the total capacity of the production cell is eight and the whole cell contains a loop with material feedback: faulty blanks are transported by Crane from DBelt back to FBelt. Moreover, the feedback event $DB \_ n$ (the blank fails the check) is uncontrollable, so at least one empty slot must be maintained in the cell.
% %
% %CO1:要等Press到底层才能伸长A2到80，或者转回40du
% %CO2：A1是65的时候，不能转到90度，因为会撞。或者是Press不在中间的时候不能伸长。
% %CO3：要等Press到底层时才能伸长到80
% %CO4: 往DBelt（容量为2）里送了2个东西以后，（A2OFF或者A2S0发生两次） FBEL只剩下一个容量的时候，需要禁止往系统里送东西，只到DB的东西被送出系统或者送回FBEL，防止系统整体的OBVERFLOW。
% %我们与原来多了9个状态，是因为我们的CO需要观察DB的东西数量与FB的数量来判断系统内已经存在的东西的数量。而原来的CO只需要观察系统的输入数量与输出数量就能知道系统内的部品数量。
% %

% For the four coordinators $\textbf{CO}_1,...,\textbf{CO}_4$ synthesized by our approach,   the control logic and the comparison with $\textbf{CO}_{01}$ and $\textbf{CO}_{02}$ are given in the following.

% The control logic of $\textbf{CO}_{1}$: \\
% 1. When event $Ro\_C$ occurs (RBase turns clockwise back to 40 degrees), the event $A2\_F80$ is disabled before the event $Pr\_B$  occurs. 
% Since event $Ro\_C$ occurs, Press is not in its first work cycle. 
% Therefore, the difference between $\textbf{CO}_{01}$ and $\textbf{CO}_{1}$ is that: $\textbf{CO}_{1}$ ensures that if RBase is at 40 degrees, Arm2 can extend its length to 80 only when Press descends back to bottom  to avoid the collision, instead of forcing Arm2 to stay put at its initial state during the first work cycle of Press by $\textbf{CO}_{01}$. 
% Note that this control logic is in fact redundant because this collision prevention is already ensured by supervisor $\textbf{SUP}_{\textbf{A2P}}$.\\
% 2. Disable event $Ro\_C$ when Arm2 has extended its length to 80 (event $A2\_F80$) but not placed a blank onto DBelt yet. 
% This control logic is not contained in $\textbf{CO}_{01}$ and $\textbf{CO}_{02}$.
% Note that  this second control of $\textbf{CO}_{1}$ is also redundant because supervisor $\textbf{SUP}_{\textbf{R4}}$ already has this control logic.

% Next, the control logic of $\textbf{CO}_{2}$: \\
% 1. Disable event $Ro\_CC$ (RBase turns clockwise to 90 degrees) when Arm1 has extended its length to 65 (event $A2\_F65$), for preventing the collision.\\
% 2. Disable event $A2\_F65$ to avoid the collision circumstances that RBase is at 90 degrees (event $Ro\_CC$ occurs) and the length of Arm1 is longer than 37 ($A2\_S52$ occurs). \\
% These two control logic prevent Arm1 from collision, which are also contained in supervisor $\textbf{SUP}_{\textbf{A1P}}$.

% As shown in Fig.\ref{fig:PC_CO123}, the control logic of $\textbf{CO}_{3}$ is same as $\textbf{CO}_{01}$ 
% which disables event $A2\_F80$ before event $Pr\_B$  occurs. 

% The control logic of $\textbf{CO}_{4}$:\\ 
% When DBelt already holds two blanks (event $A2\_Off$ occurs twice) and ERTable already holds one blank (event $FB\_s1Off$ occurs),  disable event $St\_add$ if there exists a new blank in Fbelt (event $FB\_s1On$ occurs).
% %如介绍CO02时所说，此PC系统必须要留出一个空位来应对不合格faulty blanks are transported by Crane from DBelt back to FBelt; moreover, the feedback event DB_n is uncontrollable. 

% This control logic is similar to $\textbf{CO}_{02}$ that $\textbf{CO}_{4}$ ensures that Fbelt has one empty slot at least such that the faulty blanks can be transported by Crane from DBelt back to FBelt.
% The difference is that $\textbf{CO}_{02}$ only observes how many blanks are added in the PC and how many blanks are passed the test (event $DB\_y$) or outputted from the system (event $DB\_O$). There are eight states in $\textbf{CO}_{02}$ to execute its control logic.
% However, the $\textbf{CO}_{4}$ (16 states) needs to observe the blank number in Fbelt, ERTable, and DBelt to determine if the event $St\_add$ needs to be disabled to prevent the system from being `chocked'. 
%CO02只有8个状态的原因是它只需要观察有多少blank进入了PC，有多少blank被送出了系统。而我们需要通过同时观察DBelt，Rrtable和Fbelt里blank的数量来防止整个系统出现冲突。






%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\begin{comment}
%
            %row1
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row2 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row3 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row4 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row5 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row6 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row7 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
             %row8 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row9 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row10 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row11 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row12 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row13 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row14 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row15 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
             %row16 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row17 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%
            %row18 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
%
            %row19 
             &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
\end{comment}

==> tex/Chapter4_case_AGV.tex <==
\section{Case studies}
\label{chap:4}
In this section, we demonstrate the effectiveness of our proposed Markov clustering based approach on two benchmark case studies: 
automatic guided vehicles (AGVs) 
%\cite{AGV} 
and Production Cell. 
%\cite{PC}.

\subsection{Automatic Guided Vehicles}\label{sec:AGV}
%大概介绍AGV，输入G和E,输出结果，结果表（infl不同），然后再说一句可以确认
The AGV system consists of five automatic guided vehicles {\bf AGV1}$,...,${\bf AGV5} serving a manufacturing workcell.  This workcell consists of two input stations {\rm IPS1, IPS2}; three workstations {\rm WS1, WS2, WS3}; one completed parts station {\rm CPS}; and four shared zones Z1, Z2, Z3, Z4 for the AGVs. Detailed description of the system and the automata of the AGVs are referred to \cite{Feng2008}. 
For this system, the following control specifications are imposed:
\begin{itemize}
\item Each of the four shared zones Z1, Z2, Z3, Z4 should be occupied by at most one AGV at a time.
\item Only one of {\bf AGV1, AGV2} can be loaded at a time in two input stations {\rm IPS1, IPS2}.
\item Only one part can be processed at a time by each of {\rm WS2}, {\rm WS3}, while {\rm WS1} can assemble just two parts (a Type1 and a Type2) at a time into a complete part. Three workstations must be protected against overflow and underflow. 
\end{itemize}
The above requirements can be modeled by 9 specification automata (\cite{Feng2008}): $\textbf{Z}_1, \textbf{Z}_2,\textbf{Z}_3, \textbf{Z}_4, \textbf{WS}_{13}, \textbf{WS}_{14}, \textbf{WS}_{2}, \textbf{WS}_{3}, \textbf{IPS}.$
% \[
% \textbf{Z}_1, \textbf{Z}_2,\textbf{Z}_3, \textbf{Z}_4, \textbf{WS}_{13}, \textbf{WS}_{14}, \textbf{WS}_{2}, \textbf{WS}_{3}, \textbf{IPS}.
% \]



%%%%%fig
% \begin{figure}[t]
% 	\centering
	
% 	\includegraphics[width=60mm]{fig/AGV.jpg}
%  	\caption{AGVs system, taken from \cite{Feng2008}}
%  	\label{fig:AGVworkcell}
% \end{figure}

% \begin{figure}[t]
% 	\centering

% 	\includegraphics[width=80mm]{fig/AGV_G.jpg}
% \caption{Plant components of AGV, taken from \cite{SUPLOC}}
%  	\label{fig:AGVplant}
% \end{figure}
%%%%%


%%%%%
%定理NB 
%超过2个
%proposition

% %%%%%%%%%%%%events of AGV
% \renewcommand{\arraystretch}{0.8}
% \begin{table}[H]
%  	\caption{Interpretation of events }
% 	\label{table:AGVevent}
% 	\centering
% 	\begin{tabular}{ l|l|l}
% 		\hline\hline
% 		Event & \textbf{AGV} & Interpretation \\
% 		\hline
% 		11 & 1 &  Leaves {\bf WS2} and enters Zone 1 \\
% 		\hline
% 		10 &  &  Exits Zone 1 and loads from {\bf IPS1} \\
% 		\hline
% 		13 &  &  Re-enters Zone 1 \\
% 		\hline
% 		12 &  &  Exits Zone 1, unloads to {\bf WS2} and parks \\
% 		\hline
% 		21 & 2 & Leaves {\bf WS3} and enters Zone 3  \\
% 		\hline
% 		18 &  &  Exits Zone 3 and enters Zone 2 \\
% 		\hline
% 		20 &  &  Exits Zone 2 and enters Zone 1 \\
% 		\hline
% 		22 &  & Exits Zone 1 and loads from {\bf IPS2}  \\
% 		\hline
% 		23 &  & Re-enters Zone 1  \\
% 		\hline
% 		24 &  & Exits Zone 1 and re-enters Zone 2  \\
% 		\hline
% 		26 &  &  Exits Zone 2 and re-enters Zone 3 \\
% 		\hline
% 		28 &  & Exits Zone 3, unloads to {\bf WS3} and parks  \\
% 		\hline
% 		33 & 3 & Leaves {\bf WS1} and enters Zone 2  \\
% 		\hline
% 		34 &  &  Exits Zone 2 and loads from {\bf WS2} \\
% 		\hline
% 		31 &  &  Re-enters Zone 2 \\
% 		\hline
% 		32 &  &  Exits Zone 2, unloads to {\bf WS1} and parks \\
% 		\hline
% 		41 & 4 & Leaves {\bf WS1} and enters Zone 3  \\
% 		\hline
% 		40 &  & Exits Zone 3 and enters Zone 4  \\
% 		\hline
% 		42 &  &  Exits Zone 4 and loads from {\bf WS3} \\
% 		\hline
% 		43 &  &  Re-enters Zone 4 \\
% 		\hline
% 		44 &  & Exits Zone 4 and re-enters Zone 3  \\
% 		\hline
% 		46 &  &  Exits Zone 3, unloads at {\bf WS1} and parks \\
% 		\hline
% 		51 & 5 & Leaves {\bf CPS} and enters Zone 4  \\
% 		\hline
% 		50 &  &  Exits Zone 4 and loads from {\bf WS1} \\
% 		\hline
% 		53 &  &  Re-enters Zone 4 \\
% 		\hline
% 		52 &  &  Exits Zone 4, unloads to {\bf CPS} and parks \\
% 		\hline

% 	\end{tabular}

% \end{table}

%%%%%%%%%%%%%
%%%%%fig





% These specifications are modeled by nine automata shown in Fig.\ref{fig:AGVSPEC} :
% \[
% \textbf{Z}_1, \textbf{Z}_2,\textbf{Z}_3, \textbf{Z}_4, \textbf{WS}_{13}, \textbf{WS}_{14}, \textbf{WS}_{2}, \textbf{WS}_{3}, \textbf{IPS}
% \]

%%%%%fig
% \begin{figure}[t]
% 	\centering

% 	\includegraphics[width=70mm]{fig/AGV_E.jpg}
 	
%  	\label{fig:AGVSPEC}
%   	\caption{Specifications of AGVs, taken from \cite{SUPLOC}}
% \end{figure}

%%%%%
In the following, we apply our proposed 6-step procedure. Due to space limit, details are referred to \cite{longversion}. Specific to Markov clustering, first in Step~2 we need to cluster the nine decentralized supervisors (computed in Step~1 for the nice specifications). To this  end, the following stochastic matrix is constructed: 

% employ this case to illustrative the steps of our proposed method.

% By {\bf Step 1}: We synthesize decentralized supervisors for these nine specifications in the following.
% Let the event set of the specification $\textbf{Z}_1$ be $\Sigma_{\textbf{Z}_1}$.
% Firstly, we obtain the decentralized plant $\textbf{G}_{\textbf{Z}_{1}}$ which is the synchronous product of the \textbf{AGV}s that share events with $\Sigma_{\textbf{Z}_1}$, namely
% $\textbf{G}_{\textbf{Z}_1}:= (\textbf{AGV1}||\textbf{AGV2})$.
% Then we compute the decentralized supervisor $\textbf{SUP}_{\textbf{Z}_1}$ such that 
% \[
% L_m(\textbf{SUP}_{\textbf{Z}_1})=\textrm{sup}\textit{C}(\textbf{Z}_1||L_m(\textbf{G}_{\textbf{Z}_{1}})) 
% \]
% Similarly, we get nine decentralized supervisors 
% \[
% \textbf{SUP}_{\textbf{Z}_1}, \textbf{SUP}_{\textbf{Z}_2}, \textbf{SUP}_{\textbf{Z}_3}, \textbf{SUP}_{\textbf{Z}_4}, \textbf{SUP}_{\textbf{WS}_{13}},
% \]
% \[
% \textbf{SUP}_{\textbf{WS}_{14}}, 
% \textbf{SUP}_{\textbf{WS}_{2}}, \textbf{SUP}_{\textbf{WS}_{3}}, 
% \textbf{SUP}_{\textbf{IPS}}.
% \]
% By {\bf Step 2}: We create a DMM {\bf P} to record the dependencies between models $\textbf{AGV1},..,\textbf{AGV5}$ and nine decentralized supervisors, which is shown below.


% %%%%% table PR  %%%



% \renewcommand{\arraystretch}{1.6}
% \begin{table}[h]
% 	\caption{The DMM {\bf P} of the AGV system. \\ }
% 	\label{table:AGV_DMM}
% 	\centering
%  \setlength{\tabcolsep}{0.9mm}{
% 	\begin{tabular}{c c||c|c|c|c|c|}

% 		 &\ & $\textbf{AGV}_1$ & $\textbf{AGV}_2$& $\textbf{AGV}_3$ & $\textbf{AGV}_4$ & $\textbf{AGV}_5$ \\
% 		\hline
% 		\hline
% 		$\textbf{Z}_1$      & $\textbf{SUP}_{\textbf{Z}_1}$             & 1& 1 & 0 & 0 & 0 \\
% 	\hline
% 		$\textbf{Z}_2$      & $\textbf{SUP}_{\textbf{Z}_2}$             & 0& 1 & 1 & 0 & 0 \\
% 	\hline
% 		$\textbf{Z}_3$      & $\textbf{SUP}_{\textbf{Z}_3}$             & 0& 1 & 0 & 1 & 0 \\
% 	\hline
% 		$\textbf{Z}_4$      & $\textbf{SUP}_{\textbf{Z}_4}$             & 0& 0 & 0 & 1 & 1 \\
% 	\hline
% 		$\textbf{WS}_{13}$ & $\textbf{SUP}_{\textbf{WS}_{13}}$  & 0& 0 & 1 & 0 & 1 \\
% 	\hline
% 		$\textbf{WS}_{14}$ & $\textbf{SUP}_{\textbf{WS}_{14}}$   & 0& 0 & 0 & 1 & 1 \\
% 	\hline
% 		$\textbf{WS}_2$   & $\textbf{SUP}_{\textbf{WS}_{2}}$       & 1& 0 & 1 & 0 & 0 \\
% 	\hline
% 		$\textbf{WS}_3$   & $\textbf{SUP}_{\textbf{WS}_{3}}$       & 0& 1 & 0 & 1 & 0 \\
% 	\hline
% 		$\textbf{IPS}$      & $\textbf{SUP}_{\textbf{IPS}}$             & 1& 1 & 0 & 0 & 0 \\
% 	\hline
%   \end{tabular}}
% \end{table}
% \renewcommand{\arraystretch}{1}
 
% Then, we multiply {\bf P} with its tranpose matrix ${\bf P^\top}$ to get the DSM shown in Table \ref{tab:AGV_DSM}. 

% %%%%%%%table PC

% \renewcommand{\arraystretch}{1.4}

% \begin{table}[H]
% 	\caption{The DSM of the AGV system: ${\bf P_{D}=P\times P^\top}$}
% 	\label{tab:AGV_DSM}
% 	\centering
% 	\begin{tabular}{c||c|c|c|c|c|c|c|c|c|}
	
%  & \rotatebox{90}{$\textbf{SUP}_{\textbf{Z}_1}$}  & \rotatebox{90}{$\textbf{SUP}_{\textbf{Z}_2}$} 
% &\rotatebox{90}{$\textbf{SUP}_{\textbf{Z}_3}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{Z}_4}$}
%  & \rotatebox{90}{$\textbf{SUP}_{\textbf{WS}_{13}}$} 
% & \rotatebox{90}{$\textbf{SUP}_{\textbf{WS}_{14}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{WS}_{2}}$ }
% & \rotatebox{90}{$\textbf{SUP}_{\textbf{WS}_{3}}$} & \rotatebox{90}{$\textbf{SUP}_{\textbf{IPS}}$} \\
%  %\ & \multicolumn{9}{|c|}{\rotatebox{90}{$\textbf{SUP}_{\textbf{Z}_1},...,\textbf{SUP}_{\textbf{IPS}}$}} \\
		
% 		\hline
% 		\hline
% 		 $\textbf{SUP}_{\textbf{Z}_1}$             & 2 & 1 & 1 & 0 & 0 & 0 & 1 & 1 & 2  \\
% 				\hline
%        $\textbf{SUP}_{\textbf{Z}_2}$             & 1 & 2 & 1 & 0 & 1 & 0 & 1 & 1 & 1  \\
% 		\hline
%        $\textbf{SUP}_{\textbf{Z}_3}$             & 1 & 1 & 2 & 1 & 0 & 1 & 0 & 2 & 1  \\
% 		\hline
%        $\textbf{SUP}_{\textbf{Z}_4}$             & 0 &0  & 1 &2  & 1  & 2 &0  & 1 &  0 \\
% 		\hline
%  		 $\textbf{SUP}_{\textbf{WS}_{13}}$  	  &  0&  1& 0 &  1&  2&  1&  1&  0&  0\\
% 		\hline
%  		 $\textbf{SUP}_{\textbf{WS}_{14}}$     &  0&  0&  1&  2&  1&  2&  0&  1& 0  \\
% 		\hline
%    		 $\textbf{SUP}_{\textbf{WS}_{2}}$       &  1&  1&  0&  0&  1&  0&  2&  0&  1 \\
% 		\hline
%    		 $\textbf{SUP}_{\textbf{WS}_{3}}$       &  1&  1&  2&  1&  0&  1&  0&  2&  1 \\
% 		\hline
%        $\textbf{SUP}_{\textbf{IPS}}$             &  2&  1&  1&  0&  0&  0&  1&  1&  2 \\
% 		\hline
%   \end{tabular}
% \end{table}
% %%%%%%%%%% makov  input M %%%%%%%%
% To turn the DSM ${\bf P_{D}}$ into a probability matrix $\textbf{M}$ for the clustering step, we do the column normalization. The result is:

\[
\textbf{M} = \left(
\begin{smallmatrix}
	0.2500  &  0.1250  &  0.1111     &    0          &    0          &    0            & 0.1667     &  0.1111     &  0.2500 \\
    0.1250  &  0.2500  &  0.1111     &      0       & 0.1667     &       0         &  0.1667    &  0.1111    &   0.1250 \\
    0.1250  &  0.1250  &  0.2222    &  0.1429   &     0          &   0.1429   &      0         & 0.2222      & 0.1250 \\
         0     &    0        & 0.1111        & 0.2857  &  0.1667    &  0.2857     &    0          & 0.1111      &      0 \\
         0   & 0.1250     &    0          &  0.1429    & 0.3333     &  0.1429     &  0.1667   &       0        &   0 \\ 
         0     &    0         & 0.1111      & 0.2857   &  0.1667     & 0.2857    &     0           &  0.1111   &      0 \\
    0.1250 &   0.1250    &     0        &     0        &   0.1667    &     0     &  0.3333         &     0         &  0.1250  \\
    0.1250 &   0.1250  &  0.2222    & 0.1429    &     0         &  0.1429     &    0           &  0.2222    &  0.1250  \\ 
    0.2500  &  0.1250  &  0.1111     &    0        &   0            &   0            & 0.1667     &  0.1111    &  0.2500 \\
\end{smallmatrix}
\right).
\]

\renewcommand{\arraystretch}{1}

%%%%%% if=3

This {\bf M} is used as the input of the Markov clustering algorithm. While we fix parameter $\alpha=2$, the parameter $\beta$ is varied for different values ($2.5 \sim 10$) as shown in Table~I. Observe that larger $\beta$ results in more clusters (with fewer decentralized supervisors in each cluster). The third column in Table~I shows that for all tried values of $\beta$, there is only one higher-level coordinator needs to be computed to ensure global nonblocking behavior; however, small values of $\beta$ cause the coordinator to have larger state sizes. 
% \footnote{Here we show different values of $\beta$ is for the purpose of illustrating the role this single parameter plays. When we use our proposed approach, we simply fix an arbitrary value for $\beta$, run our 6-step algorithm, and obtain a set of supervisors and coordinators. If we are unsatisfied with the obtained result (say some coordinator has very big state size), then we know that $\beta$ should be increased and run the 6-step algorithm again, such that the result may be improved.} 
{\color{blue} On the other hand, larger values of $\beta$ often require more execution times of the algorithm (see the fourth column of Table~I),\footnote{Time is measured on a personal computer with i7 CPU and 8G memory.} as more layers of computations are needed.}

% 13.164429
% 17.937868
% 17.876168
% 19.11998
% 24.805674
% 30.13544
% 22.142875
% 22.069978
% 22.224776
% 22.581423
% 22.220457
% 90.649986
% 98.517249
% 106.298754
% 115.80526
% 123.900985


\renewcommand{\arraystretch}{0.8}
\begin{table}[H]
    \centering
    \caption{Tuning parameter $\beta$ for different clusters}
\label{tab:AGV_beta}
    %\scalebox{0.8}{
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        
        \begin{tabular}{c}
          $\beta$
        \end{tabular}
        &  
        \begin{tabular}{c}
          Numbers of clusters for\\
           decentralized supervisors
        \end{tabular}
        &
        \begin{tabular}{c}
           
          Coordinator\\
        (state size)
        \end{tabular}
        &
        \begin{tabular}{c}
           
          {\color{blue} Execution}\\
        {\color{blue} time [s]}
        \end{tabular}\\
        \hline
        \hline
        2.5  & 2&  $\textbf{CO}$ (64) & {\color{blue} 13.164} \\
        \hline
		3    & 3 & $\textbf{CO}$ (51) & {\color{blue} 17.938} \\
         \hline
		3.5  &  3 & $\textbf{CO}$ (27) & {\color{blue} 17.876} \\
        \hline
		4    &  4 & $\textbf{CO}$ (10) & {\color{blue} 19.120} \\
  \hline
		4.5  & 4 & $\textbf{CO}$ (10) & {\color{blue} 24.806} \\
  \hline
		5    & 4 & $\textbf{CO}$ (10) & {\color{blue} 30.135} \\
  \hline
		5.5  &5 &  $\textbf{CO}$  (10) & {\color{blue} 22.143} \\
  \hline
		6    & 5 & $\textbf{CO}$ (10) & {\color{blue} 22.070}\\
  \hline
		6.5  & 5  &  $\textbf{CO}$ (10) & {\color{blue} 22.225} \\
  \hline
		7    & 5  &  $\textbf{CO}$ (10) & {\color{blue} 22.581} \\
  \hline
    	7.5  &  5 &  $\textbf{CO}$ (10) & {\color{blue} 22.220} \\
     \hline
		8    &6  & $\textbf{CO}$ (10) & {\color{blue} 90.650}  \\
  \hline
		8.5  & 6  & $\textbf{CO}$ (10) & {\color{blue} 98.517}  \\
  \hline
		9    & 6 & $\textbf{CO}$ (10) & {\color{blue} 106.299}  \\
  \hline
		9.5  & 6 & $\textbf{CO}$ (10) & {\color{blue} 115.805}   \\
  \hline
		10   &  6 & $\textbf{CO}$ (10) & {\color{blue} 123.901}  \\

        \hline
    \end{tabular}
    %}
\end{table}


As an example, consider $\beta = 4$. The resulting $4$ clusters of decentralized supervisors are shown in Table~II. Also the 10-state higher-level coordinator is displayed in Fig.~\ref{fig:AGVco10}.\footnote{In \cite{Feng2008} by detailed analysis of the structure of the AGV system, a higher-level coordinator of 7 states is found. Our automatically resulted coordinator is fairly close to the handcrafted one in \cite{Feng2008}.} 
%解释4和4以上的话第二层以上cluster数量不会减少
%and the clustering result diverge from 4. 
%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.5}
\begin{table}[h]
	\centering
 \caption{Clusters of decentralized supervisors ($\beta = 4$)}
\label{tab:AGV_C}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Cluster 1 &Cluster 2&Cluster 3 &Cluster 4\\
		\hline
		\hline
		$\textbf{SUP}_{\textbf{WS}_{13}}$ & $\textbf{SUP}_{\textbf{Z}_4}$ & $\textbf{SUP}_{\textbf{Z}_3}$ & $\textbf{SUP}_{\textbf{Z}_1}$ \\
		                                                          & $\textbf{SUP}_{\textbf{WS}_{14}}$ & $\textbf{SUP}_{\textbf{WS}_{3}}$ & $\textbf{SUP}_{\textbf{Z}_2}$\\
		                                                            &                                                &                                                          & $\textbf{SUP}_{\textbf{WS}_{2}}$ \\
		                                                           &                                                &                                                           &  $\textbf{SUP}_{\textbf{IPS}}$\\
		\hline
	\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}
%%%%%%%%%%%%%%%



%%%%%fig
% \begin{figure}[H]
% 	\centering

% 	\includegraphics[width=80mm]{fig/CLS=4.jpg}
% 	\caption{Control architecture resulted from our approach} 	
%  	\label{fig:AGVcls4}
% \end{figure}

% By {\bf Step 3}: The components of each cluster are combined using synchronous product to create the subsystem model {\bf SUB}, namely: 
% %%%%%%%%%%%%
% \begin{itemize}
% \item $\textbf{SUB}_1 = \textbf{SUP}_{\textbf{WS}_{13}}$
% \item $\textbf{SUB}_2 =\textbf{SUP}_{\textbf{Z}_4} || \textbf{SUP}_{\textbf{WS}_{14}}$
% \item $\textbf{SUB}_3 =\textbf{SUP}_{\textbf{Z}_3} || \textbf{SUP}_{\textbf{WS}_{3}}$
% \item $\textbf{SUB}_4 =\textbf{SUP}_{\textbf{Z}_1} || \textbf{SUP}_{\textbf{Z}_2} || \textbf{SUP}_{\textbf{WS}_{2}}|| \textbf{SUP}_{\textbf{IPS}} $
% \end{itemize}

% We check the nonblokingness inside of each subsystem and design the coordinator supervisor if conflict exists. 
% The subsystems $\textbf{SUB}_{1},\textbf{SUB}_{2},\textbf{SUB}_{3},\textbf{SUB}_{4}$ are nonblocking, so there is no need to design coordinator to remove the conflict inside each subsystem.

% By {\bf Step 4}: Then we perform the subsystem abstraction of each subsystem and obtain $\textbf{ABS}_{1},\textbf{ABS}_{2},\textbf{ABS}_{3},\textbf{ABS}_{4}$. We employ the synthesis procedure of $\textbf{SUB}_{1}$ to introduce this step. 
% Firstly, the shared event set $\Sigma_o$ of the four subsystems is given by
% \[
% \Sigma_o := \{\sigma\in\Sigma | \sigma\in (\Sigma_{\textbf{SUB}_1}\cap\Sigma_{\textbf{SUB}_2}\cap\Sigma_{\textbf{SUB}_3}\cap\Sigma_{\textbf{SUB}_4}) \},
% \]
% where $\Sigma_{\textbf{SUB}_i}$ is the event set of $\textbf{SUB}_i$ for $i\in [1,4]$.
% Let $\Sigma_{\textbf{ABS}_1}$ be the event set of $\textbf{ABS}_1$. Then we get that $\Sigma_{\textbf{ABS}_1} := \Sigma_o \cap \Sigma_{\textbf{SUB}_1}$. 
% $\textbf{ABS}_{1}$ thus can be generated by a natural projection $\textit{P}_1 : \Sigma_{\textbf{SUB}_1}^{\ast} \rightarrow \Sigma^{\ast}_{\textbf{ABS}_1} $.
% Check and extend $\textit{P}_1$ to ensure $\textit{P}_1$ satisfies the natural observer and OCC. 

% %%%第二次MCL

% Return back to {\bf Step 2}: We perform the clustering again for the four abstractions $\textbf{ABS}_{1},...,\textbf{ABS}_{4}$ and five plant components $\textbf{AGV1},...,\textbf{AGV5}$. Construct a new DMM {\bf P} to record the dependencies between abstractions and plant components. The matrices {\bf P}, $\textbf{P}_D$ and {\bf M} for this second level clustering are shown below.


% \renewcommand{\arraystretch}{1.3}
% \begin{table}[H]
% 	\caption{The DMM {\bf P} of the {\bf AGVs} and abstractions \\ }
% 	\label{table:AGV_DMM_layer2}
% 	\centering
% 	\begin{tabular}{c||c|c|c|c|c|}

% 		 \ & $\textbf{AGV}_1$ & $\textbf{AGV}_2$& $\textbf{AGV}_3$ & $\textbf{AGV}_4$ & $\textbf{AGV}_5$ \\
% 		\hline
% 		\hline
%     $\textbf{ABS}_{1}$             & 0& 0 & 1 & 0 & 1 \\
% 	\hline
%      $\textbf{ABS}_{2}$             & 0& 0 & 0 & 1 & 1 \\
% 	\hline
%       $\textbf{ABS}_{3}$             & 0& 1 & 0 & 1 & 0 \\
% 	\hline
% 	 $\textbf{ABS}_{4}$             & 1& 1 & 1 & 0 & 0 \\
% 	\hline
%   \end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}
% %%%
% %%%DSM layer2
% \renewcommand{\arraystretch}{1.3}
% \begin{table}[H]
% 	\caption{ ${\bf P_{D}=P\times P^\top}$ }
% 	\label{table:AGV_DMM_layer2}
% 	\centering
% 	\begin{tabular}{c||c|c|c|c|}

% 		 \ &  $\textbf{ABS}_{1}$  &  $\textbf{ABS}_{2}$  &  $\textbf{ABS}_{3}$  &  $\textbf{ABS}_{4}$  \\
% 		\hline
% 		\hline
%     $\textbf{ABS}_{1}$             & 2& 1 & 0 & 1  \\
% 	\hline
%      $\textbf{ABS}_{2}$             & 1& 2 & 1 & 0  \\
% 	\hline
%       $\textbf{ABS}_{3}$             & 0& 1 & 2 & 1  \\
% 	\hline
% 	 $\textbf{ABS}_{4}$             & 1& 0 & 1 & 3  \\
% 	\hline
%   \end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}

% %%%%%%% M
% \[
% \textbf{M} = \left(
% \begin{array}{cccc}
%      0.50 & 0.25 & 0 & 0.20 \\
%      0.25 & 0.50 & 0.25 & 0 \\
%      0 & 0.25 & 0.50 & 0.20 \\
%      0.25 & 0 & 0.25 & 0.60 \\
% \end{array}
% \right)
% \]
% %%%

% Then we apply the clustering algorithm again using the same $\beta(=4)$. 
% \renewcommand{\arraystretch}{1.3}
% \begin{table}[H]
% \label{tab:AGV_ABS_C}
% 	\centering
% 	\begin{tabular}{|c|c|c|c|}
% 		\hline
% 		Cluster 1 &Cluster 2& Cluster 3 & Cluster 4 \\
% 		\hline
% 		\hline
% 		$\textbf{ABS}_{1}$ & $\textbf{ABS}_{2}$ &$\textbf{ABS}_{3}$  & $\textbf{ABS}_{4}$ \\
% 		\hline
%   \end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}

% As shown above, the cluster number does not reduce compared to the previous clustering. Therefore, we reduce $\beta$ value by 0.5 (i.e. $\beta = 3.5$), and show the result in the following.
% \renewcommand{\arraystretch}{1.4}
% \begin{table}[H]
% \label{tab:AGV_ABS_C}
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Cluster 1 &Cluster 2\\
% 		\hline
% 		\hline
% 		$\textbf{ABS}_{2}$ & $\textbf{ABS}_{1}$\\
%   		                                 &$\textbf{ABS}_{3}$\\
%   		                                 &$\textbf{ABS}_{4}$\\
% 		\hline
% 	\end{tabular}
% \end{table}
% \renewcommand{\arraystretch}{1}
% By {\bf Step 3}: After the new clustering, we get 2 new clusters in this upper layer. 
% Specifically, there is only one abstraction in cluster 1, so $\textbf{ABS}_{2}$ is the new subsystem directly.
% For cluster 2, however, there are three abstractions ${\bf ABS}_1$, ${\bf ABS}_3$, ${\bf ABS}_4$. We thus get a new subsystem for cluster 2 by the synchronous product of these three abstractions, i.e., 
% \begin{itemize}
% \item $\textbf{SUB}_{layer2,1} = \textbf{ABS}_{2}$
% \item $\textbf{SUB}_{layer2,2} =\textbf{ABS}_{1} || \textbf{ABS}_{3} || \textbf{ABS}_{4}$
% \end{itemize}
% Check possible conflict inside $\textbf{SUB}_{layer2,1}, \textbf{SUB}_{layer2,2}$ and get that they are nonblocking. 



%%%%%

% Our result consists of nine decentralized supervisors $\textbf{SUP}_{\textbf{Z}_1},$
% $\textbf{SUP}_{\textbf{Z}_2},$
% $\textbf{SUP}_{\textbf{Z}_3},$
% $\textbf{SUP}_{\textbf{Z}_4},$
% $\textbf{SUP}_{\textbf{WS}_{13}},$
% $\textbf{SUP}_{\textbf{WS}_{14}},$
% $\textbf{SUP}_{\textbf{WS}_{2}},$ 
% $\textbf{SUP}_{\textbf{WS}_{3}},$
% $\textbf{SUP}_{\textbf{IPS}}$, and one coordinator {\bf CO}.
% For the initial parameter $\beta=4$, the resulting control architecture has two abstraction levels, in which the coordinator $\textbf{CO}$ has 10 states.
% % infl=4 table
% \begin{table}[H]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{|c|c|c|c|}
%     \hline
        
%         \begin{tabular}{c}
%           $\beta$
%         \end{tabular}
%         &  
%         \begin{tabular}{c}
%           Cluster numbers of\\
%            decentralized supervisor
%         \end{tabular}
%         &
%         \begin{tabular}{c}
%           The number of\\
%          abstraction levels 
%         \end{tabular}
%         & 
%         \begin{tabular}{c}
           
%           Coordinator\\
%           (state numbers)
%         \end{tabular}\\
%         \hline
%         \hline
%          4    & 4&2& $\textbf{CO}$ (10)\\

%         \hline
%     \end{tabular}
%     }
%     \label{tab:AGV_inf4}
% \end{table}



%  %the monolithic supervisor {\bf SUP} (4406 states) is computable. 
%  For this AGV system, the standard centralized approach is still possible. The monolithic supervisor \textbf{SUP} has 4406 states.
% So we can confirm that the joint behavior of the supervisors and the coordinator is the same as the monolithic controlled behavior, i.e.,
% \[
% \textbf{SUP}_{\textbf{Z}_1}|| ... ||\textbf{SUP}_{\textbf{IPS}}||\textbf{CO} = \textbf{SUP}
% \]




% We change the clustering {\it inflation} $\beta$ and find that the number of cluster increases as $\beta$ increases.
% %%%
% The following table is the result obtained based on the assumption $ 2.5\leq\beta\leq 10$, which includes the number that the decentralized supervisors are clustered, the number of abstraction, and the state number of the coordinator.
% %
% \renewcommand{\arraystretch}{0.8}
% \begin{table}[H]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{|c|c|c|c|}
%     \hline
        
%         \begin{tabular}{c}
%           $\beta$
%         \end{tabular}
%         &  
%         \begin{tabular}{c}
%           Cluster numbers for\\
%            decentralized supervisor
%         \end{tabular}
%         &
%         \begin{tabular}{c}
%           The number of\\
%          abstraction 
%         \end{tabular}
%         & 
%         \begin{tabular}{c}
           
%           Coordinator\\
%           (state numbers)
%         \end{tabular}\\
%         \hline
%         \hline
%         2.5  & 2&  1 & $\textbf{CO}$ (64) \\
%         \hline
% 		3    & 3&  2 & $\textbf{CO}$ (51) \\
%          \hline
% 		3.5  &  3& 2 & $\textbf{CO}$ (27) \\
%         \hline
% 		4    &  4& 2 & $\textbf{CO}$ (10) \\
%   \hline
% 		4.5  & 4&  2 & $\textbf{CO}$ (10) \\
%   \hline
% 		5    & 4&  2 & $\textbf{CO}$ (10) \\
%   \hline
% 		5.5  &5& 3 &  $\textbf{CO}$  (10) \\
%   \hline
% 		6    & 5 &3 & $\textbf{CO}$ (10)\\
%   \hline
% 		6.5  & 5 & 3 &  $\textbf{CO}$ (10) \\
%   \hline
% 		7    & 5 & 3 &  $\textbf{CO}$ (10) \\
%   \hline
%     	7.5  &  5& 3 &  $\textbf{CO}$ (10) \\
%      \hline
% 		8    &6 & 3 & $\textbf{CO}$ (10)   \\
%   \hline
% 		8.5  & 6 & 3 & $\textbf{CO}$ (10)   \\
%   \hline
% 		9    & 6 &3 & $\textbf{CO}$ (10)   \\
%   \hline
% 		9.5  & 6& 3 & $\textbf{CO}$ (10)   \\
%   \hline
% 		10   &  6& 3 & $\textbf{CO}$ (10)  \\

%         \hline
%     \end{tabular}
%     }
%     \label{tab:AGV_inf2.5-10}
% \end{table}



% {\bf Comparison of coordinators }
% %%%%%fig
% %如上表，从infl4-10的13个CO都是iso的，接下来我们将这个10个状态数的CO写作从（10）。
% %我们把co（10）与手法【】中的7个状态数的CO（7）进行一个简短的比较。co10和CO7的自动机图分别是
% %两个自动机的说明

% As shown in Table~\ref{tab:AGV_inf2.5-10}, there are 13 coordinators having 10 states for inflation $\beta=4$  to $\beta=10$. 
% It is verified that these 13 coordinators are isomorphic. 
% The coordinator $\textbf{CO}_{(10)}$ is shown in Fig.\ref{fig:AGVco10}. 
% On the other hand, relying on engineering insight for system decomposition, it is known that the coordinator $\textbf{CO}_{(7)}$ for the same AGV system designed by the approach in \cite{Feng2008} has 7 states which is shown in Fig.4.5.
% We now make a brief comparison between $\textbf{CO}_{(7)}$ and $\textbf{CO}_{(10)}$.
% %%%%%
% %%%%%fig
% \begin{figure}[H]
% 		\centering
% 	\includegraphics[width=80mm]{Fig1.pdf}
%  	\label{fig:AGVco7}
%   	\caption{7-state coordinator by approach in \cite{Feng2008}}
% \end{figure}

%%%%%
%%%%%fig
\begin{figure}[H]
	\centering

	\includegraphics[width=80mm]{Fig2.pdf}
	\caption{10-state coordinator {\bf CO} ($\beta = 4$)}
 	\label{fig:AGVco10}
\end{figure}
%
%%%%%

Finally it is confirmed that the joint behavior of the 10-state coordinator and the nine decentralized supervisors is not only nonblocking, but also in this case maximally permissive (thus equivalent to the controlled behavior of the monolithic supervisor). Therefore for this case study, our fully automated approach successfully solve the nonblcoking hierarchical control problem and moreover the resulting coordinator is fairly simple (the derivation of which does not need knowing or analysis of system's structure).

% The control logic of $\textbf{CO}_{(7)}$ is: \\
% 1. Disable event 11 ($\textbf{AGV1}$ leaves $\textbf{WS2}$ and enters Zone 1) if event 13 ($\textbf{AGV1}$ re-enters Zone 1) has occurred three more times than event 23 ($\textbf{AGV2}$ re-enters Zone 1). \\
% 2. Disable event 21 ($\textbf{AGV2}$ leaves $\textbf{WS3}$ and enters Zone 3) if event 23 has occurred three more times than event 13.
% %

% The control logic of $\textbf{CO}_{(10)}$ is: \\
% 1. Disable event 11 if event 11 has occurred three more times than event 23.\\
% %这里写对第一的比较。为什么11和13一样
% This first control logic of $\textbf{CO}_{(10)}$ is the same as $\textbf{CO}_{(7)}$.
% The reason is that for the automaton of $\textbf{AGV1}$ shown in Fig.\ref{fig:AGVplant}, 
% events 11 and 13 can only occur cyclically, so observing event 11 is equivalent to observing event 13 for the purpose of controlling 11.\\
% %11和13的区别
% %
% 2. Disable event 21 if event 23 has occurred three more times than event 11.

%%%%%%%%%%%
%这里需要观察比原先更多的event，显示比如每次在执行21前zone3都是空的（40，42，43，46）
%在CO10的受理语言中 同时，我们会观察到有关AGV4的event。在执行23（AGv2进入zone3前最后一个可控event）或者21（）之前，zone3都显示是空的（只会出现44和41以外的），但是对zone3的控制对全局无冲突无关，由于只要对WS3的控制到位了，zone4也是无冲突的。

%First by the same reason as above, observing event 11 is equivalent to observing event 13 for the control of 21. In addition, $\textbf{CO}_{(10)}$ observes more for the events of \textbf{AGV4} than $\textbf{CO}_{(7)}$   (e.g. event 40 (\textbf{AGV4} exits Zone 3 and enters Zone 4), event 42 (\textbf{AGV4} exits Zone 4 and loads from {\bf WS3}), event 43 (\textbf{AGV4} re-enters Zone 4), and event 46 (\textbf{AGV4} exits Zone 3, unloads at {\bf WS1} and parks)). These events show that $\textbf{AGV4}$ is not in Zone 3 before event 21 occurs (\textbf{AGV2} leaves $\textbf{WS3}$ and enters Zone 3). Since only $\textbf{AGV2}$ and $\textbf{AGV4}$ can enter Zone 3, no more than one \textbf{AGV} occupies Zone 3.  But this control logic is in fact redundant because  the decentralized supervisor $\textbf{SUP}_{\textbf{Z}_3}$ already ensures it. 
%%
%%
\begin{comment}

\renewcommand{\arraystretch}{0.7}
\begin{table}[H]
\label{tab:AGV_infl}
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		{\it inflation} $\beta$ & Cluster numbers  & {\bf CO} State numbers\\
		value  & of decentralized supervisor& \\
		\hline
	%	2         &   1 &  64 \\
		2.5  &   2 &  64 \\
		3    &   3 &  51 \\
		3.5  &   3 &  27 \\
		4    &   3 &  10 \\
		4.5  &   3 &  10 \\
		5    &   3 &  10 \\
		5.5  & 5 &    10 \\
		6    & 5 &  10\\
		6.5  & 5 &   10 \\
		7    & 5 &   10 \\
    	7.5  & 5 &   10 \\
		8    & 6 & 10   \\
		8.5  & 6 & 10   \\
		9    & 6 & 10   \\
		9.5  & 6 & 10   \\
		10   & 6 & 10  \\
		%8      &      &    \\
		\hline
	\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

Since $\textbf{WS1}$ needs to wait for part Type1 and part Type2 to exist at the same time before they can be assembled, part Type1 in $\textbf{WS1}$ will be placed until part Type2 arrives in $\textbf{WS1}$. Since there is only one $\textbf{AGV1}$, if event 13 has occurred three more times than event 23, or event 11 has occurred three more times than event 23 and still executed 11 again, the following result will be achieved: four parts Type1 will exist in $\textbf{IPS1}$, $\textbf{WS2}$, Zone 2 and $\textbf{WS1}$. 
Since only one of $\textbf{AGV1}$, $\textbf{AGV2}$ can be loaded at a time in two input stations $\textbf{IPS1}$, $\textbf{IPS2}$, $\textbf{AGV2}$ needs to wait for part Type1 to be shipped out of $\textbf{IPS1}$ by $\textbf{AGV1}$,  but this will cause $\textbf{WS2}$ to overflow.
Therefore, although $\textbf{CO}_{(10)}$ differs from $\textbf{CO}_{(7)}$
in that $\textbf{CO}_{(10)}$ disables event 11 by observing 11 instead of 13, we can say that he first control logic of $\textbf{CO}_{(10)}$ is the same as $\textbf{CO}_{(7)}$ which protects $\textbf{WS2}$ from overflow.\\
\end{comment}

==> tex/Chapter4_case_TAGV.tex <==
\subsection{Timed Automatic Guided Vehicles}
%预想：1写加了时间限制后总体的状态数变化2三个时间轴的结果，第三种就无法计算了。
%

The timed-AGV(TAGV) system structure and the control specifications are the same as in Sec.\ref{sec:AGV} shown in Fig.\ref{fig:AGVworkcell} and Fig.4.3. The only change we make is to set time bounds for all events of the five AGVs, as shown in the following Table.\ref{table:TAGVe_time}.
%
%%%%%%%%%%%%%%%%%
%%%%%Time bound 

\begin{table}[H]
 	\caption{Time bounds of events }
	\label{table:TAGVe_time}
	\centering
     \scalebox{0.7}{
	\begin{tabular}{ l|c|c|c}
		\hline\hline
       \multirow{2}{*}{\textbf{AGV}} & \multirow{2}{*}{Event} & \multicolumn{2}{c}{Time bound}\\
        \cline{3-4} 
		&  & Lower & Upper \\
		\hline
		1 & 11 & 0 &  $\infty$ \\
		\hline
		& 10 & 0 & 1  \\
		\hline
		&13 & 0 & $\infty$  \\
		\hline
		&12 &  0&  1 \\
		\hline
		2 & 21 & 0 & $\infty$ \\
		\hline
		&18 & 0 & 1 \\
		\hline
		&20 & 0 &  1 \\
		\hline
		&22 & 0 & 1  \\
		\hline
		&23 & 0 & $\infty$  \\
		\hline
		&24 & 0 &  1 \\
		\hline
		&26 & 0 &  1 \\
		\hline
		&28 & 0 &  1\\
		\hline
		3 &31 & 0 &  $\infty$ \\
		\hline
		&32 & 0 &  1 \\
		\hline
		&33 & 0 & $\infty$ \\
		\hline
		&34 & 0 & 1 \\
		\hline
		4 &41 & 0 & $\infty$  \\
		\hline
		&40 & 0 &  1 \\
		\hline
		&42 & 0 & 1 \\
		\hline
		&43 & 0 & $\infty$ \\
		\hline
		&44 & 0 &  1 \\
		\hline
		&46 & 0 &  1 \\
		\hline
		5 &51 & 0 & $\infty$ \\
		\hline
		&50 & 0 & 1  \\
		\hline
		&53 & 0 & $\infty$ \\
		\hline
		&52 & 0 & 1  \\
		\hline

	\end{tabular}
    }
\end{table}

The five AGV models explicitly incorporating the $tick$ transition are shown in Fig.\ref{fig:TAGVplant}.
\begin{figure}[H]
	\centering

	\includegraphics[width=150mm]{fig/TAGVplant.jpg}
\caption{Plant components of TAGV}
 	\label{fig:TAGVplant}
\end{figure}
%
The forcible events set $\Sigma_{for}$ of TAGV is
\[
\Sigma_{for}= \{ 11,13,21,23,31,33,41,43,51,53 \}
\]
%
%
We apply our proposed method to TAGV.
The difference from AGV is that we obtain the decentralized plant by $composition$ introduced in Sec.2.4.1 instead of the normal synchronous product.
For example, the decentralized plant $\textbf{G}_{\textbf{Z}_{1}}$ for specification ${\bf Z}_1$ is the composition of the AGVs that share events with $\Sigma_{\textbf{Z}_1}$, i.e.
\[
\textbf{G}_{\textbf{Z}_1}:= \textbf{compose}(\textbf{AGV1},\textbf{AGV2})
\]
Based on ${\bf G}_{{\bf Z}_1}$ we compute the decentralized supervisor $\textbf{SUP}_{\textbf{Z}_1}$ such that 
\[
L_m(\textbf{SUP}_{\textbf{Z}_1})=\textrm{sup}\textit{C}(\textbf{Z}_1||L_m(\textbf{G}_{\textbf{Z}_{1}})) 
\]
By the same steps, we get nine decentralized supervisors 
\[
\textbf{SUP}_{\textbf{Z}_1}, \textbf{SUP}_{\textbf{Z}_2}, \textbf{SUP}_{\textbf{Z}_3}, \textbf{SUP}_{\textbf{Z}_4}, \textbf{SUP}_{\textbf{WS}_{13}},
\]
\[
\textbf{SUP}_{\textbf{WS}_{14}}, 
\textbf{SUP}_{\textbf{WS}_{2}}, \textbf{SUP}_{\textbf{WS}_{3}}, 
\textbf{SUP}_{\textbf{IPS}}
\]
For TAGV, the following table is the result of $ 2.5\leq\beta\leq 10$ which includes the cluster numbers of decentralized supervisors and the state numbers of coordinator.
\renewcommand{\arraystretch}{0.8}
\begin{table}[H]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{|c|c|c|c|}
    \hline
        
        \begin{tabular}{c}
          $inflation$ $\beta$ \\
          value
        \end{tabular}
        &  
        \begin{tabular}{c}
          Cluster numbers of\\
           decentralized supervisor
        \end{tabular}
        &
        \begin{tabular}{c}
          The number of\\
         abstraction level 
        \end{tabular}
        & 
        \begin{tabular}{c}
           
          Coordinator (state numbers)
        \end{tabular}\\
        \hline
        \hline
        2.5  & 2&  1 & $\textbf{CO}$ (84) \\
        \hline
		3    & 3&  2 & $\textbf{CO}$ (84) \\
         \hline
		3.5  &  3& 2 & $\textbf{CO}$ (27) \\
        \hline
		4    &  4& 2 & $\textbf{CO}$ (10) \\
  \hline
		4.5  & 4&  2 & $\textbf{CO}$ (10) \\
  \hline
		5    & 4&  2 & $\textbf{CO}$ (10) \\
  \hline
		5.5  &5& 3 &  $\textbf{CO}$  (10) \\
  \hline
		6    & 5 &3 & $\textbf{CO}$ (10)\\
  \hline
		6.5  & 5 & 3 &  $\textbf{CO}$ (10) \\
  \hline
		7    & 5 & 3 &  $\textbf{CO}$ (10) \\
  \hline
    	7.5  &  5& 3 &  $\textbf{CO}$ (10) \\
     \hline
		8    &6 & 3 & $\textbf{CO}$ (10)   \\
  \hline
		8.5  & 6 & 3 & $\textbf{CO}$ (10)   \\
  \hline
		9    & 6 &3 & $\textbf{CO}$ (10)   \\
  \hline
		9.5  & 6& 3 & $\textbf{CO}$ (10)   \\
  \hline
		10   &  6& 3 & $\textbf{CO}$ (10)  \\

        \hline
    \end{tabular}
    }
    \label{tab:TAGV_inf2.5-10}
\end{table}
%这个系统的单个SUP也是可算的，所有的co都是经过了验算，10状态的co都一样。
For this TAGV system, the monolithic supervisor {\bf SUP} is also computable, which has 14744 states.
So we can confirm the joint behavior of the supervisors and the coordinator is the same as the monolithic controlled behavior. Namely :
\[
\textbf{SUP}_{\textbf{Z}_1}|| ... ||\textbf{SUP}_{\textbf{IPS}}||\textbf{CO} = \textbf{SUP}
\]
 Observe that there are 13 coordinators having 10 states for inflation $\beta$
values from 4 to 10. 
It is verified that these 13 coordinators are identical.
%%%%%fig
\begin{figure}[H]
	\centering

	\includegraphics[width=100mm]{fig/TAGV_CO10.jpg}
	\caption{10-state coordinator by our approach}
 	\label{fig:TAGVco10}
\end{figure}
%
The 10-state coordinator is shown in Fig.\ref{fig:TAGVco10}.
Observe that there is no $tick$ event in this coordinator. This means that the conflict-resolving logic of the coordinator is not time related.

==> tex/Conclusions.tex <==
\chapter{Conclusions}

This thesis has proposed a streamlined algorithm for heterarchical supervisory control that automatically conducts horizontal decomposition and vertical aggregation and achieve global nonblocking. 
Our algorithm combines the horizontal decomposition by clustering approach with the vertical abstraction-based approach. 
Our algorithm needs only three inputs: plant component models, specifications models, and a clustering parameter. Without any engineering insight into system structure, the outputs are decentralized supervisors and coordinators whose joint behavior is proved to be nonblocking. 
Moreover, we have demonstrated the effectiveness of our proposed approach on several large-scale benchmark examples.
In our ongoing work, we aim to generalize our approach to extended finite state machine models and systems with only partial observations. We are also going to apply this approach to real systems with a large number of components.

==> tex/old_proof_20220201.tex <==
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem*{thm*}{Theorem}
\newtheorem{prop}{Proposition}
\theoremstyle{definition}
\newtheorem{dfn}{Definition}
%%%%proof:
Using the above procedure, we obtain $I$ decentralized supervisors 
$\textbf{SUP}_1,...,\textbf{SUP}_I$ and $H$ coordinators (the number of coordinators is case-dependent). 
We conclude that the synchronized behavior of these supervisors and coordinators is identical to the behavior of the monolithic supervisor \textbf{SUP}.
%%%%%
%Your theorem statement is wrong. You only considered Natural observer and OCC for SUB. You are right if there is only one-level up in the hierarchy. Namely if you do clustering only once. But in general you need to do clustering many times to produce multi-level abstractions. So Natural Observer and OCC properties must hold for all ABS in all levels.
%%%5

\begin{thm}\label{thm1}

Suppose that the proposed procedure terminates after $L (\geq 1)$ levels of clustering/abstraction, and in each level $l \in \{1,\ldots,L\}$ there are $N_l$ clusters ${\bf SUB}_{n_l}$ ($n_l \in \{1,\ldots,N_l\}$). Assume that the procedure generates $I$ decentralized supervisors ${\bf SUP}_i$ $(i \in \{1, \ldots, I\})$ and $H$ coordinators ${\bf CO}_h$ $(h \in \{1, \ldots, H\})$. If for every $l \in \{1,\ldots,L\}, n_l \in \{1,\ldots,N_l$, $P_{n_l}$ is an $L_m({\bf SUB}_{n_l})$-observer and OCC for $L_m({\bf SUB}_{n_l})$, then


\begin{eqnarray}
%||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))= 
%\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}\\
%(||_{i\in I} \textbf{SUP}_i)|| (||_{w\in W}\textbf{CO}_w)=\textbf{SUP}
(||_{i\in I} L(\textbf{SUP}_i)) || (||_{h\in H}L(\textbf{CO}_h)) || L(\textbf{G})=L(\textbf{SUP})\\
(||_{i\in I} L_m(\textbf{SUP}_i)) || (||_{h\in H}L_m(\textbf{CO}_h)) || L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\end{thm}




%有w层，经过几次抽象化以后的CO，也能去除底层DESUP的冲突。NATOB和OCC的连锁性？

Theorem \ref{thm1} asserts that decentralized supervisors and coordinators designed using our proposed method jointly achieve global optimal and nonblocking controlled behavior. 
%%%开始证明
%
%%
To prove Theorem \ref{thm1}, we need the following proposition from \cite{Feng2008}:
%sub先定义，然后证明我们的sub里面就是sup的组合，sup组合的话已经被证明
\begin{prop}[\cite{Feng2008}]\label{prop1}
Consider decentralized supervisors $\textbf{SUP}_i(i\in I)$  and $H$ coordinators ${\bf CO}_h$ $(h \in \{1, \ldots, H\})$  based on abstractions. If for every $i \in I$, 
$P_i$ is an $Lm(\textbf{SUP}_i)$-observer and OCC for $L_m(\textbf{SUP}_i)$, then
\footnotesize
\begin{eqnarray}
(||_{i\in I} L(\textbf{SUP}_i)) ||(||_{h\in H}L(\textbf{CO}))= 
\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||L_m(\textbf{CO})}\\
||_{i\in I} L(\textbf{SUP}_i) ||L(\textbf{CO})||L(\textbf{G})=L(\textbf{SUP})\\
||_{i\in I} L_m(\textbf{SUP}_i) ||L_m(\textbf{CO})||L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\normalsize
\end{prop}
%$\textbf{SUB}_{n} = ||(\textbf{SUP}_i|i\in CLS_n)$ and\\
%
%By Proposition \ref{prop1}, we can easily say that T coordinators $\textbf{CO}_t (t\in T)$ based on subsystems' abstractions also can make remove conflicts in the joint behavior of subsystems, which is shown following.
%
%主要是经过step2之后我们还是可以保证nonblocking
%我们cluster组合后不会忽视supi
%各个cluster好好地被observer和occ
\begin{proof}[Proof of Theorem 1]

Consider a system with $I$ specification models. After step 2, $I$ decentralized supervisors $\textbf{SUP}_i\{i\in I,I\in\mathbb{N}^+\}$ are partitioned into $N$ clusters$\{1,\dots N\}$.
In this level 1,
let a set $\mathcal{X}_{1,n}\{n\in N,N\in\mathbb{N}^+\}$ contains all index $i$ of decentralized supervisors $\textbf{SUP}_i$ in each cluster.
Each cluster will form by synchronous product a subsystem $\textbf{SUB}_{1,n}\{n\in N,N\in\mathbb{N}^+\}$, written $\textbf{SUB}_{1,n} = ||\{\textbf{SUP}_i|i\in \mathcal{X}_{1,n}\}$.
The subsystem $\textbf{SUB}_{1,n} = ||_{i\in \mathcal{X}_{1,n}}(\textbf{SUP}_i)||\textbf{CO}_{h}\{h\in H,H\in\mathbb{N}^+\}$ as in step 3 is nonblocking, namely
%
%
\begin{eqnarray}
(||_{i\in \mathcal{X}_{1,n}}L(\textbf{SUP}_i))||L(\textbf{CO}_{h})
=\overline{||_{i\in \mathcal{X}_{1,n}}L_m(\textbf{SUP}_i)||L_m(\textbf{CO}_{h})}
\end{eqnarray}
%
In this level 1, $N$ abstractions $\textbf{ABS}_{1,n}\{n\in N,N\in\mathbb{N}^+\}$ as in step 4 are obtained by natural projection $\textit{P}_{1,n}$ from $\textbf{SUB}_{1,n} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{1,n})=\textit{P}_{1,n} L(\textbf{SUB}_{1,n}), L_m(\textbf{ABS}_{1,n})=\textit{P}_{1,n} L_m(\textbf{SUB}_{1,n})
\end{eqnarray}
%
and the projection $P_{1,n}$ in step 4 is an $L_m(\textbf{SUB}_{1,n})$-observer and OCC for $L_m(\textbf{SUB}_{1,n})$.

When the number of clusters is bigger than two, we do further clustering of abstractions $\textbf{ABS}_{1,n}$. 
After second level clustering, consider we get $N$ clusters in this level 2 and 
the set $\mathcal{X}_{2,n}\{n\in N,N\in\mathbb{N}^+\}$ contains all index $n$ of level 1 abstractions $\textbf{ABS}_{1,n}$ in each cluster.
Each cluster will be synthesized into a subsystem $\textbf{SUB}_{2,n}\{n\in N,N\in\mathbb{N}^+\}$, written $\textbf{SUB}_{2,n} = ||\{\textbf{ABS}_{1,n}\{n\in \mathcal{X}_{2,n}\}$.
The subsystem 
\[\textbf{SUB}_{2,n} = ||_{n\in \mathcal{X}_{2,n}}(\textbf{ABS}_{1,n})||\textbf{CO}_{h}\{h\in H,H\in\mathbb{N}^+\}
\]as in step 3 is nonblocking, namely
%
%
\begin{eqnarray}
||_{n\in \mathcal{X}_{2,n}}L(\textbf{ABS}_{1,n})||L(\textbf{CO}_{h})
=\overline{||_{n\in \mathcal{X}_{2,n}}L_m(\textbf{ABS}_{1,n})||L_m(\textbf{CO}_{h})}
\end{eqnarray}
%
By Proposition \ref{prop1}, we can say that the coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{1,n}\{n\in \mathcal{X}_{2,n}\}$ also can remove the conflicts between subsystems $\textbf{SUB}_{1,n}\{n\in \mathcal{X}_{2,n}\}$ : 
%
\begin{eqnarray}
||_{n\in \mathcal{X}_{2,n}}L(\textbf{SUB}_{1,n})||L(\textbf{CO}_{h})
=\overline{||_{n\in \mathcal{X}_{2,n}}L_m(\textbf{SUB}_{1,n})||L_m(\textbf{CO}_{h})}
\end{eqnarray}
%
In this level $2$, $N$ abstractions $\textbf{ABS}_{2,n}\{n\in N,N\in\mathbb{N}^+\}$ as in step 4 are obtained by natural projection $\textit{P}_{2,n}$ from $\textbf{SUB}_{2,n} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{2,n})=\textit{P}_{2,n} L(\textbf{SUB}_{2,n}), L_m(\textbf{ABS}_{2,n})=\textit{P}_{2,n} L_m(\textbf{SUB}_{2,n})
\end{eqnarray}
%
and the projection $P_{2,n}$ in step 4 is an $L_m(\textbf{SUB}_{2,n})$-observer and
OCC for $L_m(\textbf{SUB}_{2,n})$.

Consider we do clustering $L\{L\in\mathbb{N}^+\}$ times to produce $L$ levels abstractions.  In the level $L$, let $\mathcal{X}_{L,n}\{n\in N,N\in\mathbb{N}^+\}$ contains all index $n$ of the level $(L-1)$ abstractions $\textbf{ABS}_{(L-1,n)}$ in each cluster. 

%
The subsystem 
\[\textbf{SUB}_{L,n} = ||_{n\in \mathcal{X}_{L,n}}(\textbf{ABS}_{(L-1,n)})||\textbf{CO}_{h}\{h\in H,H\in\mathbb{N}^+\}
\]as in step 3 is nonblocking, namely
%
%
\begin{eqnarray}
||_{n\in \mathcal{X}_{L,n}}L(\textbf{ABS}_{(L-1,n)})||L(\textbf{CO}_{h})
=\overline{||_{n\in \mathcal{X}_{L,n}}L_m(\textbf{ABS}_{(L-1,n)})||L_m(\textbf{CO}_{h})}
\end{eqnarray}
%
Since the natural projection $\textit{P}_{(L-1,n)}$ from $\textbf{SUB}_{(L-1,n)} $:
%
\footnotesize
\begin{eqnarray}
L(\textbf{ABS}_{(L-1,n)})=\textit{P}_{(L-1,n)} L(\textbf{SUB}_{(L-1,n)}),
L_m(\textbf{ABS}_{(L-1,n)})=\textit{P}_{(L-1,n)} L_m(\textbf{SUB}_{(L-1,n)})
\end{eqnarray}
\normalsize
%
is an $L_m(\textbf{SUB}_{2,n})$-observer and OCC for $L_m(\textbf{SUB}_{(L-1,n)})$. 
The coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{(L-1,n)}\{n\in \mathcal{X}_{L,n}\}$ also can remove the conflicts between subsystems $\textbf{SUB}_{(L-1,n)}\{n\in \mathcal{X}_{L,n}\}$ : 
%
\begin{eqnarray}
||_{n\in \mathcal{X}_{L,n}}L(\textbf{SUB}_{(L-1,n)})||L(\textbf{CO}_{h})
=\overline{||_{n\in \mathcal{X}_{L,n}}
L_m(\textbf{SUB}_{(L-1,n)})||L_m(\textbf{CO}_{h})}
\end{eqnarray}

In this level $L$, $N$ abstractions $\textbf{ABS}_{L,n}\{n\in N,N\in\mathbb{N}^+\}$ as in step 4 are obtained by natural projection $\textit{P}_{L,n}$ from $\textbf{SUB}_{L,n} $:
%
\begin{eqnarray}
L(\textbf{ABS}_{L,n})=\textit{P}_{L,n} L(\textbf{SUB}_{L,n}), L_m(\textbf{ABS}_{L,n})=\textit{P}_{L,n} L_m(\textbf{SUB}_{L,n})
\end{eqnarray}
%
and the projection $P_{L,n}$ in step 4 is an $L_m(\textbf{SUB}_{L,n})$-observer and
OCC for $L_m(\textbf{SUB}_{L,n})$.


If the number of clusters in this level $L$ is not greater than two, 
namely $N\leq 2$, we do not do any further clustering of abstractions. By Proposition \ref{prop1}, we can also say that the coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{L,n}$ also can remove the conflicts between subsystems $\textbf{SUB}_{L,n}$ : 



%\footnotesize
%\begin{eqnarray}
%(||_{n\in N} L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(||_{t\in T}L_m(\textbf{CO})})
%\end{eqnarray}
%\normalsize
%

%
\begin{eqnarray}
(||_{n\in N} L(\textbf{SUB}_{L,n}))||(L(\textbf{CO}_h))
=\overline{(||_{n\in N}L_m(\textbf{SUB}_{L,n}))||(L_m(\textbf{CO}_h)})
\end{eqnarray}
%
Since in each level $l\in L$ of natural projection satisfies $L_m(\textbf{SUB})$-observer and OCC for $L_m(\textbf{SUB})$. Removing each subsystem's internal conflict is equivalent to removing the conflict between subsystems at a lower layer contained in this subsystem before it was abstracted. After the conflicts at the top layer are removed, the conflicts between all elements at the bottom layer are also removed:
\begin{eqnarray}
||_{i\in I} L(\textbf{SUP}_i) ||_{h\in H}L(\textbf{CO})= 
\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||_{h\in H}L_m(\textbf{CO})}\\
\end{eqnarray}
This completes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%Trash%%%%%%%%%%%%%%%%%%%
\begin{comment}

\begin{thm}\label{thm1}
Consider decentralized supervisors $\textbf{SUP}_i(i\in I)$ as in step 1, subsystems $\textbf{SUB}_n(n\in N)$ as in step 3 and coordinator $\textbf{CO}_w(w\in W)$ as in step 3 and step 6 based on subsystem's abstractions. If for every $n \in N$, 
$P_n$ is an $L_m(\textbf{SUB}_n)$-observer and OCC for $L_m(\textbf{SUB}_n)$, then
\footnotesize
\begin{eqnarray}
%||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))= 
%\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}\\
%(||_{i\in I} \textbf{SUP}_i)|| (||_{w\in W}\textbf{CO}_w)=\textbf{SUP}
||_{i\in I} L(\textbf{SUP}_i) ||_{w\in W}L(\textbf{CO}_w)||L(\textbf{G})=L(\textbf{SUP})\\
||_{i\in I} L_m(\textbf{SUP}_i) ||_{w\in W}L_m(\textbf{CO}_w)||L_m(\textbf{G})=L_m(\textbf{SUP})
\end{eqnarray}
\normalsize
\end{thm}

The clustering only does partitioning and does not delete any element ($\textbf{SUP}_i$). Therefore, the synthesis of all clusters equals the synthesis of all decentralized supervisors:
%
\footnotesize
\begin{eqnarray}
||_{n\in N}L(\textbf{SUB}_{n})=
(||_{i \in I}L(\textbf{SUP}_{i}))||(||_{h \in H}L(\textbf{CO}_{h}))
\end{eqnarray}
\normalsize
%
Let $W (w\in W)$ be the new indexs of all coordinators, 
the equation $(30)$ becomes:

%
%\footnotesize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(L(\textbf{CO}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(L_m(\textbf{CO}))}\\
%=\overline{(||_{n\in N}(||_{i\in CLS_n}L_m(\textbf{SUP}_i)||L_m(\textbf{CO}_{h})))||(L_m(\textbf{CO}))}\\
%(||_{n\in N}\textbf{SUB}_{n})||(||_{h\in H}L(\textbf{CO}_h)) = (||_{i\in I} L(\textbf{SUP}_i)) ||(||_{h\in H}L(\textbf{CO}_h))
%\end{eqnarray*}
%\normalsize
%



%
%\footnotesize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}_{t}))
%=\overline{(||_{n\in N}L_m(\textbf{SUB}_{n}))||(||_{t\in T}L_m(\textbf{CO}_{t}))}\\
%=\overline{(||_{n\in N}(||_{i\in CLS_n}L_m(\textbf{SUP}_i)||L_m(\textbf{CO}_{h})))||(||_{t\in T}L_m(\textbf{CO}_{t}))}\\
%(||_{n\in N}\textbf{SUB}_{n})||(||_{h\in H}L(\textbf{CO}_h)) = (||_{i\in I} L(\textbf{SUP}_i)) ||(||_{h\in H}L(\textbf{CO}_h))
%\end{eqnarray*}
%\normalsize
%

%\scriptsize
%\begin{eqnarray*}
%(||_{n\in N}L(\textbf{SUB}_{n}))||(||_{t\in T}L(\textbf{CO}_{t}))=
%(||_{i\in I} L(\textbf{SUP}_i))||(||_{h\in H}L(\textbf{CO}_h))||(||_{t\in T}L(\textbf{CO}_{t}))\\
%=\overline{(||_{i\in I} L_m(\textbf{SUP}_i))||(||_{h\in H}L_m(\textbf{CO}_h))(||_{t\in T}L_m(\textbf{CO}_{t}))}
%\end{eqnarray*}
%\normalsize
%
%Since $h\in H$ and $t\in T$ only are the indexs of coordinators, we put $W=H+T$ and relabel each of coordinators by $w, w\in W$.
%
\footnotesize
\begin{eqnarray*}
%(||_{i\in I} L(\textbf{SUP}_i))||(||_{h\in H}L(\textbf{CO}_h))||(||_{t\in T}L(\textbf{CO}_{t}))
%=||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))\\
||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))
=\overline{||{}_{i\in I}L_m(\textbf{SUP}_i)||(||_{w\in W}L_m(\textbf{CO}_w))}
\end{eqnarray*}
\normalsize
%
Therefore, the synchronized behavior of $I$ decentralized supervisors $\textbf{SUP}_i$ and $W$ coordinators $\textbf{CO}_w$ is nonblocking. Since coordinator only remove the conflicts that proven in \cite{Feng2008},
\footnotesize
\begin{eqnarray*}
||_{i\in I} L(\textbf{SUP}_i) || (||_{w\in W}L(\textbf{CO}_w))=L(\textbf{SUP})\\
||_{i\in I} L_m(\textbf{SUP}_i) || (||_{w\in W}L_m(\textbf{CO}_w))=L_m(\textbf{SUP})
\end{eqnarray*}
\normalsize

When the number of clusters in this level 1 is not greater than two, namely $N\leq 2$, we do not do any further clustering of abstractions. By Proposition \ref{prop1}, we can say that the coordinator $\textbf{CO}_h$  based on abstractions $\textbf{ABS}_{1,n}$ also can remove the conflicts between subsystems $\textbf{SUB}_{1,n}$ : 
%
\begin{eqnarray}
(||_{n\in N} L(\textbf{SUB}_{1,n}))||_{h\in H}(L(\textbf{CO}_h))
=\overline{(||_{n\in N}L_m(\textbf{SUB}_{1,n}))||_{h\in H}(L_m(\textbf{CO}_h)})
\end{eqnarray}
%

Consider $I$ decentralized supervisors $\textbf{SUP}_i \{i\in I,I\in\mathbb{N}^+\}$ as in step 1.
After $L\{L\in\mathbb{N}^+\}$ levels clustering and abstraction, in each level $l\in L$, consider there are $N$ subsystems $\textbf{SUB}_{l,n}\{n\in N,N\in\mathbb{N}^+\}$ as in step 3 based on subsystem's abstractions.
$H$ coordinators $\textbf{CO}_h\{h\in H,H\in\mathbb{N}^+\}$ as in step 3 and step 6 be designed to remove conflicts of subsystems.
If for every $l \in L$, $n \in N$, 
$P_{l,n}$ is an $L_m(\textbf{SUB}_{l,n})$-observer and OCC for $L_m(\textbf{SUB}_{l,n})$, then

\end{comment}
